Testing of Index-Invariant Properties in the Huge Object Model

The study of distribution testing has become ubiquitous in the area of property testing, both for its theoretical appeal, as well as for its applications in other fields of Computer Science. The original distribution testing model relies on samples drawn independently from the distribution to be tested. However, when testing distributions over the $n$-dimensional Hamming cube $\left\{0,1\right\}^{n}$ for a large $n$, even reading a few samples is infeasible. To address this, Goldreich and Ron [ITCS 2022] have defined a model called the huge object model, in which the samples may only be queried in a few places. In this work, we initiate a study of a general class of properties in the huge object model, those that are invariant under a permutation of the indices of the vectors in $\left\{0,1\right\}^{n}$, while still not being necessarily fully symmetric as per the definition used in traditional distribution testing. We prove that every index-invariant property satisfying a bounded VC-dimension restriction admits a property tester with a number of queries independent of n. To complement this result, we argue that satisfying only index-invariance or only a VC-dimension bound is insufficient to guarantee a tester whose query complexity is independent of n. Moreover, we prove that the dependency of sample and query complexities of our tester on the VC-dimension is tight. As a second part of this work, we address the question of the number of queries required for non-adaptive testing. We show that it can be at most quadratic in the number of queries required for an adaptive tester of index-invariant properties. This is in contrast with the tight exponential gap for general non-index-invariant properties. Finally, we provide an index-invariant property for which the quadratic gap between adaptive and non-adaptive query complexities for testing is almost tight.

==> Algorithm.tex <==
\begin{algorithm}
%\scriptsize

\SetAlgoLined

\caption{\learn}
\label{alg:testcluster--}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^n$, and parameters $\zeta,\delta, r$ with $\zeta ,\delta \in (0,1)$ and $r \in \N$. }
\KwOut{Either reports a full description of a distribution over $\{0,1\}^n$ or {\sc Fail}, satisfying (i) and (ii) as stated in Theorem~\ref{theo:mainthm1}.}
%\LinesNumbered
\begin{description}
\item[(i)] Take $t_1=\Oh(\frac{r}{\zeta} \log \frac{r}{\zeta})$ samples $\mathcal{S} = \mathbf{X}_1, \dots, \mathbf{X}_{t_1}$ from $D$.

\item[(ii)] Take $t_2=\Oh(\frac{t_1^2}{\zeta^2} \log t_1)$ samples $\cT=\mathbf{Y}_1, \dots, \mathbf{Y}_{t_2}$ from $D$.

\item[(iii)]  Pick a random subset $R \subset [n]$ with $\size{R}=\Oh(\frac{r}{\delta^2\zeta} \log \frac{r}{\delta\zeta})$. Query the indices corresponding to $R$ in each sample in $\cS$, to obtain the sequence of vectors $\mathcal{S}_x = \mathbf{x}_1, \dots, \mathbf{x}_{t_1}$,  where $\mathbf{x}_{i} = \mathbf{X}_i\mid_R$ for each $i \in [t_1]$. Also,  query the indices corresponding to $R$ in each sample in $\cT$, to obtain the sequence of vectors $\mathcal{T}_y = \mathbf{y}_1, \dots, \mathbf{y}_{t_2}$, where $\mathbf{y}_{i} = \mathbf{Y}_i\mid_R$ for each $i \in [t_2]$.

\item[(iv)] For $j = 1, \ldots, t_2$,  if there exists an $i \in [t_1]$ such that $d_H(\mathbf{y}_j, \mathbf{x}_i)\leq 2 \delta$, assign $\mathbf{y}_j$ to $\mathbf{x}_i$, breaking ties by assigning $\mathbf{y}_j$ to the vector in $\mathcal{S}_x$ with the minimum index.

If for some $\mathbf{y}_j$ no suitable $\mathbf{x}_i$ is found, then $\mathbf{y}_j$ remains unassigned.

\item[(v)] If the total number of unassigned vectors in $\mathcal{T}_y$ is more than $3\zeta t_2$, then output {\sc Fail}.

\item[(vi)] For each $i \in 1, \dots, t_1$, the weight of $\mathbf{x}_i$ is defined as 
$$w_i=w(\mathbf{x}_i)=\frac{\mbox{Number of vectors in } \mathcal{T}_y \mbox{ assigned to } \mathbf{x}_i}{t_2}.$$
%and $w_0=1-\sum\limits_{i=1}^{t_1} w_i$.

\item[(vii)] Use \aprox (as described in Algorithm~\ref{alg:approx}) with $R$ and $\mathbf{x}_1, \ldots, \mathbf{x}_{t_1}$ to obtain $\mathbf{S}_1, \ldots, \mathbf{S}_{t_1} \in \{0,1\}^n$ (as stated in Lemma~\ref{lem:approxguarantee}).
    
    
    %Call \est with $\mathbf{O}_1, \ldots, \mathbf{O}_m$ obtained from Step (i). Let us assume $\mathbf{C}_1, \ldots, \mathbf{C}_m$ be the set of centers returned by \est.
    
%\item[(viii)] \comments{Find a vector $\mathbf{s}_0$ which is $\frac{\delta}{10}$-far from all the vectors $\mathbf{s}_1, \ldots, \mathbf{s}_{t_1}$.}
    
\item[(viii)] Construct and return any distribution $D'$ over $\{0,1\}^n$ such that 
\begin{itemize}
    \item For each $i = 1, \dots, t_1$,  $D'(\mathbf{S}_i) \geq w(\mathbf{x}_i)$;
   % \item $D'(\mathbf{s}_0) = 1 - \sum\limits_{i=1}^{t_1} w({\mathbf{s}_i^{(1)}})$
   \item $\sum\limits_{i=1}^{t_1} D'(\mathbf{S}_i)=1$;
    \item $D'(\mathbf{S})=0$ for all $\mathbf{S} \in \{0,1\}^n \setminus \{\mathbf{S}_1, \ldots, \mathbf{S}_{t_1}\}$.
\end{itemize}
\end{description}
\end{algorithm}

\begin{algorithm}
%\scriptsize

\SetAlgoLined

\caption{\aprox}
\label{alg:approx}
\KwIn{A random subset $R \subseteq [n]$ with $\size{R}=\Oh(\frac{r}{\delta^2\zeta} \log \frac{r}{\delta\zeta})$, and a sequence of vectors $\mathbf{x}_1, \ldots,\mathbf{x}_{t_1} \in \{0,1\}^{\size{R}}$ drawn from the distribution $D\mid_{R}$.}
\KwOut{Sequence of vectors $\mathbf{S}_1, \ldots, \mathbf{S}_{t_1}$ such that, with probability $99/100$ over the random choice of $R$, for all $i \in [t_1]$, $d_H(\sigma(\mathbf{X}_i), \mathbf{S}_i) \leq \delta/10$, where $\sigma: [n] \rightarrow [n]$ is some  permutation.}
\LinesNumbered
\begin{description}
     \item[(i)] For each $i \in R$,  construct the vector $\mathbf{C}_i \in \{0,1\}^{t_1}$ such that $\mathbf{C}_i(j) = \mathbf{x}_j(i)$.
     %whose $j$-th bit is same as the $i$-th bit of $\mathbf{x}_j$, for every $j \in [{t_1}]$.
    
    
    \item[(ii)] For any $J\in \{0,1\}^{t_1}$, determine 
    $\gamma_J=\frac{|\{i\in R\mid \mathbf{C}_i = J\}|}{\size{R}}$.
    

    \item[(iii)] Apply Observation~\ref{obs:integral}, to obtain for any $J\in \{0,1\}^{t_1}$ an approximation $\Gamma_J$, such that $\Gamma_J \in \{\lfloor \gamma_J \cdot n\rfloor, \lceil \gamma_J \cdot n\rceil \}$ and $\sum\limits_{J\in \{0,1\}^{t_1}}\Gamma_J = n$.
    
    \item[(v)]
    Construct a matrix $A$ of dimension $t_1 \times n$ by putting $\Gamma_J$ many $J$ column vectors, for each $J \in \{0,1\}^{t_1}$. 
    
    \item[(vi)] Return the row vectors of the matrix as $\mathbf{S}_1,\ldots,\mathbf{S}_{t_1}$.
    
    
    
    %Determine a set of $m$ vectors $\mathbf{x}_1,\ldots,\mathbf{x}_{t_1}$ by using the procedure described in the proof of Observation~\ref{obs:approxcluster} such that  $\mu(\mathbf{x}_i ,\sigma(\mathbf{O}_i)) \leq \frac{1}{2^{t_1}}\sum\limits_{j \in [2^{t_1}]}\size{a_j-\size{T_j}} $ for some permutation $\sigma:[n]\rightarrow [n]$. 
    %(We are applying Observation~\ref{obs:approxcluster} with $k=t_1$, $\mathbf{v}_1 = \mathbf{O}_1, \ldots, \mathbf{v}_{t_1} = \mathbf{O}_{t_1}$ and $\widetilde{\mathbf{v}_1} = \mathbf{x}_1, \ldots, \widetilde{\mathbf{v}_{t_1}} = \mathbf{x}_{t_1}$).
    
    
    %Using $t_1, \ldots, t_{2^m})$, construct approximate cluster centers $C_1, \ldots, C_m$ as described in Observation~\ref{obs:approxcluster}. {\sc Return} $C_1, \ldots, C_m$.
    
    %Using the vectors $q_1, \ldots, q_{K}$ along with $T_1, \ldots, T_{2^{m}}$, construct the approximate centers $C_1, \ldots, C_{m}$. 
    
    %\item[(iv)] Return $C_1, \ldots, C_{m}$.
    
    
\end{description}

\end{algorithm}






==> name.tex <==
\subsection{Determining the permutation $\pi$}\label{sec:quadratic_determine_permutation}

%\comments{
Here we design an algorithm that, given a distribution $D \in \cP_{\mbox{Gap}}$, can learn the permutation $\pi$ for which $D_{\pi} \in P^0_{\mbox{Gap}}$ with high probability. 

The crux of the algorithm is that if $D \in \cP_{\mbox{Gap}}$, then there exist $\mathbf{U}'=\mathbf{U}_\pi \in \{0,1\}^n$, $\cS'=\{\mathbf{\mathbf{V}}_i'=(\mathbf{V}_i)_\pi: i \in [b]\}$ and $\cT'=\{\mathbf{W}_j'=(\mathbf{W}_j)_\pi:j \in \{0\}\cup [\lceil \log kn\rceil]-1\}$ in the support of $D$ such that $D(\mathbf{U}')=\alpha$, $D(\mathbf{V}_i')=\alpha/b$ for every $i \in [b]$ and  $D(\mathbf{W}_j')=\alpha/\lceil \log kn\rceil$. \comments{Note that $\mathbf{U},\mathbf{V}_i$'s and $\mathbf{V}_j$'s are as defined in the property $\cP_{\mbox{Gap}}^0$}. The main observation is that, if we are given the set of special vectors $\{\mathbf{U'}\} \cup \cS' \cup \cT'$, then we can determine the permutation $\pi$. Our algorithm can find  $\mathbf{U}', \cS'$ and $\cT'$ with high probability, if they exist, by taking $\Oh(\log^2 N/\alpha)=\Oh(\log^2 n/\alpha)$ samples and reading them in their entirety. This is due to the fact that the probability mass of every vector in the set of special vectors is at least $\Omega(\alpha/\log n)$.

%}

The algorithm is described in the following subroutine \findpi (see Algorithm~\ref{algo:perm})~\footnote{This algorithm is not adaptive in itself, but its output is used adaptively in the testing algorithm described later.}.

\begin{algorithm}[H]\label{algo:perm}
%\scriptsize

\SetAlgoLined

\caption{\findpi}
\label{alg:findpi}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^N$.}
\KwOut{Either a permutation $\pi:[N] \rightarrow [N]$, or {\sc Fail}.}
\LinesNumbered
\begin{description}
     \item[(i)] First take a multi-set $\cX$ of $\Oh(\log^2 N/\alpha)$ samples from $D$, and query all the entries of the sampled vectors of $\cX$ to know the vectors of $\cX$ completely.
    
    
    \item[(ii)] Find the set of distinct vectors in $\cX$ that have exactly one $1$. If no such vector exists or there is more than one such vector, {\sc Fail}. Otherwise, denote by $\mathbf{U'}$ the vector that has exactly one $1$, and denote the corresponding index by $i^*$. Set $\pi(i^*)=1$, and proceed to the next step.    
    %let the vector be $\mathbf{U'}$ that has $1$ at the index $i^*$. 
    

    \item[(iii)] Find the set of distinct vectors $\cS' \subseteq \cX \setminus \{\mathbf{U'}\}$ such that every vector in $\cS'$ has $1$ at the index $i^*$ and has at least another $1$ among other indices. If no such vector exists, or $\size{\cS'} \neq b$, {\sc Fail}. Otherwise, if the vectors of $\cS'$ form a chain $\mathbf{V}'_1, \ldots, \mathbf{V}'_b$, where $\mathbf{V}'_j$ has exactly $j+1$ many $1$, then set $\pi(i_j)=j+1$, where $i_j$ is the index where $\mathbf{V}'_j$ has $1$, but $\mathbf{V}'_{j-1}$ has $0$ there, for every $j \in [b]$ (denoting $\mathbf{V'}_0=\mathbf{U'}$ for the purpose here). Also, set $B'=(i_1, \ldots,i_b)$. If $\cS'$ does not form a chain $\mathbf{V}'_1, \ldots, \mathbf{V}'_b$ as mentioned above, {\sc Fail}.
    
    
    \item[(iv)] Let $\cT' \subseteq \cX$ be the set of distinct vectors such that every vector in $\cT'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. If no such vector exists, {\sc Fail}. For every $j$, denote by $\mathbf{W}'_j$ the vector in $\cT'$ for which $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$. For every $j \in \{0\} \cup [\lceil \log kn \rceil -1]$, if either there are no vectors $\mathbf{W}'_j \in \cT'$ or there is more than one distinct vector with $\mathbf{W'_j} \mid_{B'}=b(j)$, {\sc Fail}.
    Also, if there is any vector in $\mathbf{W}'_j \in \cT'$ such that $\mathbf{W}'_j \mid_{B'} = b(j)$ for $\log kn \leq j < 2^b -1$, {\sc Fail}.
    
    \item[(v)] For any $i \in [N]\setminus (\{i^*\} \cup B')$, let $l_i$ be the integer with binary representation $(\mathbf{W'}_0)_i, \ldots, (\mathbf{W'}_{\lceil \log kn \rceil -1})_i$.
Set $\pi(i)=b+2+l_i$ for every $i \in [N]\setminus (\{i^*\} \cup B')$. If $\pi$ is not a permutation of $[N]$, {\sc Fail}.

    \item[(vi)] Take another multi-set $\cX'$ of $\Oh(\log^2 N/\alpha)$ samples from $D$, and query all the entries of the sampled vectors of $\cX'$ to know the vectors of $\cX'$ completely. Let $\cY$ be a set of vectors in $\cX'$ such that $\cY=\{\mathbf{Z} \in \cX': \mathbf{Z} \mid_{{\{i^*\} \cup B'}} \neq \mathbf{0}\mathbf{1}^b \}$. If $\size{\cY}/\size{\cX'} > 4\alpha$, {\sc Fail}. Otherwise, output $\pi$.
    
    %Estimate the fraction of vectors in $X'$ that are in $\{\mathbf{U'}\}\cup S' \cup T'$. If it is less than $4\alpha$. Otherwise, {\sc Fail}.
    
\end{description}

\end{algorithm}

\vspace{10pt}

Let us start by analyzing  the query complexity of \findpi.

\begin{lem}[Query complexity of \findpi]\label{lem:queryfindpi}
The query complexity of the above defined \findpi is $\tOh(N)$.
\end{lem}

\begin{proof}
Note that \findpi takes a multi-set $\cX$ of $\Oh(\log^2 N/\alpha)$ samples from $D$ in Step (i), and queries them completely. So, \findpi performs $\Oh(N \log^2 N/\alpha)$ queries in Step (i). \findpi does not perform any new query in Step (ii), Step (iii), Step (iv) and Step (v). Finally, \findpi takes another multi-set $\cX'$ of $\Oh(\log^2 N/\alpha)$ samples from $D$ and queries them completely, similar to Step (i). Recalling that $\alpha=1/\log n$, the query complexity of \findpi is $\tOh(N)= \tOh(n)$ in total.
\end{proof}


Now we proceed to prove the correctness of \findpi.
\color{blue}
\begin{lem}[Guarantee when $D \in \cP_{\mbox{Gap}}$]\label{lem:findpicompleteness}
If $D$ is a distribution defined over $\{0,1\}^N$ such that $D \in \cP_{\mbox{Gap}}$, then with probability at least $9/10$, \findpi reports permutation $\pi$ such that $D_{\pi} \in \cP_{\mbox{Gap}}^0$.
\end{lem}

We prove the above lemma by a series of intermediate lemmas. \color{black} In the following lemmas, we consider $\mathbf{U}$, $\cS$ and $\cT$ as per the definition of $\cP^0_{\mbox{Gap}}$. Also, consider the permutation $\pi$ such that $D_\pi \in \cP_{\mbox{Gap}}$.
%To argue the completeness of our algorithm, consider a distribution $D$ over $\{0,1\}^N$ such that $D\in \cP_{\mbox{Gap}}$, and let $\pi$ be the permutation for which $D_{\pi} \in \cP^0_{\mbox{Gap}}$. 

%Now consider the following lemma.

%So, there exists the four types of vectors as described in the definition of $\cP_{\mbox{Gap}}$. By using Chernoff bound, we have the following:

\begin{lem}[correctly finding $\pi^{-1}(1)$]\label{lem:hittingU}
With probability at least $1-1/N^3$, $\cX$ will contain the vector $\mathbf{U'}$ for which $\mathbf{U'}_{\pi}=\mathbf{U}$, and $i^*=\pi^{-1}(1)$ will be identified correctly.
\comments{Moreover, \findpi proceeds to Step (iii).}
%Let $\mathbf{U'} \in \{0,1\}^N$ be a vector that has exactly a single $1$ at some index $i^*$, and $D$ be a distribution over $\{0,1\}^N$ such that $D(\mathbf{U'})= \alpha$. Consider the multi-set of samples $X$ taken from $D$ in Step (i) of \findpi such that $\size{X} = \Oh(\log^2 N/\alpha)$. Then with probability at least $1 - \frac{1}{N^3}$, $\mathbf{U'} \in X$. 
\end{lem}

\begin{proof}
By the definition of $\cP^0_{\mbox{Gap}}$, the vector $\mathbf{U'}$ is the only vector in the support of $D$ containing a single $1$. Since $D(\mathbf{U'}) = D(\mathbf{U}_{\pi^{-1}(1)}) = \alpha$, and we are taking $\size{\cX}$ many samples from $D$, the probability that $\mathbf{U'}$ will not appear in $\cX$ is at most $(1- \alpha)^{\size{X}} \leq \frac{1}{N^3}$. Thus, with probability at least $1 - \frac{1}{N^3}$, $\mathbf{U'} \in \cX$ and \findpi in Step (ii) proceeds to the next step
%This completes the proof of the lemma.
\end{proof}

\begin{lem}[correctly finding $B' = \pi^{-1}(B)$]\label{lem:hittingS}
With probability at least $1-1/N^3$, the algorithm \findpi will correctly identify $\mathbf{V'}_1, \ldots, \mathbf{V'}_b$ for which $\mathbf{V'}_{i,\pi} = \mathbf{V}_i$, and $B'={\pi^{-1}(2), \ldots, \pi^{-1}(b+1)}$ will be identified correctly as well. \comments{Moreover, \findpi proceeds to Step (iv).}

%Let $S'= \{\mathbf{V}'_1, \ldots, \mathbf{V}'_b\}$ be a set of vectors in $\{0,1\}^N$ such that for each $\mathbf{V}'_i \in S'$, $\mathbf{V}'_i$ has $1$ at some index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B$. Moreover, $D(\mathbf{V}'_i) = \alpha/b$ for each $i \in [b]$. Then with probability at least $1 - \frac{1}{N^3}$, $S' \subseteq X$, where $X$ is the multi-set of samples obtained from $D$ and $\size{X}= \Oh(\log^2 N/\alpha)$.
\end{lem}

\begin{proof}
%Let us consider an arbitrary vector $\mathbf{V}'_i \in S'$.

Let $\mathbf{V'}_1, \ldots, \mathbf{V'}_b$ denote the vectors for which $\mathbf{V'}_{i,\pi}=\mathbf{V}_i$ for every $i$. Note that these are the only vectors outside $\mathbf{U'}$ in the support of $D$ that have $1$ at the index $i^*$.
As $D(\mathbf{V}'_i)= \frac{\alpha}{b}$, the probability that $\mathbf{V}'_i$ does not appear in $\cX$ is at most $(1- \frac{\alpha}{b})^{\size{X}}$. Since $\size{\cX} = \Oh(\log^2 N/\alpha)$ and $b = \Oh(\log \log kn)$, the probability that $\mathbf{V}'_i \in \cX$ is at least $1 - \frac{1}{N^4}$. Using the union bound over all the vectors of $\cS'$, with probability at least $1-1/N^3$, we know that all of these vectors are in $\cX$, in which case they are identified correctly, so $B'$ is identified correctly as well, and \findpi in Step (iii) proceeds to the next step.
\end{proof}

\begin{lem}[correctly identifying $\pi^{-1}(b+2), \ldots, \pi^{-1}(N)$]\label{lem:hittingT}
Let $\mathbf{W'}_1, \ldots, \mathbf{W'}_{\lceil \log kn \rceil -1}$ denote the vectors for which $\mathbf{W'}_{j,\pi} = \mathbf{W}_j$ for every $j$. With probability at least $1-1/N^3$, all these vectors appear in $\cX$, in which case they are identified correctly, and so are $\pi^{-1}(b+2), \ldots, \pi^{-1}(N)$. \comments{Moreover, \findpi proceeds to Step (vi).}

%Let $T'= \{\mathbf{W}'_1, \ldots, \mathbf{W}'_{\log kn}\}$ be a set of vectors (disjoint from $S'$) in $\{0,1\}^N$ such that for each $\mathbf{W}'_i \in T'$, $\mathbf{W}'_i$ contains $1$ at the index $i^*$, for every $i \in [\log n]$, the decimal evaluation of $\mathbf{W}'_i \mid_{B'}$ is $i$. Moreover, $D(\mathbf{W}'_i) = \alpha/\log kn$ for each $i \in \{0\} \cup [\log kn -1]$. Then with probability at least $1 - \frac{1}{N^3}$, $T' \subseteq X$, where $X$ is the multi-set of samples obtained from $D$ and $\size{X}= \Oh(\log^2 N/\alpha)$.
\end{lem}

The proof of the above lemma is similar to the proof of Lemma~\ref{lem:hittingS} and is omitted. Note that from Lemma~\ref{lem:hittingU}, Lemma~\ref{lem:hittingS} and Lemma~\ref{lem:hittingT}, we know that with probability at least $1-o(1)$, the algorithm \findpi has correctly determined the permutation $\pi$ and proceeded to Step (vi). We will finish up the proof of Lemma~\ref{lem:findpicompleteness} having the following lemma.

%proceeded to Step (v). Since the vectors in $\{\mathbf{U}\} \cup S \cup T$ are disjoint, \findpi correctly determines the permutation $\pi$ with probability at least $1-o(1)$.

\begin{lem}
The probability that \findpi outputs {\sc Fail} in Step (vi) (instead of outputting $\pi$) is at most $1/N^3$.

%With probability at least $1 - \frac{1}{N^3}$, $\size{\cY}/\size{X'} \leq 4 \alpha$.
%the fraction of vectors in $X'$ that are in $\{\mathbf{U}\} \cup S \cup T$ is at most $4 \alpha$.
\end{lem}

\begin{proof}
As $D \in \cP_{\mbox{Gap}}$, from the description of the property, we know that $D(\{\mathbf{U'}\} \cup \cS' \cup \cT')= 3 \alpha$. As $\size{\cX'}= \Oh(\log^2 N/\alpha)$, using the Chernoff bound, we have the result.
\end{proof}

Combining the above lemmas, we conclude that with probability at least $9/10$, the algorithm \findpi outputs a correct permutation $\pi$, completing the proof of Lemma~\ref{lem:findpicompleteness}.

To conclude this section, we show that with high probability, we will not output $\pi$ for which too much weight is placed outside the ``\emph{encoded part}'' of the distribution.

%Now consider the case when $D(\{\mathbf{U'}\}\cup S' \cup T'\}) \geq 5 \alpha$. Then we can say that \findpi will output {\sc Fail} with high probability.

\begin{lem}\label{lem:findpisumfourthtype}
For any distribution $D$ (regardless of whether $D$ is in $\cP_{\mbox{Gap}}$ or not), the probability that \findpi outputs a permutation $\pi$ for which $D(\{\mathbf{X}:\mathbf{X}_{\{i^*\} \cup B'}=\mathbf{0}\mathbf{1}^b\}) \leq 1-5\alpha$ is at most $1/10$.

%Consider any distribution $D$ over $\{0,1\}^N$ such that $D(\{\mathbf{U'}\}\cup S' \cup T'\}) \geq 5 \alpha$. Then with probability at most $1/10$, \findpi outputs a permutation $\pi$.
\end{lem}

\begin{proof}
Recall the set of vectors $\cY$ as defined in Step (vi) of \findpi: $\cY=\{\mathbf{Z} \in \cX': \mathbf{Z} \mid_{{{i^*} \cup B'}} \neq \mathbf{0}\mathbf{1}^b \}$, where $\cX'$ is the multi-set of (new) samples obtained in Step (vi) of \findpi. Consider a distribution $D$ such that $D(\{\mathbf{X}:\mathbf{X}_{\{i^*\} \cup B'}=\mathbf{0}\mathbf{1}^b\}) \leq 1-5\alpha$. This implies that $\E\left[\size{\cY}/\size{\cX'}\right] \geq 5 \alpha$. As $\size{\cX'} = \Oh(\log^2 N/\alpha)$, using the Chernoff bound, we obtain that with probability at least $9/10$, the algorithm \findpi outputs {\sc Fail} in Step (vi), and does not output any permutation $\pi$. This completes the proof.
\end{proof}

\subsection{The upper bound on adaptive testing for property $\cP_{\mbox{Gap}}$}\label{sec:quadratic_adaptive_ub}

In this subsection, we design the adaptive tester for the property $\cP_{\mbox{Gap}}$. Given a distribution $D$ over $\{0,1\}^N$, with high probability, \algadpt outputs {\sc Accept} when $D \in \cP_{\mbox{Gap}}$, and outputs {\sc Reject} when $D$ is far from $\cP_{\mbox{Gap}}$. The formal adaptive algorithm is presented in \algadpt (see Algorithm~\ref{algo:adaptive}). Note that it has only two adaptive steps.

%\comments{

In the first adaptive step, our tester \algadpt starts by calling the algorithm \findpi (as described in Subsection~\ref{sec:quadratic_determine_permutation}) whose  query complexity is $\tOh(n)$. If $D \in \cP_{\mbox{Gap}}$, with high probability, \findpi returns the permutation $\pi$ such that $D_{\pi} \in \cP_{\mbox{Gap}}^0$. Once $\pi$ is known, when we obtain a sample $\mathbf{X}$ from $D$, we can consider it as $\mathbf{X}_\pi$ from $D_{\pi}$. Also, from the structure of the vectors in the support of the distributions in $P^0_{\mbox{Gap}}$, we can decide whether $X_{\pi}$ is a special vector, that is, $X_{\pi} \in \{\mathbf{U}\} \cup \cS \cup \cT$ or $\mathbf{X}_\pi$ is an encoding vector, that is, $\mathbf{X}_\pi=\fen(\mathbf{z},\mathbf{x})$ for some $\mathbf{z}\in [n]^m$ and $\mathbf{x} \in \{0,1\}^n$. Observe that, in the later case, we can decode any bit of $\mathbf{x}$ (say $\mathbf{x}_j$) by finding $\mathbf{X}_\pi$ projected into $C_j$, which can be done by performing $\Oh(\log n)$ queries.

%} 

%\comments{
As the second adaptive step, our algorithm asks for a sequence $\cY$ of $\Oh(n/\eps)$ samples from $D$, that is, from $D_{\pi}$. Let $\cY'\subseteq \cY$ be the sequence of encoding vectors in $\cY$. We now call {\sc Supp-Est}$(\cY', \eps/3)$ (from Lemma~\ref{pre:suppest}), and depending on its output, \algadpt either reports {\sc Accept} or {\sc Reject}. Note that we can execute every query by {\sc Supp-Est}$(\cY', \eps/3)$, by performing $\Oh(\log n)$ queries to the corresponding sample in $\cY'$ \comments{as discussed towords the end of the above paragraph.}
%}  

\comments{
When $D \in \cP_{\mbox{Gap}}$ (that is, $D_\pi \in \cP_{\mbox{Gap}}^0$ for the permutation $\pi$), the set of encoding vectors in $D_\pi$ is the encoding of at most $n$ vectors in $\{0,1\}^n$. So, in that case, \algadpt reports {\sc Accept} with high probability. Now consider the case, when $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. If \algadpt has not rejected $D$ before calling {\sc Supp-Est}$(\cY', \eps/3)$, we will show that the distribution over $\{0,1\}^n$ induced by the vectors decoded from the encoding vectors in $D_{\pi}$ is ${\eps}/3$-far from having support size $n$. Then, \algadpt will reject $D$ with high probability.
}


\begin{algorithm}[H]\label{algo:adaptive}
%\scriptsize
\SetAlgoLined

\caption{\algadpt}
\label{alg:adaptive}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^N$, and a parameter $\eps \in (0,1)$.}
\KwOut{Either {\sc Accept} or {\sc Reject}.}
\LinesNumbered
\begin{description}
     \item[(i)] Call \findpi. If \findpi returns {\sc Fail}, {\sc Reject}. Otherwise, let $\pi$ be the permutation returned by \findpi. Denote for convenience $i^*=\pi^{-1}(1), B'=\pi^{-1}(B)$, and $C'_j=\pi^{-1}(C_j)$ for every $j \in [n]$.
     
     \item[(ii)] Take a multi-set $\cX$ of $\Oh(1/\eps)$ samples from $D$, and query all the entries of the sampled vectors of $\cX$ to know the vectors of $\cX$ completely. If there is any vector $\mathbf{X}$ for which $\mathbf{X} \mid_{\{i^*\} \cup B'} = \mathbf{0}\mathbf{1}^b$ (according to the permutation $\pi$ obtained from Step (i)) for which $\mathbf{X}_{\pi}$ is not in the image of $\mbox{{\sc FE}}$ (i.e. it is not a valid encoding of any vector in $\{0,1\}^n$), {\sc Reject}. Otherwise, proceed to the next step.
     
     %Construct a sequence of vectors $X' \subseteq X$ such that for every $\mathbf{X} \in X'$, $\mathbf{X} \mid_{\{i^*\}\cup B'} = \mathbf{0}\mathbf{1}^b$ (according to the permutation $\pi$ obtained from Step (i)). If the fraction $\frac{\size{X \setminus X'}}{\size{X}} > \frac{\eps}{10}$
     
     %For every $\mathbf{X} \in X$, query the indices $\{i^*\} \cup B'$ (according to the permutation $\pi$ obtained from Step (i)) to $\mathbf{X}$. 
     %For any $\mathbf{X} \in X$, if $\mathbf{X} \mid_{\{i^*\}\cup B'} = \mathbf{0}\mathbf{1}^b$, then choose a uniformly random $j \in [n]$, and check whether $\mathbf{X} \mid_{C'_j} \in \mathcal{E}(0)\cup\mathcal{E}(1)$, that is, whether it is a valid encoding of some value in $\{0,1\}$. If any invalid encoding is found for any $\mathbf{X} \mid_{C'_j}$, {\sc Reject}.

     %Construct the sequence of vectors $X'$ such that $X' = \{\mathbf{X} \in X: \mathbf{X} \mid_{\{i^*\} \cup B'} = \mathbf{0} \mathbf{1}^b\}$. Now sample a set of indices $\cI \subseteq [n]$ without replacement such that $\size{\cI}=\Oh(1/\eps)$. 
     
     %For every $\mathbf{X} \in X'$, choose a $j \in \cI$  randomly, and  check if $\mathbf{X} \mid_{C'_j}$ is a valid encoding of some vector $\mathbf{x} \in \{0,1\}^n$ with respect to the code ensemble $\cE$ by querying the appropriate indices of $\mathbf{X}$. If $\mathbf{X} \mid_{C'_j}$ is not a valid encoding for some $j \in \cI$, {\sc Reject}.
     
     %where $C_j$ denotes the set of indices of $[N]$ such that $C_j= \{b+2+k(j-1), \ldots, b+1+kj\}$.

    \item[(iii)]Take a sequence of samples $\cY$ such that $\size{\cY}=\Oh(n/\eps)$ from $D$. Now construct the sequence of vectors $\cY'$ such that $\cY'= \{\mathbf{Y} \in \cY: \mathbf{Y} \mid_{\{i^*\} \cup B'} = \mathbf{0} \mathbf{1}^b\}$ by querying the indices corresponding to $\{i^*\} \cup B'$.

    \item[(iv)] Call {\sc Supp-Est}$(\cY', \eps/3)$ (from Lemma~\ref{pre:suppest}), where a query to an index $j$ is simulated by querying the indices of $C'_j$ and decoding the obtained vector with respect to to $\mbox{{\sc SE}}$ (that is, checking whether the restriction of the queried vector to $C'_j$ is equal to $\mbox{{\sc SE}}(i,0)$ for some $i$, or equal to $\mbox{{\sc SE}}(i,1)$ for some i). {\sc Reject} if any of the following conditions hold:
    \begin{itemize}
        \item[(a)] $\size{\cY'}/\size{\cY} \leq 1/2$ (due to the absence of sufficiently many samples in $\cY'$ to apply {\sc Supp-Est}).

        \item[(b)] {\sc Supp-Est}$(\cY', \eps/3)$ queries an index $j$ from some $\comments{\mathbf{Y}_i}$ corresponding to an invalid encoding of $\comments{\mathbf{Y}_i} \mid_{C'_j}$ (that is, when $\comments{\mathbf{Y}_i} \mid_{C'_j}$ is not in the image of $\mbox{{\sc SE}}$).
        
        \item[(c)] {\sc Supp-Est}$(\cY',\eps/3)$ outputs {\sc Reject}.
    \end{itemize}

    Otherwise, {\sc Accept}.

\end{description}

\end{algorithm}

\vspace{10pt}

Let us first discuss the query complexity of \algadpt.

\begin{lem}[Query complexity of \algadpt]
The query complexity of the adaptive tester \algadpt for testing the property $\cP_{\mbox{Gap}}$ is $\tOh(N)= \tOh(n)$.    
\end{lem}

\begin{proof}
Note that \algadpt calls the algorithm \findpi in Step (i). Following the query complexity lemma of \findpi (Lemma~\ref{lem:queryfindpi}), we know that \findpi performs $\tOh(N)$ queries.

For every sample taken in Step (ii), the sampled vectors of the multi-set $\cX$ are queried completely. Since we take $\Oh(1/\eps)$ samples, this step requires $\Oh(N/\eps) = \widetilde{\Oh}(n/\eps)$ queries in total.  
    
%the indices of $\{i^*\}\cup B'$ are queried (taking $b+1=\Oh(\log \log kn/\eps)$ many queries), as well as possibly the indices of some $C'_j$ (taking $k=\Oh(\log n)$ many queries). Since we take $\Oh(1/\eps)$ many samples, this step requires $\Oh(\log n/\eps)$ many queries in total.

%In Step (ii), \algadpt first takes a multi-set of samples $X$ such that $\size{X}= \Oh(1/\eps)$ and then queries the indices of $\{i^*\} \cup B'$ of the vectors of $X$ to obtain $X'$. This procedure requires $\Oh(\log \log kn/ \eps)$ many queries. Also, in the same step, \algadpt tests whether the vectors of $X'$ are valid encodings with respect to the code ensemble $\cE$. This requires $\Oh(\log n/\eps^2)$ many queries.

Then in Step (iii), \algadpt takes a multi-set $\cY$ of $\Oh(n/\eps)$ samples, and queries for the indices in $\{i^*\} \cup B'$ to obtain the vectors in $\cY'$, which takes $\Oh(n \log \log kn/\eps)$ queries. Finally, in Step (iv), \algadpt calls the algorithm {\sc Supp-Est}, which performs $\tOh(n)$ queries (following Lemma~\ref{pre:suppest}), each of them simulated by $\Oh(\log n)$ queries to some $\comments{\mathbf{Y}_i} \mid_{{C'_j}}$. Thus, in total, \algadpt performs $\tOh(N) = \tOh(n)$ queries.
\end{proof}

Now we prove the correctness of \algadpt. We will start with the completeness proof.

\begin{lem}[Completeness]
Let $D$ be a distribution defined over $\{0,1\}^N$. If $D \in \cP_{\mbox{Gap}}$, then the algorithm \algadpt will output {\sc Accept} with probability at least $2/3$.
\end{lem}

\begin{proof}
Consider a distribution $D \in \cP_{\mbox{Gap}}$. From the completeness lemma of \findpi (Lemma~\ref{lem:findpicompleteness}), we infer that with probability at least $9/10$, \findpi returns the correct permutation $\pi$ in Step (i). Then, by the definition of $\cP_{\mbox{Gap}}$, the algorithm \algadpt can never encounter any samples with invalid encodings in Step (ii) which could cause it to {\sc Reject}. Thus, with probability at least $9/10$, the algorithm proceeds, with the correct permutation $\pi$, to Step (iii) and Step (iv).
    
%and no invalid encodings have been encountered. Thus \algadpt proceeds to Step (ii) with the same probability. Since $D \in \cP_{\mbox{Gap}}$, the total mass of the valid encoding vectors of $D$ is $1-3\alpha$. Thus, using the Chernoff bound, we can say that in Step (ii), the fraction of sampled vectors in $X$ that are not in $X'$ is at most $\eps/10$. So, \algadpt successfully completes this step and proceeds to Step (iii) and Step (iv).

As $D \in \cP_{\mbox{Gap}}$, $D(\{\mathbf{U'}\} \cup \cS' \cup \cT') = 3 \alpha$. As $\size{\cY}= \Oh(n/\eps)$, using the Chernoff bound, we can say that, with probability at least $9/10$, $\size{\cY'}/\size{\cY} \geq 1/2$. Moreover, as the vectors in $\cY'$ are valid encodings with respect to the function $\mbox{{\sc FE}}$ of at most $n$ vectors from $[2n]$, following the support estimation upper bound lemma (Lemma~\ref{pre:suppest}), we obtain that {\sc Supp-Est} outputs {\sc Accept} with probability at least $9/10$. Combining these, we conclude that \algadpt outputs {\sc Accept} with probability at least $2/3$.
\end{proof}

Now we prove that when $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, \algadpt will output {\sc Reject} with probability at least $2/3$.

\begin{lem}[Soundness]\label{lem:sound}
    Let $\eps \in (0,1)$ be a proximity parameter. Assume that $D$ is a distribution defined over $\{0,1\}^N$ such that $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. Then \algadpt outputs {\sc Reject} with probability at least $2/3$.
\end{lem}

%From the description of \algadpt (Algorithm~\ref{algo:adaptive}), if the tester reports {\sc Reject} before executing all the steps of {{\sc Supp-Est}}$(\cY',\eps/3)$ in Step (iv),  then we are done. So, assume that \algadpt executes all the steps of {{\sc Supp-Est}}$(\cY',\eps/3)$. Let $\cY'$ be the set of samples from distribution $D^*$ over $\{0,1\}^n$. Note that $D^*$ is unknown and we are accessing $D^*$ indirectly via decoding sample from $D$ over $\{0,1\}^n$. From the correctness {{\sc Supp-Est}}$(\cY',\eps/3)$, we will be done with the proof of Lemma~\ref{lem:sound}.
\comments{We prove the above lemma by a series of claims.}
%\begin{proof}
Let $D$ be a distribution which is $\eps$-far from $\cP_{\mbox{Gap}}$, and $\mathcal{V}$ denote the set $\{\mathbf{X} \in \mbox{Supp}(D) : \mathbf{X} \mid_{\{i^*\}\cup B'}=\mathbf{0}\mathbf{1}^b\}$, and let us define $\mathcal{U}= \mbox{Supp}(D) \setminus \mathcal{V}$. Let us start with the following observation.

%If \algadpt outputs {\sc Reject} in either Step (i) or Step (ii), then we are done. Otherwise, let us assume that \algadpt has proceeded to Step (iii) and Step (iv). Now we need to argue that when we call the algorithm {\sc Supp-Est}, it will output {\sc Reject} with probability at least $9/10$.

\begin{obs}\label{obs:sumdothervec}
$D(\mathcal{U}) \leq 5\alpha$, unless the algorithm \algadpt has rejected with probability at least $1-1/N^3$ in Step (i).
%$D(\{\mathbf{U'}\}\cup S' \cup T') \leq 5\alpha$ with probability at least $1- \frac{1}{N^3}$.
\end{obs}

\begin{proof}
Since \algadpt in Step (i) invokes the algorithm \findpi, this follows immediately from Lemma~\ref{lem:findpisumfourthtype}.
%Since \findpi has not output {\sc Fail} for the input distribution $D$ in Step $(vi)$, this implies that the fraction of vectors in $Y'$ that belong to the set $\{\mathbf{U'}\} \cup S' \cup T'$ is at most $4 \alpha$. Since $\size{Y} = \Oh(n/\eps)$, using the Chernoff bound, we can say that with probability at least $1- \frac{1}{N^3}$, $D(\{\mathbf{U'}\} \cup S' \cup T') \leq 5 \alpha$.
\end{proof}

% Thus with probability at least $1- \frac{1}{N^3}$, we can say that: 
% \begin{itemize}

%     \item[(i)] There exists a vector $\mathbf{U}' \in \{0,1\}^N$ that has $0$ at some index $i^*$ and $0$ in all other indices. 
    
%     %Also, $D(\mathbf{U})= \alpha$.
    
%     \item[(ii)] There exists a set of vectors $S'=\{\mathbf{V'}_1, \ldots, \mathbf{V'}_b\}$ in $\{0,1\}^N$ such that for every $\mathbf{V'}_i \in S$, $\mathbf{V'}_i$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B'$ and $0$ in all other indices. 
    
%     %Moreover, $D(\mathbf{V_i}) = \alpha/\size{B}$ for every $i \in [\size{B}]$.

%     \item[(iii)] There exists a set of vectors $T'= \{\mathbf{W_0}, \ldots, \mathbf{W}_{\lceil \log kn \rceil -1}\}$ (disjoint from $S'$) in $\{0,1\}^N$ such that each vector in $T'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. For every $j$, denote by $\mathbf{W}'_j$ the vector in $T'$ for which $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$.

%     %for each $\mathbf{W}_i \in T'$, $\mathbf{W}_i$ is of the form $\mathbf{0}(b(i))(\mathbf{0}^{2^i}\mathbf{1}^{2^i})^{kn/2^{i+1}}$, where $b(i)$ denotes the binary representation of $i$.
%     %for each $\mathbf{W_i} \in T$, $\mathbf{W_i}$ has $0$ at the index $i^*$ and the decimal evaluation of $\mathbf{W_i}$ is $i$ when projected to the indices in $B$. Let $N' = [N]\setminus B\cup \{i^*\}$ and $\mathbf{W}_i'=\mathbf{W}_i \mid_{N'}$ for every $i \in [\log n]$ such that for every $j \in N'$, the $j$-th bit of $\mathbf{W}'_i$ is $1$ if and only if $j$ divided by $2^i$ produces an odd number. 
    
%     %Moreover, $D(\mathbf{W_i}) = \alpha/\log n$ for every $i \in [\log n]$.
%     \item[(iv)] $D(\{\mathbf{U}'\}\cup S' \cup T') \leq 5\alpha$.
    
%     \item[(v)] Let $\pi$ be the permutation obtained from \findpi. Let $\mathcal{V}$ be the set of vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$. For each vector $\mathbf{V} \in \mathcal{V}$, consider a set of $\Gamma_{\mathbf{V}}=\{\mathbf{v_1,\ldots,\mathbf{v}_{n}}\}$ of $n$ vectors in $\{0,1\}^{n}$, such that
%     the $j$-th index of $\mathbf{v}_i$ has the same value present in the $\{\pi((i-1)\lceil \log kn \rceil +j)$-th index of $\mathbf{V}$. Let $\Gamma'_{\mathbf{V}} \subseteq \Gamma_{\mathbf{V}}$ be the set of vectors that are not valid encoding with respect to $\cE$. Let $\Gamma=\bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$.
    
%     %Then $\sum_{\mathbf{V}\in \mathcal{V}} D(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \alpha$.
    
    
%    % $\mathbf{V}$ is not an encoding with respect to $\cE$. Then $D(\mathcal{V})\leq \alpha$.
%     %and the remaining set of indices are code ensemble of vectors in $\{0,1\}^{n/\log n}$.
    
% \end{itemize}

%Let $\mathcal{V}$ be the set of vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$. For each vector $\mathbf{V} \in \mathcal{V}$, consider a set of $\Gamma_{\mathbf{V}}=\{\mathbf{v_1,\ldots,\mathbf{v}_{n}}\}$ of $n$ vectors in $\{0,1\}^{n}$, such that the $j$-th index of $\mathbf{v}_i$ has the same value present in the $\{\pi((i-1)\lceil \log kn \rceil +j)$-th index of $\mathbf{V}$, where $\pi$ is the permutation returned by \findpi. Let $\Gamma'_{\mathbf{V}} \subseteq \Gamma_{\mathbf{V}}$ be the set of vectors that are not valid encodings with respect to $\cE$. Let $\Gamma=\bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$ be the set of all such vectors. 


Let $\mathcal{V}^{\mbox{inv}} \subseteq \mathcal{V}$ denote the following set of vectors:
$$\mathcal{V}^{\mbox{inv}} = \{\mathbf{X} \in \mathcal{V}: \mathbf{X} \neq \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \ \mbox{for all} \ \mathbf{z} \in [n]^m, \mathbf{x} \in \{0,1\}^n\}$$

For every vector $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$, let $\Gamma'_{\mathbf{V}}=\{j\in [n]: \mathbf{V}\mid_{C'_j} \ \mbox{is not in the image of} \ \mbox{{\sc SE}}\}$ denotes \comments{the set of indices in $[n]$ of chunks of all the ``\emph{locally invalid}'' encodings} in the vector $\mathbf{V}$~\footnote{Note that it may be the case that $\Gamma'_{\mathbf{V}}=\emptyset$, for example when for every $j \in [n]$, we have $\mathbf{V} \mid_{C'_j} = \mbox{{\sc SE}}(i_j, \mathbf{x}_j)$, for some $i_1, \ldots, i_n$ and $\mathbf{x}_1, \ldots, \mathbf{x}_n$ for which $i_1, \ldots, i_n$ are not in the image of $\mbox{{\sc GE}}$.}.

%Now we have the following lemma.

% \begin{lem}\label{lem:sumencvector}
%     $\sum_{\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}} D(\mathbf{V})\frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \eps/10$, unless \algadpt has rejected with probability at least $2/3$ in Step (ii).
% \end{lem}

% \begin{proof}
% For every $\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}$, the probability that a sample $\mathbf{X}$ taken in Step (ii) is equal to $\mathbf{V}$ is $D(\mathbf{V})$, and then the probability that $\mathbf{V} \mid_{C'_j}$ is an invalid encoding is exactly $|\Gamma'_{\mathbf{V}}|/n$. This implies that for every sample $\mathbf{X} \in X$, the probability that it causes a rejection is exactly $\sum_{\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}}D(\mathbf{V})|\Gamma'_{\mathbf{V}}|/n$.  The lemma follows since we have taken $\Oh(1/\eps)$ many independent samples in Step (ii).

% %Recall that during the execution of the tester \algadpt in Step (ii), \algadpt selects a subset of indices $\cI \subseteq [n]$, and for every $\mathbf{V} \in X'$, chooses an index $j \in \cI$ randomly and checks whether $\mathbf{V} \mid_{C'_j}$ is a valid encoding with respect to $\cE$ or not. As $\Gamma'_{\mathbf{V}}$ is the set of vectors that are not valid encodings of any vector $\mathbf{V}$, the probability that \algadpt \ {\sc Rejects} a fixed vector $\mathbf{V}$ is $\frac{\size{\Gamma'_{\mathbf{V}}}}{n}$. As $\size{\cI} = \Oh(1/\eps)$, applying the Chernoff bound and summing over all vectors $\mathbf{V} \in \mathcal{V}$, we have the result.
% \end{proof}

For any distribution $D$ that has not been rejected by \algadpt in Step (i) and Step (ii), let us define another distribution $D_1$ over $\{0,1\}^N$ such that $D_1(\mathbf{U}') = \alpha$, $D_1(\mathbf{X}) = \frac{\alpha}{b}$ for every $\mathbf{X} \in \cS'$, $D_1(\mathbf{X}) = \frac{\alpha}{\lceil \log kn \rceil}$ for every $\mathbf{X} \in \cT'$, and $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$. Then we have the following lemma.

\begin{lem}\label{obs:massnonenc}
$D_1(\mathcal{V}^{\mbox{inv}}) \leq \eps/8$.
\end{lem}

%$\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}} D_1(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \frac{\eps}{8}$.

\begin{proof}
We first note that unless $D(\mathcal{V}^{\mbox{inv}}) \leq \eps/10$, Step (ii) of \algadpt would have rejected with probability at least $2/3$. Additionally, from Observation~\ref{obs:sumdothervec}, we know that $D(\{\mathbf{U}'\} \cup \cS' \cup \cT') \leq 5 \alpha$. As $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$, and $\mathcal{V}^{\mbox{inv}} \subseteq \mathcal{V}$, we can say that for every $\mathbf{X} \in \mathcal{V}^{\mbox{inv}}$, $D_1(\mathbf{X}) \leq (1- 3 \alpha)D(\mathbf{X})/(1-5 \alpha)$. Since $\alpha = 1/\log n$, we obtain the result for sufficiently large $n$.
\end{proof}

%From Observation~\ref{obs:sumdothervec}, we know that $D(\{\mathbf{U}'\} \cup S' \cup T') \leq 5 \alpha$. As $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$, and $\mathcal{V}^{\mbox{invalid}} \subseteq \mathcal{V}$, we can say that for every $\mathbf{X} \in \mathcal{V}^{\mbox{invalid}}$, $D_1(\mathbf{X}) \leq \frac{1- 3 \alpha}{1 - 5 \alpha} D(\mathbf{X})$. Since $\alpha=1/\log n$, from Lemma~\ref{lem:sumencvector}, we know that $\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}} D(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \frac{\eps}{10}$, for sufficiently large $n$, we have the result.


Now we show that the Earth Mover Distance between the distributions $D$ and $D_1$ is not large.

\begin{lem}\label{lem:dd1emd}
The Earth Mover Distance between $D$ and $D_1$ is at most $6\alpha$.
\end{lem}

\begin{proof}
We will bound the Earth Mover Distance between $D$ and $D_1$ in terms of the variation distance between them as follows:
\begin{eqnarray}
    EMD(D,D_1) &\leq& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N}|D(\mathbf{X}) - D_1(\mathbf{X})| \nonumber \\ &=& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})| + \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})| \label{eqn:emddd1}
\end{eqnarray}

\color{blue}

Let us bound the first term as follows:
\begin{eqnarray*}
    \sum_{\mathbf{X} \in \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})|
    &=& \sum_{\mathbf{X} \in \mathcal{V}}| (1- 3 \alpha) \frac{D(\mathbf{X})}{D(\mathcal{V})} - D(\mathbf{X})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D(\mathbf{X})}{D(\mathcal{V})} |(1- 3 \alpha) - D(\mathcal{V})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D(\mathbf{X})}{D(\mathcal{V})} |3 \alpha - (1- D(\mathcal{V}))| \\ &\leq & \sum_{\mathbf{X} \in \mathcal{V}} 3 \alpha \frac{D(\mathbf{X})}{D(\mathcal{V})} \leq 3 \alpha ~~~(\because D(\mathcal{V})=1-D(\mathcal{U})\geq 1- 5 \alpha)
\end{eqnarray*}

\color{black}

As $D(\mathcal{U}) \leq 5 \alpha$, and $D_1(\mathcal{U}) \leq 3 \alpha$, we have
    $\sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})| \leq 8 \alpha$.
Following Equation~\ref{eqn:emddd1}, we conclude that $EMD(D,D_1) \leq 6 \alpha$, which completes the proof.
\end{proof}
% Recall that the  EMD between $D$ and $D_1$ is the solution to the following LP:
% \begin{eqnarray*}
%     &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
%     &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D(\mathbf{X})~\forall \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
%     \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_1(\mathbf{Y})~\forall \mathbf{Y} \in \{0,1\}^N.
% \end{eqnarray*}
% % Now consider the following two cases:
% % \begin{itemize}
% %     \item[(a)] $\sum_{\mathbf{Y} \notin \{\mathbf{U}\} \cup S \cup T} D(\mathbf{Y}) \geq 1-3 \alpha$: 
% % \end{itemize}
% % In this case $D_1(\mathbf{Y})\geq D(\mathbf{Y})$ for every $\mathbf{Y} \notin \{\mathbf{U}\} \cup S \cup T$.
% Consider the flow $f^*$ such that
% $f^*_{\mathbf{XX}}=D(\mathbf{X})$ for every $\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'$.

% \begin{obs}
% $\sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{\mathbf{XX}} \geq 1-5 \alpha$.
% \end{obs}

% \begin{proof}
% \begin{eqnarray*}
% \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{\mathbf{XX}}&=&\sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} \min \{D(\mathbf{X}),D_1(\mathbf{X})\} \\ &=&
% \min \left \lbrace \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} D(\mathbf{X}), \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} D_1(\mathbf{X}) \right \rbrace \\
% &\geq& \min \{1-5\alpha,1-3\alpha\}=1-5\alpha.
% \end{eqnarray*}
% %&=& \sum_{\mathbf{X} \notin \{\mathbf{U}\} \cup S \cup T} D(\mathbf{X}) \min\{1, \frac{(1 - 3 \alpha)}{1- \sum_{\mathbf{Y} \in S \cup T \cup \{\mathbf{U}\}}D(\mathbf{Y})}\}\\
% \end{proof}
% Thus the EMD between $D$ and $D_1$ can be expressed as follows:
% \begin{eqnarray*}
% \mbox{EMD}(D,D_1) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^*_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
% &\leq& \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{{\bf X X}}d_H({\bf X},{\bf X}) +\left( 1-\sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{\mathbf{XX}}\right)\\
% &\leq& 0 + 5 \alpha=5\alpha
% \end{eqnarray*}
% This completes the proof of the lemma.


Let us define a distribution $D_2$ over $\{0,1\}^N$ using the following procedure:
\begin{itemize}
    %\item $D_2(\mathbf{U}')=\alpha$;
    %\item There exists a set of vectors $S'=\{\mathbf{V'}_1, \ldots, \mathbf{V'}_b\}$ in $\{0,1\}^N$ such that for every $\mathbf{V'}_i \in S$, $\mathbf{V'}_i$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B'$ and $0$ in all other indices. Moreover, $D_2(\mathbf{V'}_i) = \alpha/b$ for every $i \in [\size{B}]$.
    
    %There exists a set of vectors $S= \{\mathbf{V_1}, \ldots, \mathbf{V_{\size{B}}}\}$ in $\{0,1\}^N$ such that for every $\mathbf{V_i} \in S$, $\mathbf{V_i}$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B$ and $0$ in all other indices. 
    
    %\item There exists a set of vectors $T'= \{\mathbf{W}_0, \ldots, \mathbf{W}_{\lceil \log kn \rceil -1}\}$ (disjoint from $S'$) in $\{0,1\}^N$ such that every vector in $T'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. For every $j \in \{0\} \cup [\lceil \log kn \rceil -1]$, $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$. Moreover, $D_2(\mathbf{W}_i) = \alpha/\lceil \log kn \rceil$ for every $i \in [\size{T'}]$.
    
    %There exists a set of vectors $T= \{\mathbf{W_1}, \ldots, \mathbf{W_{\log n}}\}$ (disjoint from $S$) in $\{0,1\}^N$ such that for each $\mathbf{W_i} \in T$, $\mathbf{W_i}$ has $0$ at the index $i^*$ and the decimal evaluation of $\mathbf{W_i}$ is $i$ when projected to the indices in $B$. Let $N' = [N]\setminus B\cup \{i^*\}$ and $\mathbf{W}_i'=\mathbf{W}_i \mid_{N'}$ for every $i \in [\log n]$ such that for every $j \in N'$, the $j$-th bit of $\mathbf{W}'_i$ is $1$ if and only if $j$ divided by $2^i$ produces an odd number. 
    
     %Consider the set of vectors $\mathcal{V}$  that contains vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$, and let us define the set $\Gamma = \bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$. 

     \item Set $D_2(\mathbf{X})= D_1(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U}$. 
    
    \item Recall that $\Gamma'_{\mathbf{V}}=\{j\in [n]: \mathbf{V}\mid_{C'_j} \ \mbox{is not in the image of} \ \mbox{{\sc SE}}\}$ for every vector $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$. For every vector $\mathbf{V}\in \mathcal{V}^{\mbox{inv}}$, we perform the following steps:

    \begin{itemize}
        \item[(a)] For every $j \notin \Gamma'_{\mathbf{V}}$, decode the vector $\mathbf{V} \mid_{C'_j}$ using $\mbox{{\sc SE}}$ to obtain $\mathbf{x}_j \in \{0,1\}$.

        \item[(b)] For every $j \in \Gamma'_{\mathbf{V}}$, choose an arbitrary value $\mathbf{x}_j$ from $\{0,1\}$.

        \item[(c)] Using $\mathbf{x} = (\mathbf{x}_1, \ldots, \mathbf{x}_n)$ obtained from (a) and (b), construct a new vector $\mathbf{V}'$ for which $\mathbf{V}'_{\pi}=\mbox{{\sc FE}}(\mathbf{z},\mathbf{x})$ for an arbitrary $\mathbf{z} \in [n]^m$, where $\pi$ is the permutation obtained from \findpi in Step (i) of \algadpt.
    \end{itemize}    

    \item For every vector $\mathbf{V} \in \mathcal{V} \setminus \mathcal{V}^{\mbox{inv}}$, set $\mathbf{V}' = \mathbf{V}$.

    \item Finally define $D_2(\mathbf{W})=\sum_{\mathbf{V}: \mathbf{V'} =\mathbf{W}} D_1(\mathbf{V})$ for every $\mathbf{W} \in \mathcal{V}$.

\end{itemize}
  


    %For every $\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}$ and $j \in \Gamma'_{\mathbf{V}}$, replace $\mathbf{V} \mid_{C'_j}$ with an arbitrary valid encoding, that is, an element of $\mathcal{E}(0) \cup \mathcal{E}(1)$.  For every vector $\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}$, let $\mathbf{V}'$ be the vector that we obtain after the above replacement. Now define $D_2(\mathbf{W})=\sum_{\mathbf{V}: \mathbf{V'} =\mathbf{W}} D_1(\mathbf{V})$ for every $\mathbf{W} \in \mathcal{V}^{\mbox{invalid}}$.

    
    %and $\mathbf{v} \in \Gamma'_{\mathbf{v}}$, replace $\mathbf{v}$ with another vector $\mathbf{v}' \in \{0,1\}^{n}$ that is a valid encoding of either $0$ or $1$ (arbitrarily chosen) with respect to the code ensemble $\cE$.  
    %$D_2(\mathbf{V}')=D_1(\mathbf{V})$ for every $\mathbf{V} \in \mathcal{V}$.


Now we prove that the distributions $D_1$ and $D_2$ are not far in Earth Mover Distance.

\begin{lem}\label{lem:d1d2emd}
The Earth Mover Distance between $D_1$ and $D_2$ is at most $\eps/8$.
\end{lem}

\begin{proof}
Recall that the EMD between $D_1$ and $D_2$ is the solution to the following LP:
\begin{eqnarray*}
    &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
    &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_1(\mathbf{X})~\forall \ \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
    \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_2(\mathbf{Y})~\forall \ \mathbf{Y} \in \{0,1\}^N.
\end{eqnarray*}

Consider the flow $f^*$ such that $f^*_{\mathbf{XX}}=D_1(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U} \cup (\mathcal{V} \setminus \mathcal{V}^{\mbox{inv}})$, $f^*_{\mathbf{VV'}}=D_1(\mathbf{V})$ for every $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$, and $f^*_{\mathbf{X}\mathbf{Y}}=0$ for all other vectors. Then we have the following:
\begin{eqnarray*}
\mbox{EMD}(D_1,D_2) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^*_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
&\leq& \sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}^{\mbox{inv}}} f^*_{{\bf X X}}d_H({\bf X},{\bf X}) + \sum_{{\bf V} \in \mathcal{V}^{\mbox{inv}}} f^*_{{\bf V} {\bf V}'}d_H({\bf V},{\bf V'})\\
&\leq& 0 + \sum_{\mathbf{V}\in \mathcal{V}^{\mbox{inv}}}D_1(\mathbf{V})d_H({\bf V},{\bf V'}) 
\end{eqnarray*}

To bound the second term of the last expression, note that $\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{inv}}}D_1(\mathbf{V})d_H({\bf V},{\bf V'}) \leq D_1(\mathcal{V}^{\mbox{inv}}) \leq \eps/8$. This follows from Lemma~\ref{obs:massnonenc}. Thus, we conclude that $EMD(D_1,D_2) \leq \eps/8$, completing the proof of the lemma.
\end{proof}

%$D_1({\bf x})=0$ for each ${\bf x} \in \{\mathbf{U}\} \cup S \cup T$, and $D_1({\bf x})=\frac{D(\bf x)}{1-\sum_{{\bf y} \in \{\mathbf{U}\} \cup S \cup T}D({\bf y})}$ for each ${\bf x} \notin \{\mathbf{U}\} \cup S \cup T$. Note that the Earth Mover distance between $D$ and $D_1$ is at most $3 \alpha$. Since $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, using the triangle inequality, we can say that $D_1$ is $\frac{9\eps}{10}$-far from $\cP_{\mbox{Gap}}$.


%Now construct a distribution $D_1'$ over $\{0,1\}^n$ by projecting the support vectors of $D_1$ onto the set of indices $N' = [N] \setminus B \cup \{i^*\}$. Note that we can assume that we are decoding samples the {\sc Supp-Est} algorithm $\cA$.

Now we have the following observation regarding the rejection probabilities of \algadpt for the distributions $D_1$ and $D_2$.

\begin{obs}
The probability that the tester \algadpt outputs {\sc Reject} in Step (iv) when the input distribution is $D_1$ is at least as large as the probability that \algadpt outputs {\sc Reject} in Step (iv) when the input distribution is $D_2$.
%Let $Q$ be the set of indices queried by the algorithm {\sc Alg-Adaptive} in Step (iv). Then {\sc Alg-Adaptive} is oblivious to $D_1$ and $D_2$ with respect to $Q$.
\end{obs}

\begin{proof}
Note that in the distribution $D_1$, there can be some vectors in $\mbox{Supp}(D_1)$ that are not valid encodings with respect to the function $\mbox{{\sc FE}}$. Thus during execution, the tester \algadpt can {\sc Reject} $D_1$ by Condition (ii) and Condition (iv) (b). However, by the construction of $D_2$ from $D_1$, we have replaced the invalid encoding vectors with valid encoding vectors. Thus, the only difference it makes here is that \algadpt may eventually accept a sample from $D_2$ when encountering such a place where a sample from $D_1$ would have been immediately rejected by Condition (ii) or Condition (iv) (b). Other than this difference, the distributions $D_1$ and $D_2$ are identical. So, the probability that \algadpt outputs {\sc Reject} $D_1$ is at least as large as the probability that it {\sc Rejects} $D_2$.
\end{proof}

%Consider the case when the input distribution is $D_1$ to \algadpt. Note that \algadpt can {\sc Reject} $D_1$ immediately in Step (ii), which is not the case when $D_2$ is the input distribution to \algadpt.

%First note that the structure of the set of vectors $\{\mathbf{U}\} \cup S \cup T$ is identical for both the distributions $D_1$ and $D_2$. Thus, the algorithm {\sc Alg-Adaptive} can not distinguish between $D_1$ and $D_2$ in Phase $1$.

%Consider the case when  \algadpt proceeds to Step (iv). This implies that, \algadpt has not output {\sc Reject} for the input distribution till now. Assume that {\sc Supp-Est} queries for the set of indices $Q$ in Step (iv). 

%Consider a fixed set of random bits $\mathcal{R}$ to be used by \algadpt. Now let us take a distribution $D^{R}$ which is either $D_1$ or $D_2$ with equal probability. Since we have replaced every vector in $\mathcal{V}$ with a corresponding correct encoding while constructing $D_2$, the output of \algadpt with $\mathcal{R}$ as the random bits used during its execution will remain invariant whether $D^R = D_1$ or $D^R = D_2$.
%For a fixed set of random bits used by {\sc Alg-Adaptive}, if the input distribution is either $D_1$ or $D_2$, {\sc Alg-Adaptive} will output the same answer for both of them.


%For every vector $\mathbf{x}\in \{0,1\}^{n}$ and $\mathbf{z} \in [n]^m$, let $\mbox{{\sc FE}}(\mathbf{z}, \mathbf{x}) \subset \{0,1\}^N$ be the set of vectors that are valid encodings with respect to $\mbox{{\sc FE}},i^*,B'$ and $\pi$. 

Let us now define a distribution $D_2^{dec}$ over $\{0,1\}^{n}$ as follows:
\begin{equation}\label{def:enc-dist}
    D_2^{dec}(\mathbf{x})=\frac{1}{1-3\alpha}\sum_{\substack{\mathbf{Y}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}} D_2(\mathbf{Y}) = \frac{1}{1-3\alpha}\sum_{\mathbf{z}\in [n]^m}D_2(\mathrm{FE}(\mathbf{z},\mathbf{x})_{\pi^{-1}}).
\end{equation}


\begin{lem}
The distribution $D_2^{dec}$ is $\eps/3$-far from having support size at most $n$.
\end{lem}

\begin{proof}
Recall that the input distribution $D$ is $\eps$-far from the property $\cP_{\mbox{Gap}}$. Then, by Lemma~\ref{lem:dd1emd}, we know that $d_{EM}(D,D_1) \leq 6 \alpha$. Thus, the distribution $D_1$ is $(\eps - 6 \alpha)$-far from $\cP_{\mbox{Gap}}$.

By Lemma~\ref{lem:d1d2emd}, we know that $d_{EM}(D_1,D_2) \leq \eps/8$. This implies that the distribution $D_2$ is $(\eps - 6\alpha - \eps/8) \geq 2\eps/3$-far from $\cP_{\mbox{Gap}}$. Now we will prove that $D_2^{dec}$ is $\eps/3$-far from having support size at most $n$.

\textcolor{red}{Let us prove this by contradiction. Assume that $D_2^{dec}$ is $\eps/3$-close to having support size at most $n$. Let $D_{3}$ be a distribution over $\{0,1\}^{n}$ having support size at most $n$ such that the Earth Mover Distance between $D_3$ and $D_2^{dec}$ is at most $\eps/3$.
Given the distribution $D_{3}$ over $\{0,1\}^{n}$, and the flow $f'_{\mathbf{x}\mathbf{y}}$ from $D_3$ to $D_2^{dec}$ realizing this distance, let us consider the distribution $D_3^{enc}$ over $\{0,1\}^N$ such that for any $\mathbf{X} \in \mathcal{V}$, for which $\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x})$ for some $\mathbf{z} \in [n]^m$, we have $D_3^{enc}(\mathbf{X})=\sum\limits_{\mathbf{y} \in \{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}$, and for every $\mathbf{X} \in \mathcal{U}$, $D_3^{enc}(\mathbf{X}) = D_2(\mathbf{X})$.}

%$D_3^{enc}(\mathbf{X})=D_3(\mathbf{x}) \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}$

%Given the distribution $D_{3}$ over $\{0,1\}^{n}$, let us consider the distribution $D_3^{enc}$ over $\{0,1\}^N$ such that for every $\mathbf{x} \in \{0,1\}^{n}$, $D_3^{enc}(\mathbf{X})=  (1 - 3 \alpha) D_{3}(\mathbf{x})$ with $\mathbf{X} = \cE(\mathbf{x})$, and $D_3^{enc}(\mathbf{X})= D_2(\mathbf{X})$ for every $\mathbf{X} \in \{\mathbf{U}'\} \cup S' \cup T'$.

%obtained by encoding the support vectors of $D_{*}$ using $\cE$ , as well as including the vectors in the set $\{\mathbf{U}\} \cup S \cup T$ from the support of the distribution $D_2$.

\begin{cl}\label{cl:emd-far}
Let $D_3^{enc}$ be the distribution over $\{0,1\}^N$ obtained from $D_3$. Then the EMD between $D_{3}^{enc}$ and $D_2$ is at most $\eps/3$.
\end{cl}

\begin{proof}

\color{blue}

Recall that the EMD between $D_3^{enc}$ and $D_2$ is the solution to the following LP:
\begin{eqnarray*}
    &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
    &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_3^{enc}(\mathbf{X})~\forall \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
    \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_2(\mathbf{Y})~\forall \mathbf{Y} \in \{0,1\}^N.
\end{eqnarray*}

Let $f'_{\mathbf{x} \mathbf{y}}$ be the flow realizing the EMD between $D_3$ and $D_2^{dec}$. Using $f'$, we now construct a new flow $f^\star$ between $D_3^{enc}$ and $D_2$ as follows:

\begin{itemize}
    \item[(1)]  For vectors $\mathbf{X}, \mathbf{Y} \in \mathcal{U}$,
    
\begin{itemize}
    \item[(i)] If $\mathbf{X} \neq \mathbf{Y}$, then set $f^\star_{\mathbf{X} \mathbf{Y}}=0$. 

    \item[(ii)] If $\mathbf{X} = \mathbf{Y}$, then set $f^\star_{\mathbf{X} \mathbf{Y}} = D_3^{enc}(\mathbf{X})=D_2(\mathbf{Y})$.
    \end{itemize}
    
    \item[(2)] For two vectors $\mathbf{X}, \mathbf{Y} \in \mathcal{V}$, we take the vectors $\mathbf{x}, \mathbf{y} \in \{0,1\}^n$ such that $\mathbf{X}, \mathbf{Y} \in \{0,1\}^N$ are their
valid encodings (by construction such vectors $\mathbf{x}, \mathbf{y}$ exist), and vectors $\mathbf{z}_1,\mathbf{z}_2$ such that $\mathbf{X}=\fen(\mathbf{z}_1,\mathbf{x})$ and $\mathbf{Y}=\fen(\mathbf{z}_2, \mathbf{y})$. Now we set the flow as follows:
\begin{itemize}
    \item[(i)] If $\mathbf{z}_1 \neq \mathbf{z}_2$, then set $f^\star_{\mathbf{X} \mathbf{Y}} = 0$.

    \item[(ii)] If $\mathbf{z}_1 = \mathbf{z}_2$, then set $f^\star_{\mathbf{X} \mathbf{Y}} =  f'_{\mathbf{x} \mathbf{y}} \cdot \frac{D_2(\mathbf{Y})}{D_2^{dec}(\mathbf{y})}$.
\end{itemize}

\item[(3)] If one of $\mathbf{X}$ and $\mathbf{Y}$ is in $\mathcal{U}$ and the other one is in $\mathcal{V}$, then $f^\star_{\mathbf{X}\mathbf{Y}}=0$.

\end{itemize}


We first argue that the flow $f^*_{\mathbf{X} \mathbf{Y}}$ constructed as above is indeed a valid flow, that is, we have:
$(i) \sum\limits_{\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}} = D_3^{enc}(\mathbf{X})$, and $(ii) \sum\limits_{\mathbf{X} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}} = D_2(\mathbf{Y})$. 

%We prove the first one and omit the other similar proof.

To prove $\sum\limits_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X} \mathbf{Y}} = D_3^{enc}(\mathbf{X})$, first observe that it holds when $\mathbf{X} \in \mathcal{U}$ from (1) and (3) in the description of $f^{\star}_{\mathbf{X} \mathbf{Y}}$. Now consider when $\mathbf{X} \in \mathcal{V}$. Assume $\mathbf{X}_{\pi}=\fen\left(\mathbf{z},\mathbf{x}\right)$, where $\mathbf{z} \in [n]^m$ and $\mathbf{x} \in \{0,1\}^n$. So, from (2) in the description of $f^\star_{\mathbf{X}\mathbf{Y}}$, we have
$$\sum\limits_{\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}}=\sum\limits_{\mathbf{y} \in \{0,1\}^n} f^\star_{\mathbf{X} \mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}}} = \sum_{\mathbf{y}\in\{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}=
D_3^{enc}(\mathbf{X}).$$

%\sum\limits_{\mathbf{y} \in \{0,1\}^n}f'_{\mathbf{x} \mathbf{y}} \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}=D_3(\mathbf{x})\cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}= 

%\remove{For example, for $Y \in \mathcal{U}$ it is (by the construction above) quite clear that $\sum_X f_{XY} = f_{YY} = D_2(Y)$, and for $Y=FE(z,y)$ for some $z,y$ (which is the only other non-zero option) we have $\sum_X f_{XY} = \sum_{z',x} f_{FE(z',x),Y} = \sum_x f_{FE(z,x),Y}= \sum_x f'_{xy} \cdot \frac{D_2(Y)}{D_2^{dec}(y)} = D_2(Y)$.}

For (ii), consider $\mathbf{Y}_{\pi} = \mathrm{FE}(\mathbf{z}, \mathbf{y})$ for some $\mathbf{z} \in [n]^m$. Then we have the following:
$$\sum_{\mathbf{X}\in\{0,1\}^N}f_{\mathbf{X}\mathbf{Y}}^{\star}=\sum_{\mathbf{x}\in\{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}=D_2^{dec}(\mathbf{y})\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}=D_2(\mathbf{Y}).$$

In the above, we have used the fact that $f'_{\mathbf{x} \mathbf{y}}$ is a valid flow from $D_3$ to $D_2^{dec}$.\\

Now, to bound EMD between $D_3^{enc}$ and $D_2$, let us bound the sum $\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})$.
%From (1) and (3) in the description of $f^\star$, $\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})=\sum\limits_{\mathbf{X},\mathbf{Y} \in \mathcal{V}} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y}).$
\begin{eqnarray*}
&&\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})\\
&=&\sum\limits_{\mathbf{X},\mathbf{Y} \in \mathcal{V}} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})~~~\left(\mbox{From (1) and (3) in the description of $f^\star$}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f^\star_{\mathbf{\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}}\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}}}\cdot d_H({\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}},\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})\\ &&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\left(\mbox{From (2) in the description of $f^\star$}\right)\\
&\leq&\sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f^\star_{\mathbf{\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}}\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}}}\cdot d_H(\mathbf{x},\mathbf{y})~~~\left(\mbox{Observation~\ref{obs:FEproperties} (iii)}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2(\mathbf{y})}\cdot d_H(\mathbf{x},\mathbf{y})~~~\left(\mbox{From (2) in the description of $f^\star$}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\left(f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y})\cdot  \sum\limits_{\mathbf{z}\in [n]^m} \frac{D_2(\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2(\mathbf{y})}\right)\\
&=& (1-3\alpha) \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n} f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y})~~~(\mbox{By Equation}~\eqref{def:enc-dist})\\
&\leq& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n} f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y}) \leq \frac{\eps}{3}.
\end{eqnarray*}
The last inequality follows from the fact that $f'$ realizes the EMD between $D_3$ and $D^{dec}_2$.
\end{proof}

\color{black}

% \remove{As before, we will bound the Earth Mover Distance between $D_3^{enc}$ and $D_2$ in terms of their variation distance.
% \begin{eqnarray}
%     EMD(D_{3}^{enc}, D_2) &\leq& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| \nonumber \\ &=& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| + \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{U}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| \label{eqn:emdd3encd2}
% \end{eqnarray}

% As $D_3^{enc}(\mathbf{X}) = D_2(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U}$, the second term in the above equation is $0$. Now let us bound the first term. Since for every $\mathbf{X} \in \mathcal{V}$,
% $D_3^{enc}(\mathbf{X})=(1-3\alpha)D_3(\mathbf{x}) \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}$, we can deduce the following:
% \begin{eqnarray*}
% \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| &=& \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}} |(1-3\alpha)D_3(\mathbf{x})\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}-D_2(\mathbf{X})| \\
% &\leq& 3\alpha \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}}\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}D_3(\mathbf{x}) + \\ && \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}}\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}|D_3(\mathbf{x})-D_2^{dec}(\mathbf{x})| \\
% &=&3\alpha + \sum_{\mathbf{x}\in Supp(D_2^{dec})}|D_3(\mathbf{x})-D_2^{dec}(\mathbf{x})| \\
% &\leq& 3\alpha+\frac{2\eps}{3} \leq \eps
% \end{eqnarray*}
% }
% \begin{eqnarray*}
%     \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| &=& \sum_{\mathbf{X} \in \mathcal{V}}|(1-3\alpha)D_{3}(\mathbf{x}) \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} - D_2(\mathbf{X})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} |(1-3\alpha)\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} -1| \\ &\leq & \sum_{\mathbf{X} \in \mathcal{V}} D_2(\mathbf{X}) |\frac{D_3(\mathbf{x}) - D_2^{dec}(\mathbf{x})}{D_2^{dec}(\mathbf{x})}| \\ &\leq& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} \cdot \frac{\eps}{3} \leq \frac{2 \eps}{3}
% \end{eqnarray*}

%Substituting this value in Equation~\ref{eqn:emdd3encd2}, we have the result.


% Let $f^{(1)}$ be the flow from $D_2^{dec}$ to $D_3$ realizing the EMD between $D_2^{dec}$ and $D_3$. Let us consider the flow $f^{(2)}$ from $D_2$ to $D_{3}^{enc}$ as described below:
% \begin{itemize}
%     \item $f^{(2)}_{\mathbf{X}\mathbf{X}}=D_2(\mathbf{X})=D_{3}^{enc}(\mathbf{X})$ for each $\mathbf{X} \in \{\mathbf{U}'\}\cup S' \cup T'$.
    
%     \item For every $\mathbf{x},\mathbf{y} \in \{0,1\}^{n}$, 
% $f^{(2)}_{\mathbf{XY}} = (1-3\alpha)f^{(1)}_{\mathbf{xy}}$, where $\mathbf{X}= \cE(\mathbf{x})$ and $\mathbf{Y}= \cE(\mathbf{y})$.

%       \item Otherwise, $f^{(2)}_{\mathbf{XY}}=0$.
% \end{itemize}

% Now we have the following observation which directly follows from the encoding procedure.
% \begin{obs}
% For any $\mathbf{x, y}\in \{0,1\}^{n}$, the Hamming distance between their encoding is at most the Hamming distance between them.
% \end{obs}
% Thus we have the following:
% \begin{eqnarray*}
% \mbox{EMD}(D_{3}^{enc},D_2) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^{(2)}_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
% &\leq& \sum_{\mathbf{X} \in \{\mathbf{U}'\} \cup S' \cup T' } f^{(2)}_{{\bf X X}}d_H({\bf X},{\bf X}) + \sum_{\mathbf{x,y}\in \{0,1\}^{n}} f^{(2)}_{{\bf \cE(\mathbf{x})\cE(\mathbf{y})}} d_H(\cE(\mathbf{x}),\cE(\mathbf{y}))\\
% &\leq& 0+ \sum_{\mathbf{x,y}\in \{0,1\}^{n}} f^{(1)}_{\mathbf{x}\mathbf{y}} d_H(\mathbf{x},\mathbf{y})\\
% &=& EMD(D_3,D_2^{dec})\leq \eps/3.
% \end{eqnarray*}
% \end{proof}


Since the distribution $D_{3}$ over $\{0,1\}^{n}$ has support size at most $n$, following the encoding procedure, we can say that $D_3^{enc} \in \cP_{\mbox{Gap}}$. But this would contradict the fact that $D_2$ is $2\eps/3$-far from $\cP_{\mbox{Gap}}$. This completes the proof of the lemma.
\end{proof}

Combining the arguments above, we conclude that if the input distribution $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, the tester \algadpt will output {\sc Reject} with probability at least $2/3$.

\subsection{Determining the permutation $\pi$}\label{sec:quadratic_determine_permutation}

%\comments{
Here we design an algorithm that, given a distribution $D \in \cP_{\mbox{Gap}}$, can learn the permutation $\pi$ for which $D_{\pi} \in P^0_{\mbox{Gap}}$ with high probability. 

The crux of the algorithm is that if $D \in \cP_{\mbox{Gap}}$, then there exist $\mathbf{U}'=\mathbf{U}_\pi \in \{0,1\}^n$, $\cS'=\{\mathbf{\mathbf{V}}_i'=(\mathbf{V}_i)_\pi: i \in [b]\}$ and $\cT'=\{\mathbf{W}_j'=(\mathbf{W}_j)_\pi:j \in \{0\}\cup [\lceil \log kn\rceil]-1\}$ in the support of $D$ such that $D(\mathbf{U}')=\alpha$, $D(\mathbf{V}_i')=\alpha/b$ for every $i \in [b]$ and  $D(\mathbf{W}_j')=\alpha/\lceil \log kn\rceil$. \comments{Note that $\mathbf{U},\mathbf{V}_i$'s and $\mathbf{V}_j$'s are as defined in the property $\cP_{\mbox{Gap}}^0$}. The main observation is that, if we are given the set of special vectors $\{\mathbf{U'}\} \cup \cS' \cup \cT'$, then we can determine the permutation $\pi$. Our algorithm can find  $\mathbf{U}', \cS'$ and $\cT'$ with high probability, if they exist, by taking $\Oh(\log^2 N/\alpha)=\Oh(\log^2 n/\alpha)$ samples and reading them in their entirety. This is due to the fact that the probability mass of every vector in the set of special vectors is at least $\Omega(\alpha/\log n)$.

%}

The algorithm is described in the following subroutine \findpi (see Algorithm~\ref{algo:perm})~\footnote{This algorithm is not adaptive in itself, but its output is used adaptively in the testing algorithm described later.}.

\begin{algorithm}[H]\label{algo:perm}
%\scriptsize

\SetAlgoLined

\caption{\findpi}
\label{alg:findpi}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^N$.}
\KwOut{Either a permutation $\pi:[N] \rightarrow [N]$, or {\sc Fail}.}
\LinesNumbered
\begin{description}
     \item[(i)] First take a multi-set $\cX$ of $\Oh(\log^2 N/\alpha)$ samples from $D$, and query all the entries of the sampled vectors of $\cX$ to know the vectors of $\cX$ completely.
    
    
    \item[(ii)] Find the set of distinct vectors in $\cX$ that have exactly one $1$. If no such vector exists or there is more than one such vector, {\sc Fail}. Otherwise, denote by $\mathbf{U'}$ the vector that has exactly one $1$, and denote the corresponding index by $i^*$. Set $\pi(i^*)=1$, and proceed to the next step.    
    %let the vector be $\mathbf{U'}$ that has $1$ at the index $i^*$. 
    

    \item[(iii)] Find the set of distinct vectors $\cS' \subseteq \cX \setminus \{\mathbf{U'}\}$ such that every vector in $\cS'$ has $1$ at the index $i^*$ and has at least another $1$ among other indices. If no such vector exists, or $\size{\cS'} \neq b$, {\sc Fail}. Otherwise, if the vectors of $\cS'$ form a chain $\mathbf{V}'_1, \ldots, \mathbf{V}'_b$, where $\mathbf{V}'_j$ has exactly $j+1$ many $1$, then set $\pi(i_j)=j+1$, where $i_j$ is the index where $\mathbf{V}'_j$ has $1$, but $\mathbf{V}'_{j-1}$ has $0$ there, for every $j \in [b]$ (denoting $\mathbf{V'}_0=\mathbf{U'}$ for the purpose here). Also, set $B'=(i_1, \ldots,i_b)$. If $\cS'$ does not form a chain $\mathbf{V}'_1, \ldots, \mathbf{V}'_b$ as mentioned above, {\sc Fail}.
    
    
    \item[(iv)] Let $\cT' \subseteq \cX$ be the set of distinct vectors such that every vector in $\cT'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. If no such vector exists, {\sc Fail}. For every $j$, denote by $\mathbf{W}'_j$ the vector in $\cT'$ for which $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$. For every $j \in \{0\} \cup [\lceil \log kn \rceil -1]$, if either there are no vectors $\mathbf{W}'_j \in \cT'$ or there is more than one distinct vector with $\mathbf{W'_j} \mid_{B'}=b(j)$, {\sc Fail}.
    Also, if there is any vector in $\mathbf{W}'_j \in \cT'$ such that $\mathbf{W}'_j \mid_{B'} = b(j)$ for $\log kn \leq j < 2^b -1$, {\sc Fail}.
    
    \item[(v)] For any $i \in [N]\setminus (\{i^*\} \cup B')$, let $l_i$ be the integer with binary representation $(\mathbf{W'}_0)_i, \ldots, (\mathbf{W'}_{\lceil \log kn \rceil -1})_i$.
Set $\pi(i)=b+2+l_i$ for every $i \in [N]\setminus (\{i^*\} \cup B')$. If $\pi$ is not a permutation of $[N]$, {\sc Fail}.

    \item[(vi)] Take another multi-set $\cX'$ of $\Oh(\log^2 N/\alpha)$ samples from $D$, and query all the entries of the sampled vectors of $\cX'$ to know the vectors of $\cX'$ completely. Let $\cY$ be a set of vectors in $\cX'$ such that $\cY=\{\mathbf{Z} \in \cX': \mathbf{Z} \mid_{{\{i^*\} \cup B'}} \neq \mathbf{0}\mathbf{1}^b \}$. If $\size{\cY}/\size{\cX'} > 4\alpha$, {\sc Fail}. Otherwise, output $\pi$.
    
    %Estimate the fraction of vectors in $X'$ that are in $\{\mathbf{U'}\}\cup S' \cup T'$. If it is less than $4\alpha$. Otherwise, {\sc Fail}.
    
\end{description}

\end{algorithm}

\vspace{10pt}

Let us start by analyzing  the query complexity of \findpi.

\begin{lem}[Query complexity of \findpi]\label{lem:queryfindpi}
The query complexity of the above defined \findpi is $\tOh(N)$.
\end{lem}

\begin{proof}
Note that \findpi takes a multi-set $\cX$ of $\Oh(\log^2 N/\alpha)$ samples from $D$ in Step (i), and queries them completely. So, \findpi performs $\Oh(N \log^2 N/\alpha)$ queries in Step (i). \findpi does not perform any new query in Step (ii), Step (iii), Step (iv) and Step (v). Finally, \findpi takes another multi-set $\cX'$ of $\Oh(\log^2 N/\alpha)$ samples from $D$ and queries them completely, similar to Step (i). Recalling that $\alpha=1/\log n$, the query complexity of \findpi is $\tOh(N)= \tOh(n)$ in total.
\end{proof}


Now we proceed to prove the correctness of \findpi.
\color{blue}
\begin{lem}[Guarantee when $D \in \cP_{\mbox{Gap}}$]\label{lem:findpicompleteness}
If $D$ is a distribution defined over $\{0,1\}^N$ such that $D \in \cP_{\mbox{Gap}}$, then with probability at least $9/10$, \findpi reports permutation $\pi$ such that $D_{\pi} \in \cP_{\mbox{Gap}}^0$.
\end{lem}

We prove the above lemma by a series of intermediate lemmas. \color{black} In the following lemmas, we consider $\mathbf{U}$, $\cS$ and $\cT$ as per the definition of $\cP^0_{\mbox{Gap}}$. Also, consider the permutation $\pi$ such that $D_\pi \in \cP_{\mbox{Gap}}$.
%To argue the completeness of our algorithm, consider a distribution $D$ over $\{0,1\}^N$ such that $D\in \cP_{\mbox{Gap}}$, and let $\pi$ be the permutation for which $D_{\pi} \in \cP^0_{\mbox{Gap}}$. 

%Now consider the following lemma.

%So, there exists the four types of vectors as described in the definition of $\cP_{\mbox{Gap}}$. By using Chernoff bound, we have the following:

\begin{lem}[correctly finding $\pi^{-1}(1)$]\label{lem:hittingU}
With probability at least $1-1/N^3$, $\cX$ will contain the vector $\mathbf{U'}$ for which $\mathbf{U'}_{\pi}=\mathbf{U}$, and $i^*=\pi^{-1}(1)$ will be identified correctly.
\comments{Moreover, \findpi proceeds to Step (iii).}
%Let $\mathbf{U'} \in \{0,1\}^N$ be a vector that has exactly a single $1$ at some index $i^*$, and $D$ be a distribution over $\{0,1\}^N$ such that $D(\mathbf{U'})= \alpha$. Consider the multi-set of samples $X$ taken from $D$ in Step (i) of \findpi such that $\size{X} = \Oh(\log^2 N/\alpha)$. Then with probability at least $1 - \frac{1}{N^3}$, $\mathbf{U'} \in X$. 
\end{lem}

\begin{proof}
By the definition of $\cP^0_{\mbox{Gap}}$, the vector $\mathbf{U'}$ is the only vector in the support of $D$ containing a single $1$. Since $D(\mathbf{U'}) = D(\mathbf{U}_{\pi^{-1}(1)}) = \alpha$, and we are taking $\size{\cX}$ many samples from $D$, the probability that $\mathbf{U'}$ will not appear in $\cX$ is at most $(1- \alpha)^{\size{X}} \leq \frac{1}{N^3}$. Thus, with probability at least $1 - \frac{1}{N^3}$, $\mathbf{U'} \in \cX$ and \findpi in Step (ii) proceeds to the next step
%This completes the proof of the lemma.
\end{proof}

\begin{lem}[correctly finding $B' = \pi^{-1}(B)$]\label{lem:hittingS}
With probability at least $1-1/N^3$, the algorithm \findpi will correctly identify $\mathbf{V'}_1, \ldots, \mathbf{V'}_b$ for which $\mathbf{V'}_{i,\pi} = \mathbf{V}_i$, and $B'={\pi^{-1}(2), \ldots, \pi^{-1}(b+1)}$ will be identified correctly as well. \comments{Moreover, \findpi proceeds to Step (iv).}

%Let $S'= \{\mathbf{V}'_1, \ldots, \mathbf{V}'_b\}$ be a set of vectors in $\{0,1\}^N$ such that for each $\mathbf{V}'_i \in S'$, $\mathbf{V}'_i$ has $1$ at some index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B$. Moreover, $D(\mathbf{V}'_i) = \alpha/b$ for each $i \in [b]$. Then with probability at least $1 - \frac{1}{N^3}$, $S' \subseteq X$, where $X$ is the multi-set of samples obtained from $D$ and $\size{X}= \Oh(\log^2 N/\alpha)$.
\end{lem}

\begin{proof}
%Let us consider an arbitrary vector $\mathbf{V}'_i \in S'$.

Let $\mathbf{V'}_1, \ldots, \mathbf{V'}_b$ denote the vectors for which $\mathbf{V'}_{i,\pi}=\mathbf{V}_i$ for every $i$. Note that these are the only vectors outside $\mathbf{U'}$ in the support of $D$ that have $1$ at the index $i^*$.
As $D(\mathbf{V}'_i)= \frac{\alpha}{b}$, the probability that $\mathbf{V}'_i$ does not appear in $\cX$ is at most $(1- \frac{\alpha}{b})^{\size{X}}$. Since $\size{\cX} = \Oh(\log^2 N/\alpha)$ and $b = \Oh(\log \log kn)$, the probability that $\mathbf{V}'_i \in \cX$ is at least $1 - \frac{1}{N^4}$. Using the union bound over all the vectors of $\cS'$, with probability at least $1-1/N^3$, we know that all of these vectors are in $\cX$, in which case they are identified correctly, so $B'$ is identified correctly as well, and \findpi in Step (iii) proceeds to the next step.
\end{proof}

\begin{lem}[correctly identifying $\pi^{-1}(b+2), \ldots, \pi^{-1}(N)$]\label{lem:hittingT}
Let $\mathbf{W'}_1, \ldots, \mathbf{W'}_{\lceil \log kn \rceil -1}$ denote the vectors for which $\mathbf{W'}_{j,\pi} = \mathbf{W}_j$ for every $j$. With probability at least $1-1/N^3$, all these vectors appear in $\cX$, in which case they are identified correctly, and so are $\pi^{-1}(b+2), \ldots, \pi^{-1}(N)$. \comments{Moreover, \findpi proceeds to Step (vi).}

%Let $T'= \{\mathbf{W}'_1, \ldots, \mathbf{W}'_{\log kn}\}$ be a set of vectors (disjoint from $S'$) in $\{0,1\}^N$ such that for each $\mathbf{W}'_i \in T'$, $\mathbf{W}'_i$ contains $1$ at the index $i^*$, for every $i \in [\log n]$, the decimal evaluation of $\mathbf{W}'_i \mid_{B'}$ is $i$. Moreover, $D(\mathbf{W}'_i) = \alpha/\log kn$ for each $i \in \{0\} \cup [\log kn -1]$. Then with probability at least $1 - \frac{1}{N^3}$, $T' \subseteq X$, where $X$ is the multi-set of samples obtained from $D$ and $\size{X}= \Oh(\log^2 N/\alpha)$.
\end{lem}

The proof of the above lemma is similar to the proof of Lemma~\ref{lem:hittingS} and is omitted. Note that from Lemma~\ref{lem:hittingU}, Lemma~\ref{lem:hittingS} and Lemma~\ref{lem:hittingT}, we know that with probability at least $1-o(1)$, the algorithm \findpi has correctly determined the permutation $\pi$ and proceeded to Step (vi). We will finish up the proof of Lemma~\ref{lem:findpicompleteness} having the following lemma.

%proceeded to Step (v). Since the vectors in $\{\mathbf{U}\} \cup S \cup T$ are disjoint, \findpi correctly determines the permutation $\pi$ with probability at least $1-o(1)$.

\begin{lem}
The probability that \findpi outputs {\sc Fail} in Step (vi) (instead of outputting $\pi$) is at most $1/N^3$.

%With probability at least $1 - \frac{1}{N^3}$, $\size{\cY}/\size{X'} \leq 4 \alpha$.
%the fraction of vectors in $X'$ that are in $\{\mathbf{U}\} \cup S \cup T$ is at most $4 \alpha$.
\end{lem}

\begin{proof}
As $D \in \cP_{\mbox{Gap}}$, from the description of the property, we know that $D(\{\mathbf{U'}\} \cup \cS' \cup \cT')= 3 \alpha$. As $\size{\cX'}= \Oh(\log^2 N/\alpha)$, using the Chernoff bound, we have the result.
\end{proof}

Combining the above lemmas, we conclude that with probability at least $9/10$, the algorithm \findpi outputs a correct permutation $\pi$, completing the proof of Lemma~\ref{lem:findpicompleteness}.

To conclude this section, we show that with high probability, we will not output $\pi$ for which too much weight is placed outside the ``\emph{encoded part}'' of the distribution.

%Now consider the case when $D(\{\mathbf{U'}\}\cup S' \cup T'\}) \geq 5 \alpha$. Then we can say that \findpi will output {\sc Fail} with high probability.

\begin{lem}\label{lem:findpisumfourthtype}
For any distribution $D$ (regardless of whether $D$ is in $\cP_{\mbox{Gap}}$ or not), the probability that \findpi outputs a permutation $\pi$ for which $D(\{\mathbf{X}:\mathbf{X}_{\{i^*\} \cup B'}=\mathbf{0}\mathbf{1}^b\}) \leq 1-5\alpha$ is at most $1/10$.

%Consider any distribution $D$ over $\{0,1\}^N$ such that $D(\{\mathbf{U'}\}\cup S' \cup T'\}) \geq 5 \alpha$. Then with probability at most $1/10$, \findpi outputs a permutation $\pi$.
\end{lem}

\begin{proof}
Recall the set of vectors $\cY$ as defined in Step (vi) of \findpi: $\cY=\{\mathbf{Z} \in \cX': \mathbf{Z} \mid_{{{i^*} \cup B'}} \neq \mathbf{0}\mathbf{1}^b \}$, where $\cX'$ is the multi-set of (new) samples obtained in Step (vi) of \findpi. Consider a distribution $D$ such that $D(\{\mathbf{X}:\mathbf{X}_{\{i^*\} \cup B'}=\mathbf{0}\mathbf{1}^b\}) \leq 1-5\alpha$. This implies that $\E\left[\size{\cY}/\size{\cX'}\right] \geq 5 \alpha$. As $\size{\cX'} = \Oh(\log^2 N/\alpha)$, using the Chernoff bound, we obtain that with probability at least $9/10$, the algorithm \findpi outputs {\sc Fail} in Step (vi), and does not output any permutation $\pi$. This completes the proof.
\end{proof}

\subsection{The upper bound on adaptive testing for property $\cP_{\mbox{Gap}}$}\label{sec:quadratic_adaptive_ub}

In this subsection, we design the adaptive tester for the property $\cP_{\mbox{Gap}}$. Given a distribution $D$ over $\{0,1\}^N$, with high probability, \algadpt outputs {\sc Accept} when $D \in \cP_{\mbox{Gap}}$, and outputs {\sc Reject} when $D$ is far from $\cP_{\mbox{Gap}}$. The formal adaptive algorithm is presented in \algadpt (see Algorithm~\ref{algo:adaptive}). Note that it has only two adaptive steps.

%\comments{

In the first adaptive step, our tester \algadpt starts by calling the algorithm \findpi (as described in Subsection~\ref{sec:quadratic_determine_permutation}) whose  query complexity is $\tOh(n)$. If $D \in \cP_{\mbox{Gap}}$, with high probability, \findpi returns the permutation $\pi$ such that $D_{\pi} \in \cP_{\mbox{Gap}}^0$. Once $\pi$ is known, when we obtain a sample $\mathbf{X}$ from $D$, we can consider it as $\mathbf{X}_\pi$ from $D_{\pi}$. Also, from the structure of the vectors in the support of the distributions in $P^0_{\mbox{Gap}}$, we can decide whether $X_{\pi}$ is a special vector, that is, $X_{\pi} \in \{\mathbf{U}\} \cup \cS \cup \cT$ or $\mathbf{X}_\pi$ is an encoding vector, that is, $\mathbf{X}_\pi=\fen(\mathbf{z},\mathbf{x})$ for some $\mathbf{z}\in [n]^m$ and $\mathbf{x} \in \{0,1\}^n$. Observe that, in the later case, we can decode any bit of $\mathbf{x}$ (say $\mathbf{x}_j$) by finding $\mathbf{X}_\pi$ projected into $C_j$, which can be done by performing $\Oh(\log n)$ queries.

%} 

%\comments{
As the second adaptive step, our algorithm asks for a sequence $\cY$ of $\Oh(n/\eps)$ samples from $D$, that is, from $D_{\pi}$. Let $\cY'\subseteq \cY$ be the sequence of encoding vectors in $\cY$. We now call {\sc Supp-Est}$(\cY', \eps/3)$ (from Lemma~\ref{pre:suppest}), and depending on its output, \algadpt either reports {\sc Accept} or {\sc Reject}. Note that we can execute every query by {\sc Supp-Est}$(\cY', \eps/3)$, by performing $\Oh(\log n)$ queries to the corresponding sample in $\cY'$ \comments{as discussed towords the end of the above paragraph.}
%}  

\comments{
When $D \in \cP_{\mbox{Gap}}$ (that is, $D_\pi \in \cP_{\mbox{Gap}}^0$ for the permutation $\pi$), the set of encoding vectors in $D_\pi$ is the encoding of at most $n$ vectors in $\{0,1\}^n$. So, in that case, \algadpt reports {\sc Accept} with high probability. Now consider the case, when $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. If \algadpt has not rejected $D$ before calling {\sc Supp-Est}$(\cY', \eps/3)$, we will show that the distribution over $\{0,1\}^n$ induced by the vectors decoded from the encoding vectors in $D_{\pi}$ is ${\eps}/3$-far from having support size $n$. Then, \algadpt will reject $D$ with high probability.
}


\begin{algorithm}[H]\label{algo:adaptive}
%\scriptsize
\SetAlgoLined

\caption{\algadpt}
\label{alg:adaptive}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^N$, and a parameter $\eps \in (0,1)$.}
\KwOut{Either {\sc Accept} or {\sc Reject}.}
\LinesNumbered
\begin{description}
     \item[(i)] Call \findpi. If \findpi returns {\sc Fail}, {\sc Reject}. Otherwise, let $\pi$ be the permutation returned by \findpi. Denote for convenience $i^*=\pi^{-1}(1), B'=\pi^{-1}(B)$, and $C'_j=\pi^{-1}(C_j)$ for every $j \in [n]$.
     
     \item[(ii)] Take a multi-set $\cX$ of $\Oh(1/\eps)$ samples from $D$, and query all the entries of the sampled vectors of $\cX$ to know the vectors of $\cX$ completely. If there is any vector $\mathbf{X}$ for which $\mathbf{X} \mid_{\{i^*\} \cup B'} = \mathbf{0}\mathbf{1}^b$ (according to the permutation $\pi$ obtained from Step (i)) for which $\mathbf{X}_{\pi}$ is not in the image of $\mbox{{\sc FE}}$ (i.e. it is not a valid encoding of any vector in $\{0,1\}^n$), {\sc Reject}. Otherwise, proceed to the next step.
     
     %Construct a sequence of vectors $X' \subseteq X$ such that for every $\mathbf{X} \in X'$, $\mathbf{X} \mid_{\{i^*\}\cup B'} = \mathbf{0}\mathbf{1}^b$ (according to the permutation $\pi$ obtained from Step (i)). If the fraction $\frac{\size{X \setminus X'}}{\size{X}} > \frac{\eps}{10}$
     
     %For every $\mathbf{X} \in X$, query the indices $\{i^*\} \cup B'$ (according to the permutation $\pi$ obtained from Step (i)) to $\mathbf{X}$. 
     %For any $\mathbf{X} \in X$, if $\mathbf{X} \mid_{\{i^*\}\cup B'} = \mathbf{0}\mathbf{1}^b$, then choose a uniformly random $j \in [n]$, and check whether $\mathbf{X} \mid_{C'_j} \in \mathcal{E}(0)\cup\mathcal{E}(1)$, that is, whether it is a valid encoding of some value in $\{0,1\}$. If any invalid encoding is found for any $\mathbf{X} \mid_{C'_j}$, {\sc Reject}.

     %Construct the sequence of vectors $X'$ such that $X' = \{\mathbf{X} \in X: \mathbf{X} \mid_{\{i^*\} \cup B'} = \mathbf{0} \mathbf{1}^b\}$. Now sample a set of indices $\cI \subseteq [n]$ without replacement such that $\size{\cI}=\Oh(1/\eps)$. 
     
     %For every $\mathbf{X} \in X'$, choose a $j \in \cI$  randomly, and  check if $\mathbf{X} \mid_{C'_j}$ is a valid encoding of some vector $\mathbf{x} \in \{0,1\}^n$ with respect to the code ensemble $\cE$ by querying the appropriate indices of $\mathbf{X}$. If $\mathbf{X} \mid_{C'_j}$ is not a valid encoding for some $j \in \cI$, {\sc Reject}.
     
     %where $C_j$ denotes the set of indices of $[N]$ such that $C_j= \{b+2+k(j-1), \ldots, b+1+kj\}$.

    \item[(iii)]Take a sequence of samples $\cY$ such that $\size{\cY}=\Oh(n/\eps)$ from $D$. Now construct the sequence of vectors $\cY'$ such that $\cY'= \{\mathbf{Y} \in \cY: \mathbf{Y} \mid_{\{i^*\} \cup B'} = \mathbf{0} \mathbf{1}^b\}$ by querying the indices corresponding to $\{i^*\} \cup B'$.

    \item[(iv)] Call {\sc Supp-Est}$(\cY', \eps/3)$ (from Lemma~\ref{pre:suppest}), where a query to an index $j$ is simulated by querying the indices of $C'_j$ and decoding the obtained vector with respect to to $\mbox{{\sc SE}}$ (that is, checking whether the restriction of the queried vector to $C'_j$ is equal to $\mbox{{\sc SE}}(i,0)$ for some $i$, or equal to $\mbox{{\sc SE}}(i,1)$ for some i). {\sc Reject} if any of the following conditions hold:
    \begin{itemize}
        \item[(a)] $\size{\cY'}/\size{\cY} \leq 1/2$ (due to the absence of sufficiently many samples in $\cY'$ to apply {\sc Supp-Est}).

        \item[(b)] {\sc Supp-Est}$(\cY', \eps/3)$ queries an index $j$ from some $\comments{\mathbf{Y}_i}$ corresponding to an invalid encoding of $\comments{\mathbf{Y}_i} \mid_{C'_j}$ (that is, when $\comments{\mathbf{Y}_i} \mid_{C'_j}$ is not in the image of $\mbox{{\sc SE}}$).
        
        \item[(c)] {\sc Supp-Est}$(\cY',\eps/3)$ outputs {\sc Reject}.
    \end{itemize}

    Otherwise, {\sc Accept}.

\end{description}

\end{algorithm}

\vspace{10pt}

Let us first discuss the query complexity of \algadpt.

\begin{lem}[Query complexity of \algadpt]
The query complexity of the adaptive tester \algadpt for testing the property $\cP_{\mbox{Gap}}$ is $\tOh(N)= \tOh(n)$.    
\end{lem}

\begin{proof}
Note that \algadpt calls the algorithm \findpi in Step (i). Following the query complexity lemma of \findpi (Lemma~\ref{lem:queryfindpi}), we know that \findpi performs $\tOh(N)$ queries.

For every sample taken in Step (ii), the sampled vectors of the multi-set $\cX$ are queried completely. Since we take $\Oh(1/\eps)$ samples, this step requires $\Oh(N/\eps) = \widetilde{\Oh}(n/\eps)$ queries in total.  
    
%the indices of $\{i^*\}\cup B'$ are queried (taking $b+1=\Oh(\log \log kn/\eps)$ many queries), as well as possibly the indices of some $C'_j$ (taking $k=\Oh(\log n)$ many queries). Since we take $\Oh(1/\eps)$ many samples, this step requires $\Oh(\log n/\eps)$ many queries in total.

%In Step (ii), \algadpt first takes a multi-set of samples $X$ such that $\size{X}= \Oh(1/\eps)$ and then queries the indices of $\{i^*\} \cup B'$ of the vectors of $X$ to obtain $X'$. This procedure requires $\Oh(\log \log kn/ \eps)$ many queries. Also, in the same step, \algadpt tests whether the vectors of $X'$ are valid encodings with respect to the code ensemble $\cE$. This requires $\Oh(\log n/\eps^2)$ many queries.

Then in Step (iii), \algadpt takes a multi-set $\cY$ of $\Oh(n/\eps)$ samples, and queries for the indices in $\{i^*\} \cup B'$ to obtain the vectors in $\cY'$, which takes $\Oh(n \log \log kn/\eps)$ queries. Finally, in Step (iv), \algadpt calls the algorithm {\sc Supp-Est}, which performs $\tOh(n)$ queries (following Lemma~\ref{pre:suppest}), each of them simulated by $\Oh(\log n)$ queries to some $\comments{\mathbf{Y}_i} \mid_{{C'_j}}$. Thus, in total, \algadpt performs $\tOh(N) = \tOh(n)$ queries.
\end{proof}

Now we prove the correctness of \algadpt. We will start with the completeness proof.

\begin{lem}[Completeness]
Let $D$ be a distribution defined over $\{0,1\}^N$. If $D \in \cP_{\mbox{Gap}}$, then the algorithm \algadpt will output {\sc Accept} with probability at least $2/3$.
\end{lem}

\begin{proof}
Consider a distribution $D \in \cP_{\mbox{Gap}}$. From the completeness lemma of \findpi (Lemma~\ref{lem:findpicompleteness}), we infer that with probability at least $9/10$, \findpi returns the correct permutation $\pi$ in Step (i). Then, by the definition of $\cP_{\mbox{Gap}}$, the algorithm \algadpt can never encounter any samples with invalid encodings in Step (ii) which could cause it to {\sc Reject}. Thus, with probability at least $9/10$, the algorithm proceeds, with the correct permutation $\pi$, to Step (iii) and Step (iv).
    
%and no invalid encodings have been encountered. Thus \algadpt proceeds to Step (ii) with the same probability. Since $D \in \cP_{\mbox{Gap}}$, the total mass of the valid encoding vectors of $D$ is $1-3\alpha$. Thus, using the Chernoff bound, we can say that in Step (ii), the fraction of sampled vectors in $X$ that are not in $X'$ is at most $\eps/10$. So, \algadpt successfully completes this step and proceeds to Step (iii) and Step (iv).

As $D \in \cP_{\mbox{Gap}}$, $D(\{\mathbf{U'}\} \cup \cS' \cup \cT') = 3 \alpha$. As $\size{\cY}= \Oh(n/\eps)$, using the Chernoff bound, we can say that, with probability at least $9/10$, $\size{\cY'}/\size{\cY} \geq 1/2$. Moreover, as the vectors in $\cY'$ are valid encodings with respect to the function $\mbox{{\sc FE}}$ of at most $n$ vectors from $[2n]$, following the support estimation upper bound lemma (Lemma~\ref{pre:suppest}), we obtain that {\sc Supp-Est} outputs {\sc Accept} with probability at least $9/10$. Combining these, we conclude that \algadpt outputs {\sc Accept} with probability at least $2/3$.
\end{proof}

Now we prove that when $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, \algadpt will output {\sc Reject} with probability at least $2/3$.

\begin{lem}[Soundness]\label{lem:sound}
    Let $\eps \in (0,1)$ be a proximity parameter. Assume that $D$ is a distribution defined over $\{0,1\}^N$ such that $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. Then \algadpt outputs {\sc Reject} with probability at least $2/3$.
\end{lem}

%From the description of \algadpt (Algorithm~\ref{algo:adaptive}), if the tester reports {\sc Reject} before executing all the steps of {{\sc Supp-Est}}$(\cY',\eps/3)$ in Step (iv),  then we are done. So, assume that \algadpt executes all the steps of {{\sc Supp-Est}}$(\cY',\eps/3)$. Let $\cY'$ be the set of samples from distribution $D^*$ over $\{0,1\}^n$. Note that $D^*$ is unknown and we are accessing $D^*$ indirectly via decoding sample from $D$ over $\{0,1\}^n$. From the correctness {{\sc Supp-Est}}$(\cY',\eps/3)$, we will be done with the proof of Lemma~\ref{lem:sound}.
\comments{We prove the above lemma by a series of claims.}
%\begin{proof}
Let $D$ be a distribution which is $\eps$-far from $\cP_{\mbox{Gap}}$, and $\mathcal{V}$ denote the set $\{\mathbf{X} \in \mbox{Supp}(D) : \mathbf{X} \mid_{\{i^*\}\cup B'}=\mathbf{0}\mathbf{1}^b\}$, and let us define $\mathcal{U}= \mbox{Supp}(D) \setminus \mathcal{V}$. Let us start with the following observation.

%If \algadpt outputs {\sc Reject} in either Step (i) or Step (ii), then we are done. Otherwise, let us assume that \algadpt has proceeded to Step (iii) and Step (iv). Now we need to argue that when we call the algorithm {\sc Supp-Est}, it will output {\sc Reject} with probability at least $9/10$.

\begin{obs}\label{obs:sumdothervec}
$D(\mathcal{U}) \leq 5\alpha$, unless the algorithm \algadpt has rejected with probability at least $1-1/N^3$ in Step (i).
%$D(\{\mathbf{U'}\}\cup S' \cup T') \leq 5\alpha$ with probability at least $1- \frac{1}{N^3}$.
\end{obs}

\begin{proof}
Since \algadpt in Step (i) invokes the algorithm \findpi, this follows immediately from Lemma~\ref{lem:findpisumfourthtype}.
%Since \findpi has not output {\sc Fail} for the input distribution $D$ in Step $(vi)$, this implies that the fraction of vectors in $Y'$ that belong to the set $\{\mathbf{U'}\} \cup S' \cup T'$ is at most $4 \alpha$. Since $\size{Y} = \Oh(n/\eps)$, using the Chernoff bound, we can say that with probability at least $1- \frac{1}{N^3}$, $D(\{\mathbf{U'}\} \cup S' \cup T') \leq 5 \alpha$.
\end{proof}

% Thus with probability at least $1- \frac{1}{N^3}$, we can say that: 
% \begin{itemize}

%     \item[(i)] There exists a vector $\mathbf{U}' \in \{0,1\}^N$ that has $0$ at some index $i^*$ and $0$ in all other indices. 
    
%     %Also, $D(\mathbf{U})= \alpha$.
    
%     \item[(ii)] There exists a set of vectors $S'=\{\mathbf{V'}_1, \ldots, \mathbf{V'}_b\}$ in $\{0,1\}^N$ such that for every $\mathbf{V'}_i \in S$, $\mathbf{V'}_i$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B'$ and $0$ in all other indices. 
    
%     %Moreover, $D(\mathbf{V_i}) = \alpha/\size{B}$ for every $i \in [\size{B}]$.

%     \item[(iii)] There exists a set of vectors $T'= \{\mathbf{W_0}, \ldots, \mathbf{W}_{\lceil \log kn \rceil -1}\}$ (disjoint from $S'$) in $\{0,1\}^N$ such that each vector in $T'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. For every $j$, denote by $\mathbf{W}'_j$ the vector in $T'$ for which $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$.

%     %for each $\mathbf{W}_i \in T'$, $\mathbf{W}_i$ is of the form $\mathbf{0}(b(i))(\mathbf{0}^{2^i}\mathbf{1}^{2^i})^{kn/2^{i+1}}$, where $b(i)$ denotes the binary representation of $i$.
%     %for each $\mathbf{W_i} \in T$, $\mathbf{W_i}$ has $0$ at the index $i^*$ and the decimal evaluation of $\mathbf{W_i}$ is $i$ when projected to the indices in $B$. Let $N' = [N]\setminus B\cup \{i^*\}$ and $\mathbf{W}_i'=\mathbf{W}_i \mid_{N'}$ for every $i \in [\log n]$ such that for every $j \in N'$, the $j$-th bit of $\mathbf{W}'_i$ is $1$ if and only if $j$ divided by $2^i$ produces an odd number. 
    
%     %Moreover, $D(\mathbf{W_i}) = \alpha/\log n$ for every $i \in [\log n]$.
%     \item[(iv)] $D(\{\mathbf{U}'\}\cup S' \cup T') \leq 5\alpha$.
    
%     \item[(v)] Let $\pi$ be the permutation obtained from \findpi. Let $\mathcal{V}$ be the set of vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$. For each vector $\mathbf{V} \in \mathcal{V}$, consider a set of $\Gamma_{\mathbf{V}}=\{\mathbf{v_1,\ldots,\mathbf{v}_{n}}\}$ of $n$ vectors in $\{0,1\}^{n}$, such that
%     the $j$-th index of $\mathbf{v}_i$ has the same value present in the $\{\pi((i-1)\lceil \log kn \rceil +j)$-th index of $\mathbf{V}$. Let $\Gamma'_{\mathbf{V}} \subseteq \Gamma_{\mathbf{V}}$ be the set of vectors that are not valid encoding with respect to $\cE$. Let $\Gamma=\bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$.
    
%     %Then $\sum_{\mathbf{V}\in \mathcal{V}} D(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \alpha$.
    
    
%    % $\mathbf{V}$ is not an encoding with respect to $\cE$. Then $D(\mathcal{V})\leq \alpha$.
%     %and the remaining set of indices are code ensemble of vectors in $\{0,1\}^{n/\log n}$.
    
% \end{itemize}

%Let $\mathcal{V}$ be the set of vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$. For each vector $\mathbf{V} \in \mathcal{V}$, consider a set of $\Gamma_{\mathbf{V}}=\{\mathbf{v_1,\ldots,\mathbf{v}_{n}}\}$ of $n$ vectors in $\{0,1\}^{n}$, such that the $j$-th index of $\mathbf{v}_i$ has the same value present in the $\{\pi((i-1)\lceil \log kn \rceil +j)$-th index of $\mathbf{V}$, where $\pi$ is the permutation returned by \findpi. Let $\Gamma'_{\mathbf{V}} \subseteq \Gamma_{\mathbf{V}}$ be the set of vectors that are not valid encodings with respect to $\cE$. Let $\Gamma=\bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$ be the set of all such vectors. 


Let $\mathcal{V}^{\mbox{inv}} \subseteq \mathcal{V}$ denote the following set of vectors:
$$\mathcal{V}^{\mbox{inv}} = \{\mathbf{X} \in \mathcal{V}: \mathbf{X} \neq \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \ \mbox{for all} \ \mathbf{z} \in [n]^m, \mathbf{x} \in \{0,1\}^n\}$$

For every vector $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$, let $\Gamma'_{\mathbf{V}}=\{j\in [n]: \mathbf{V}\mid_{C'_j} \ \mbox{is not in the image of} \ \mbox{{\sc SE}}\}$ denotes \comments{the set of indices in $[n]$ of chunks of all the ``\emph{locally invalid}'' encodings} in the vector $\mathbf{V}$~\footnote{Note that it may be the case that $\Gamma'_{\mathbf{V}}=\emptyset$, for example when for every $j \in [n]$, we have $\mathbf{V} \mid_{C'_j} = \mbox{{\sc SE}}(i_j, \mathbf{x}_j)$, for some $i_1, \ldots, i_n$ and $\mathbf{x}_1, \ldots, \mathbf{x}_n$ for which $i_1, \ldots, i_n$ are not in the image of $\mbox{{\sc GE}}$.}.

%Now we have the following lemma.

% \begin{lem}\label{lem:sumencvector}
%     $\sum_{\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}} D(\mathbf{V})\frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \eps/10$, unless \algadpt has rejected with probability at least $2/3$ in Step (ii).
% \end{lem}

% \begin{proof}
% For every $\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}$, the probability that a sample $\mathbf{X}$ taken in Step (ii) is equal to $\mathbf{V}$ is $D(\mathbf{V})$, and then the probability that $\mathbf{V} \mid_{C'_j}$ is an invalid encoding is exactly $|\Gamma'_{\mathbf{V}}|/n$. This implies that for every sample $\mathbf{X} \in X$, the probability that it causes a rejection is exactly $\sum_{\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}}D(\mathbf{V})|\Gamma'_{\mathbf{V}}|/n$.  The lemma follows since we have taken $\Oh(1/\eps)$ many independent samples in Step (ii).

% %Recall that during the execution of the tester \algadpt in Step (ii), \algadpt selects a subset of indices $\cI \subseteq [n]$, and for every $\mathbf{V} \in X'$, chooses an index $j \in \cI$ randomly and checks whether $\mathbf{V} \mid_{C'_j}$ is a valid encoding with respect to $\cE$ or not. As $\Gamma'_{\mathbf{V}}$ is the set of vectors that are not valid encodings of any vector $\mathbf{V}$, the probability that \algadpt \ {\sc Rejects} a fixed vector $\mathbf{V}$ is $\frac{\size{\Gamma'_{\mathbf{V}}}}{n}$. As $\size{\cI} = \Oh(1/\eps)$, applying the Chernoff bound and summing over all vectors $\mathbf{V} \in \mathcal{V}$, we have the result.
% \end{proof}

For any distribution $D$ that has not been rejected by \algadpt in Step (i) and Step (ii), let us define another distribution $D_1$ over $\{0,1\}^N$ such that $D_1(\mathbf{U}') = \alpha$, $D_1(\mathbf{X}) = \frac{\alpha}{b}$ for every $\mathbf{X} \in \cS'$, $D_1(\mathbf{X}) = \frac{\alpha}{\lceil \log kn \rceil}$ for every $\mathbf{X} \in \cT'$, and $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$. Then we have the following lemma.

\begin{lem}\label{obs:massnonenc}
$D_1(\mathcal{V}^{\mbox{inv}}) \leq \eps/8$.
\end{lem}

%$\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}} D_1(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \frac{\eps}{8}$.

\begin{proof}
We first note that unless $D(\mathcal{V}^{\mbox{inv}}) \leq \eps/10$, Step (ii) of \algadpt would have rejected with probability at least $2/3$. Additionally, from Observation~\ref{obs:sumdothervec}, we know that $D(\{\mathbf{U}'\} \cup \cS' \cup \cT') \leq 5 \alpha$. As $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$, and $\mathcal{V}^{\mbox{inv}} \subseteq \mathcal{V}$, we can say that for every $\mathbf{X} \in \mathcal{V}^{\mbox{inv}}$, $D_1(\mathbf{X}) \leq (1- 3 \alpha)D(\mathbf{X})/(1-5 \alpha)$. Since $\alpha = 1/\log n$, we obtain the result for sufficiently large $n$.
\end{proof}

%From Observation~\ref{obs:sumdothervec}, we know that $D(\{\mathbf{U}'\} \cup S' \cup T') \leq 5 \alpha$. As $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$, and $\mathcal{V}^{\mbox{invalid}} \subseteq \mathcal{V}$, we can say that for every $\mathbf{X} \in \mathcal{V}^{\mbox{invalid}}$, $D_1(\mathbf{X}) \leq \frac{1- 3 \alpha}{1 - 5 \alpha} D(\mathbf{X})$. Since $\alpha=1/\log n$, from Lemma~\ref{lem:sumencvector}, we know that $\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}} D(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \frac{\eps}{10}$, for sufficiently large $n$, we have the result.


Now we show that the Earth Mover Distance between the distributions $D$ and $D_1$ is not large.

\begin{lem}\label{lem:dd1emd}
The Earth Mover Distance between $D$ and $D_1$ is at most $6\alpha$.
\end{lem}

\begin{proof}
We will bound the Earth Mover Distance between $D$ and $D_1$ in terms of the variation distance between them as follows:
\begin{eqnarray}
    EMD(D,D_1) &\leq& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N}|D(\mathbf{X}) - D_1(\mathbf{X})| \nonumber \\ &=& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})| + \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})| \label{eqn:emddd1}
\end{eqnarray}

\color{blue}

Let us bound the first term as follows:
\begin{eqnarray*}
    \sum_{\mathbf{X} \in \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})|
    &=& \sum_{\mathbf{X} \in \mathcal{V}}| (1- 3 \alpha) \frac{D(\mathbf{X})}{D(\mathcal{V})} - D(\mathbf{X})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D(\mathbf{X})}{D(\mathcal{V})} |(1- 3 \alpha) - D(\mathcal{V})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D(\mathbf{X})}{D(\mathcal{V})} |3 \alpha - (1- D(\mathcal{V}))| \\ &\leq & \sum_{\mathbf{X} \in \mathcal{V}} 3 \alpha \frac{D(\mathbf{X})}{D(\mathcal{V})} \leq 3 \alpha ~~~(\because D(\mathcal{V})=1-D(\mathcal{U})\geq 1- 5 \alpha)
\end{eqnarray*}

\color{black}

As $D(\mathcal{U}) \leq 5 \alpha$, and $D_1(\mathcal{U}) \leq 3 \alpha$, we have
    $\sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}}|D(\mathbf{X}) - D_1(\mathbf{X})| \leq 8 \alpha$.
Following Equation~\ref{eqn:emddd1}, we conclude that $EMD(D,D_1) \leq 6 \alpha$, which completes the proof.
\end{proof}
% Recall that the  EMD between $D$ and $D_1$ is the solution to the following LP:
% \begin{eqnarray*}
%     &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
%     &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D(\mathbf{X})~\forall \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
%     \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_1(\mathbf{Y})~\forall \mathbf{Y} \in \{0,1\}^N.
% \end{eqnarray*}
% % Now consider the following two cases:
% % \begin{itemize}
% %     \item[(a)] $\sum_{\mathbf{Y} \notin \{\mathbf{U}\} \cup S \cup T} D(\mathbf{Y}) \geq 1-3 \alpha$: 
% % \end{itemize}
% % In this case $D_1(\mathbf{Y})\geq D(\mathbf{Y})$ for every $\mathbf{Y} \notin \{\mathbf{U}\} \cup S \cup T$.
% Consider the flow $f^*$ such that
% $f^*_{\mathbf{XX}}=D(\mathbf{X})$ for every $\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'$.

% \begin{obs}
% $\sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{\mathbf{XX}} \geq 1-5 \alpha$.
% \end{obs}

% \begin{proof}
% \begin{eqnarray*}
% \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{\mathbf{XX}}&=&\sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} \min \{D(\mathbf{X}),D_1(\mathbf{X})\} \\ &=&
% \min \left \lbrace \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} D(\mathbf{X}), \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} D_1(\mathbf{X}) \right \rbrace \\
% &\geq& \min \{1-5\alpha,1-3\alpha\}=1-5\alpha.
% \end{eqnarray*}
% %&=& \sum_{\mathbf{X} \notin \{\mathbf{U}\} \cup S \cup T} D(\mathbf{X}) \min\{1, \frac{(1 - 3 \alpha)}{1- \sum_{\mathbf{Y} \in S \cup T \cup \{\mathbf{U}\}}D(\mathbf{Y})}\}\\
% \end{proof}
% Thus the EMD between $D$ and $D_1$ can be expressed as follows:
% \begin{eqnarray*}
% \mbox{EMD}(D,D_1) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^*_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
% &\leq& \sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{{\bf X X}}d_H({\bf X},{\bf X}) +\left( 1-\sum_{\mathbf{X} \notin \{\mathbf{U}'\} \cup S' \cup T'} f^*_{\mathbf{XX}}\right)\\
% &\leq& 0 + 5 \alpha=5\alpha
% \end{eqnarray*}
% This completes the proof of the lemma.


Let us define a distribution $D_2$ over $\{0,1\}^N$ using the following procedure:
\begin{itemize}
    %\item $D_2(\mathbf{U}')=\alpha$;
    %\item There exists a set of vectors $S'=\{\mathbf{V'}_1, \ldots, \mathbf{V'}_b\}$ in $\{0,1\}^N$ such that for every $\mathbf{V'}_i \in S$, $\mathbf{V'}_i$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B'$ and $0$ in all other indices. Moreover, $D_2(\mathbf{V'}_i) = \alpha/b$ for every $i \in [\size{B}]$.
    
    %There exists a set of vectors $S= \{\mathbf{V_1}, \ldots, \mathbf{V_{\size{B}}}\}$ in $\{0,1\}^N$ such that for every $\mathbf{V_i} \in S$, $\mathbf{V_i}$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B$ and $0$ in all other indices. 
    
    %\item There exists a set of vectors $T'= \{\mathbf{W}_0, \ldots, \mathbf{W}_{\lceil \log kn \rceil -1}\}$ (disjoint from $S'$) in $\{0,1\}^N$ such that every vector in $T'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. For every $j \in \{0\} \cup [\lceil \log kn \rceil -1]$, $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$. Moreover, $D_2(\mathbf{W}_i) = \alpha/\lceil \log kn \rceil$ for every $i \in [\size{T'}]$.
    
    %There exists a set of vectors $T= \{\mathbf{W_1}, \ldots, \mathbf{W_{\log n}}\}$ (disjoint from $S$) in $\{0,1\}^N$ such that for each $\mathbf{W_i} \in T$, $\mathbf{W_i}$ has $0$ at the index $i^*$ and the decimal evaluation of $\mathbf{W_i}$ is $i$ when projected to the indices in $B$. Let $N' = [N]\setminus B\cup \{i^*\}$ and $\mathbf{W}_i'=\mathbf{W}_i \mid_{N'}$ for every $i \in [\log n]$ such that for every $j \in N'$, the $j$-th bit of $\mathbf{W}'_i$ is $1$ if and only if $j$ divided by $2^i$ produces an odd number. 
    
     %Consider the set of vectors $\mathcal{V}$  that contains vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$, and let us define the set $\Gamma = \bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$. 

     \item Set $D_2(\mathbf{X})= D_1(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U}$. 
    
    \item Recall that $\Gamma'_{\mathbf{V}}=\{j\in [n]: \mathbf{V}\mid_{C'_j} \ \mbox{is not in the image of} \ \mbox{{\sc SE}}\}$ for every vector $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$. For every vector $\mathbf{V}\in \mathcal{V}^{\mbox{inv}}$, we perform the following steps:

    \begin{itemize}
        \item[(a)] For every $j \notin \Gamma'_{\mathbf{V}}$, decode the vector $\mathbf{V} \mid_{C'_j}$ using $\mbox{{\sc SE}}$ to obtain $\mathbf{x}_j \in \{0,1\}$.

        \item[(b)] For every $j \in \Gamma'_{\mathbf{V}}$, choose an arbitrary value $\mathbf{x}_j$ from $\{0,1\}$.

        \item[(c)] Using $\mathbf{x} = (\mathbf{x}_1, \ldots, \mathbf{x}_n)$ obtained from (a) and (b), construct a new vector $\mathbf{V}'$ for which $\mathbf{V}'_{\pi}=\mbox{{\sc FE}}(\mathbf{z},\mathbf{x})$ for an arbitrary $\mathbf{z} \in [n]^m$, where $\pi$ is the permutation obtained from \findpi in Step (i) of \algadpt.
    \end{itemize}    

    \item For every vector $\mathbf{V} \in \mathcal{V} \setminus \mathcal{V}^{\mbox{inv}}$, set $\mathbf{V}' = \mathbf{V}$.

    \item Finally define $D_2(\mathbf{W})=\sum_{\mathbf{V}: \mathbf{V'} =\mathbf{W}} D_1(\mathbf{V})$ for every $\mathbf{W} \in \mathcal{V}$.

\end{itemize}
  


    %For every $\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}$ and $j \in \Gamma'_{\mathbf{V}}$, replace $\mathbf{V} \mid_{C'_j}$ with an arbitrary valid encoding, that is, an element of $\mathcal{E}(0) \cup \mathcal{E}(1)$.  For every vector $\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}$, let $\mathbf{V}'$ be the vector that we obtain after the above replacement. Now define $D_2(\mathbf{W})=\sum_{\mathbf{V}: \mathbf{V'} =\mathbf{W}} D_1(\mathbf{V})$ for every $\mathbf{W} \in \mathcal{V}^{\mbox{invalid}}$.

    
    %and $\mathbf{v} \in \Gamma'_{\mathbf{v}}$, replace $\mathbf{v}$ with another vector $\mathbf{v}' \in \{0,1\}^{n}$ that is a valid encoding of either $0$ or $1$ (arbitrarily chosen) with respect to the code ensemble $\cE$.  
    %$D_2(\mathbf{V}')=D_1(\mathbf{V})$ for every $\mathbf{V} \in \mathcal{V}$.


Now we prove that the distributions $D_1$ and $D_2$ are not far in Earth Mover Distance.

\begin{lem}\label{lem:d1d2emd}
The Earth Mover Distance between $D_1$ and $D_2$ is at most $\eps/8$.
\end{lem}

\begin{proof}
Recall that the EMD between $D_1$ and $D_2$ is the solution to the following LP:
\begin{eqnarray*}
    &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
    &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_1(\mathbf{X})~\forall \ \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
    \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_2(\mathbf{Y})~\forall \ \mathbf{Y} \in \{0,1\}^N.
\end{eqnarray*}

Consider the flow $f^*$ such that $f^*_{\mathbf{XX}}=D_1(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U} \cup (\mathcal{V} \setminus \mathcal{V}^{\mbox{inv}})$, $f^*_{\mathbf{VV'}}=D_1(\mathbf{V})$ for every $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$, and $f^*_{\mathbf{X}\mathbf{Y}}=0$ for all other vectors. Then we have the following:
\begin{eqnarray*}
\mbox{EMD}(D_1,D_2) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^*_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
&\leq& \sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}^{\mbox{inv}}} f^*_{{\bf X X}}d_H({\bf X},{\bf X}) + \sum_{{\bf V} \in \mathcal{V}^{\mbox{inv}}} f^*_{{\bf V} {\bf V}'}d_H({\bf V},{\bf V'})\\
&\leq& 0 + \sum_{\mathbf{V}\in \mathcal{V}^{\mbox{inv}}}D_1(\mathbf{V})d_H({\bf V},{\bf V'}) 
\end{eqnarray*}

To bound the second term of the last expression, note that $\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{inv}}}D_1(\mathbf{V})d_H({\bf V},{\bf V'}) \leq D_1(\mathcal{V}^{\mbox{inv}}) \leq \eps/8$. This follows from Lemma~\ref{obs:massnonenc}. Thus, we conclude that $EMD(D_1,D_2) \leq \eps/8$, completing the proof of the lemma.
\end{proof}

%$D_1({\bf x})=0$ for each ${\bf x} \in \{\mathbf{U}\} \cup S \cup T$, and $D_1({\bf x})=\frac{D(\bf x)}{1-\sum_{{\bf y} \in \{\mathbf{U}\} \cup S \cup T}D({\bf y})}$ for each ${\bf x} \notin \{\mathbf{U}\} \cup S \cup T$. Note that the Earth Mover distance between $D$ and $D_1$ is at most $3 \alpha$. Since $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, using the triangle inequality, we can say that $D_1$ is $\frac{9\eps}{10}$-far from $\cP_{\mbox{Gap}}$.


%Now construct a distribution $D_1'$ over $\{0,1\}^n$ by projecting the support vectors of $D_1$ onto the set of indices $N' = [N] \setminus B \cup \{i^*\}$. Note that we can assume that we are decoding samples the {\sc Supp-Est} algorithm $\cA$.

Now we have the following observation regarding the rejection probabilities of \algadpt for the distributions $D_1$ and $D_2$.

\begin{obs}
The probability that the tester \algadpt outputs {\sc Reject} in Step (iv) when the input distribution is $D_1$ is at least as large as the probability that \algadpt outputs {\sc Reject} in Step (iv) when the input distribution is $D_2$.
%Let $Q$ be the set of indices queried by the algorithm {\sc Alg-Adaptive} in Step (iv). Then {\sc Alg-Adaptive} is oblivious to $D_1$ and $D_2$ with respect to $Q$.
\end{obs}

\begin{proof}
Note that in the distribution $D_1$, there can be some vectors in $\mbox{Supp}(D_1)$ that are not valid encodings with respect to the function $\mbox{{\sc FE}}$. Thus during execution, the tester \algadpt can {\sc Reject} $D_1$ by Condition (ii) and Condition (iv) (b). However, by the construction of $D_2$ from $D_1$, we have replaced the invalid encoding vectors with valid encoding vectors. Thus, the only difference it makes here is that \algadpt may eventually accept a sample from $D_2$ when encountering such a place where a sample from $D_1$ would have been immediately rejected by Condition (ii) or Condition (iv) (b). Other than this difference, the distributions $D_1$ and $D_2$ are identical. So, the probability that \algadpt outputs {\sc Reject} $D_1$ is at least as large as the probability that it {\sc Rejects} $D_2$.
\end{proof}

%Consider the case when the input distribution is $D_1$ to \algadpt. Note that \algadpt can {\sc Reject} $D_1$ immediately in Step (ii), which is not the case when $D_2$ is the input distribution to \algadpt.

%First note that the structure of the set of vectors $\{\mathbf{U}\} \cup S \cup T$ is identical for both the distributions $D_1$ and $D_2$. Thus, the algorithm {\sc Alg-Adaptive} can not distinguish between $D_1$ and $D_2$ in Phase $1$.

%Consider the case when  \algadpt proceeds to Step (iv). This implies that, \algadpt has not output {\sc Reject} for the input distribution till now. Assume that {\sc Supp-Est} queries for the set of indices $Q$ in Step (iv). 

%Consider a fixed set of random bits $\mathcal{R}$ to be used by \algadpt. Now let us take a distribution $D^{R}$ which is either $D_1$ or $D_2$ with equal probability. Since we have replaced every vector in $\mathcal{V}$ with a corresponding correct encoding while constructing $D_2$, the output of \algadpt with $\mathcal{R}$ as the random bits used during its execution will remain invariant whether $D^R = D_1$ or $D^R = D_2$.
%For a fixed set of random bits used by {\sc Alg-Adaptive}, if the input distribution is either $D_1$ or $D_2$, {\sc Alg-Adaptive} will output the same answer for both of them.


%For every vector $\mathbf{x}\in \{0,1\}^{n}$ and $\mathbf{z} \in [n]^m$, let $\mbox{{\sc FE}}(\mathbf{z}, \mathbf{x}) \subset \{0,1\}^N$ be the set of vectors that are valid encodings with respect to $\mbox{{\sc FE}},i^*,B'$ and $\pi$. 

Let us now define a distribution $D_2^{dec}$ over $\{0,1\}^{n}$ as follows:
\begin{equation}\label{def:enc-dist}
    D_2^{dec}(\mathbf{x})=\frac{1}{1-3\alpha}\sum_{\substack{\mathbf{Y}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}} D_2(\mathbf{Y}) = \frac{1}{1-3\alpha}\sum_{\mathbf{z}\in [n]^m}D_2(\mathrm{FE}(\mathbf{z},\mathbf{x})_{\pi^{-1}}).
\end{equation}


\begin{lem}
The distribution $D_2^{dec}$ is $\eps/3$-far from having support size at most $n$.
\end{lem}

\begin{proof}
Recall that the input distribution $D$ is $\eps$-far from the property $\cP_{\mbox{Gap}}$. Then, by Lemma~\ref{lem:dd1emd}, we know that $d_{EM}(D,D_1) \leq 6 \alpha$. Thus, the distribution $D_1$ is $(\eps - 6 \alpha)$-far from $\cP_{\mbox{Gap}}$.

By Lemma~\ref{lem:d1d2emd}, we know that $d_{EM}(D_1,D_2) \leq \eps/8$. This implies that the distribution $D_2$ is $(\eps - 6\alpha - \eps/8) \geq 2\eps/3$-far from $\cP_{\mbox{Gap}}$. Now we will prove that $D_2^{dec}$ is $\eps/3$-far from having support size at most $n$.

\textcolor{red}{Let us prove this by contradiction. Assume that $D_2^{dec}$ is $\eps/3$-close to having support size at most $n$. Let $D_{3}$ be a distribution over $\{0,1\}^{n}$ having support size at most $n$ such that the Earth Mover Distance between $D_3$ and $D_2^{dec}$ is at most $\eps/3$.
Given the distribution $D_{3}$ over $\{0,1\}^{n}$, and the flow $f'_{\mathbf{x}\mathbf{y}}$ from $D_3$ to $D_2^{dec}$ realizing this distance, let us consider the distribution $D_3^{enc}$ over $\{0,1\}^N$ such that for any $\mathbf{X} \in \mathcal{V}$, for which $\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x})$ for some $\mathbf{z} \in [n]^m$, we have $D_3^{enc}(\mathbf{X})=\sum\limits_{\mathbf{y} \in \{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}$, and for every $\mathbf{X} \in \mathcal{U}$, $D_3^{enc}(\mathbf{X}) = D_2(\mathbf{X})$.}

%$D_3^{enc}(\mathbf{X})=D_3(\mathbf{x}) \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}$

%Given the distribution $D_{3}$ over $\{0,1\}^{n}$, let us consider the distribution $D_3^{enc}$ over $\{0,1\}^N$ such that for every $\mathbf{x} \in \{0,1\}^{n}$, $D_3^{enc}(\mathbf{X})=  (1 - 3 \alpha) D_{3}(\mathbf{x})$ with $\mathbf{X} = \cE(\mathbf{x})$, and $D_3^{enc}(\mathbf{X})= D_2(\mathbf{X})$ for every $\mathbf{X} \in \{\mathbf{U}'\} \cup S' \cup T'$.

%obtained by encoding the support vectors of $D_{*}$ using $\cE$ , as well as including the vectors in the set $\{\mathbf{U}\} \cup S \cup T$ from the support of the distribution $D_2$.

\begin{cl}\label{cl:emd-far}
Let $D_3^{enc}$ be the distribution over $\{0,1\}^N$ obtained from $D_3$. Then the EMD between $D_{3}^{enc}$ and $D_2$ is at most $\eps/3$.
\end{cl}

\begin{proof}

\color{blue}

Recall that the EMD between $D_3^{enc}$ and $D_2$ is the solution to the following LP:
\begin{eqnarray*}
    &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
    &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_3^{enc}(\mathbf{X})~\forall \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
    \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_2(\mathbf{Y})~\forall \mathbf{Y} \in \{0,1\}^N.
\end{eqnarray*}

Let $f'_{\mathbf{x} \mathbf{y}}$ be the flow realizing the EMD between $D_3$ and $D_2^{dec}$. Using $f'$, we now construct a new flow $f^\star$ between $D_3^{enc}$ and $D_2$ as follows:

\begin{itemize}
    \item[(1)]  For vectors $\mathbf{X}, \mathbf{Y} \in \mathcal{U}$,
    
\begin{itemize}
    \item[(i)] If $\mathbf{X} \neq \mathbf{Y}$, then set $f^\star_{\mathbf{X} \mathbf{Y}}=0$. 

    \item[(ii)] If $\mathbf{X} = \mathbf{Y}$, then set $f^\star_{\mathbf{X} \mathbf{Y}} = D_3^{enc}(\mathbf{X})=D_2(\mathbf{Y})$.
    \end{itemize}
    
    \item[(2)] For two vectors $\mathbf{X}, \mathbf{Y} \in \mathcal{V}$, we take the vectors $\mathbf{x}, \mathbf{y} \in \{0,1\}^n$ such that $\mathbf{X}, \mathbf{Y} \in \{0,1\}^N$ are their
valid encodings (by construction such vectors $\mathbf{x}, \mathbf{y}$ exist), and vectors $\mathbf{z}_1,\mathbf{z}_2$ such that $\mathbf{X}=\fen(\mathbf{z}_1,\mathbf{x})$ and $\mathbf{Y}=\fen(\mathbf{z}_2, \mathbf{y})$. Now we set the flow as follows:
\begin{itemize}
    \item[(i)] If $\mathbf{z}_1 \neq \mathbf{z}_2$, then set $f^\star_{\mathbf{X} \mathbf{Y}} = 0$.

    \item[(ii)] If $\mathbf{z}_1 = \mathbf{z}_2$, then set $f^\star_{\mathbf{X} \mathbf{Y}} =  f'_{\mathbf{x} \mathbf{y}} \cdot \frac{D_2(\mathbf{Y})}{D_2^{dec}(\mathbf{y})}$.
\end{itemize}

\item[(3)] If one of $\mathbf{X}$ and $\mathbf{Y}$ is in $\mathcal{U}$ and the other one is in $\mathcal{V}$, then $f^\star_{\mathbf{X}\mathbf{Y}}=0$.

\end{itemize}


We first argue that the flow $f^*_{\mathbf{X} \mathbf{Y}}$ constructed as above is indeed a valid flow, that is, we have:
$(i) \sum\limits_{\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}} = D_3^{enc}(\mathbf{X})$, and $(ii) \sum\limits_{\mathbf{X} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}} = D_2(\mathbf{Y})$. 

%We prove the first one and omit the other similar proof.

To prove $\sum\limits_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X} \mathbf{Y}} = D_3^{enc}(\mathbf{X})$, first observe that it holds when $\mathbf{X} \in \mathcal{U}$ from (1) and (3) in the description of $f^{\star}_{\mathbf{X} \mathbf{Y}}$. Now consider when $\mathbf{X} \in \mathcal{V}$. Assume $\mathbf{X}_{\pi}=\fen\left(\mathbf{z},\mathbf{x}\right)$, where $\mathbf{z} \in [n]^m$ and $\mathbf{x} \in \{0,1\}^n$. So, from (2) in the description of $f^\star_{\mathbf{X}\mathbf{Y}}$, we have
$$\sum\limits_{\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}}=\sum\limits_{\mathbf{y} \in \{0,1\}^n} f^\star_{\mathbf{X} \mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}}} = \sum_{\mathbf{y}\in\{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}=
D_3^{enc}(\mathbf{X}).$$

%\sum\limits_{\mathbf{y} \in \{0,1\}^n}f'_{\mathbf{x} \mathbf{y}} \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}=D_3(\mathbf{x})\cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}= 

%\remove{For example, for $Y \in \mathcal{U}$ it is (by the construction above) quite clear that $\sum_X f_{XY} = f_{YY} = D_2(Y)$, and for $Y=FE(z,y)$ for some $z,y$ (which is the only other non-zero option) we have $\sum_X f_{XY} = \sum_{z',x} f_{FE(z',x),Y} = \sum_x f_{FE(z,x),Y}= \sum_x f'_{xy} \cdot \frac{D_2(Y)}{D_2^{dec}(y)} = D_2(Y)$.}

For (ii), consider $\mathbf{Y}_{\pi} = \mathrm{FE}(\mathbf{z}, \mathbf{y})$ for some $\mathbf{z} \in [n]^m$. Then we have the following:
$$\sum_{\mathbf{X}\in\{0,1\}^N}f_{\mathbf{X}\mathbf{Y}}^{\star}=\sum_{\mathbf{x}\in\{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}=D_2^{dec}(\mathbf{y})\frac{D_2(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2^{dec}(\mathbf{y})}=D_2(\mathbf{Y}).$$

In the above, we have used the fact that $f'_{\mathbf{x} \mathbf{y}}$ is a valid flow from $D_3$ to $D_2^{dec}$.\\

Now, to bound EMD between $D_3^{enc}$ and $D_2$, let us bound the sum $\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})$.
%From (1) and (3) in the description of $f^\star$, $\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})=\sum\limits_{\mathbf{X},\mathbf{Y} \in \mathcal{V}} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y}).$
\begin{eqnarray*}
&&\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})\\
&=&\sum\limits_{\mathbf{X},\mathbf{Y} \in \mathcal{V}} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})~~~\left(\mbox{From (1) and (3) in the description of $f^\star$}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f^\star_{\mathbf{\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}}\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}}}\cdot d_H({\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}},\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})\\ &&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\left(\mbox{From (2) in the description of $f^\star$}\right)\\
&\leq&\sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f^\star_{\mathbf{\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}}\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}}}\cdot d_H(\mathbf{x},\mathbf{y})~~~\left(\mbox{Observation~\ref{obs:FEproperties} (iii)}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f'_{\mathbf{x}\mathbf{y}}\frac{D_2(\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2(\mathbf{y})}\cdot d_H(\mathbf{x},\mathbf{y})~~~\left(\mbox{From (2) in the description of $f^\star$}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\left(f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y})\cdot  \sum\limits_{\mathbf{z}\in [n]^m} \frac{D_2(\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_2(\mathbf{y})}\right)\\
&=& (1-3\alpha) \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n} f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y})~~~(\mbox{By Equation}~\eqref{def:enc-dist})\\
&\leq& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n} f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y}) \leq \frac{\eps}{3}.
\end{eqnarray*}
The last inequality follows from the fact that $f'$ realizes the EMD between $D_3$ and $D^{dec}_2$.
\end{proof}

\color{black}

% \remove{As before, we will bound the Earth Mover Distance between $D_3^{enc}$ and $D_2$ in terms of their variation distance.
% \begin{eqnarray}
%     EMD(D_{3}^{enc}, D_2) &\leq& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| \nonumber \\ &=& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| + \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{U}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| \label{eqn:emdd3encd2}
% \end{eqnarray}

% As $D_3^{enc}(\mathbf{X}) = D_2(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U}$, the second term in the above equation is $0$. Now let us bound the first term. Since for every $\mathbf{X} \in \mathcal{V}$,
% $D_3^{enc}(\mathbf{X})=(1-3\alpha)D_3(\mathbf{x}) \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}$, we can deduce the following:
% \begin{eqnarray*}
% \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| &=& \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}} |(1-3\alpha)D_3(\mathbf{x})\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}-D_2(\mathbf{X})| \\
% &\leq& 3\alpha \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}}\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}D_3(\mathbf{x}) + \\ && \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}}\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}|D_3(\mathbf{x})-D_2^{dec}(\mathbf{x})| \\
% &=&3\alpha + \sum_{\mathbf{x}\in Supp(D_2^{dec})}|D_3(\mathbf{x})-D_2^{dec}(\mathbf{x})| \\
% &\leq& 3\alpha+\frac{2\eps}{3} \leq \eps
% \end{eqnarray*}
% }
% \begin{eqnarray*}
%     \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| &=& \sum_{\mathbf{X} \in \mathcal{V}}|(1-3\alpha)D_{3}(\mathbf{x}) \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} - D_2(\mathbf{X})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} |(1-3\alpha)\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} -1| \\ &\leq & \sum_{\mathbf{X} \in \mathcal{V}} D_2(\mathbf{X}) |\frac{D_3(\mathbf{x}) - D_2^{dec}(\mathbf{x})}{D_2^{dec}(\mathbf{x})}| \\ &\leq& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} \cdot \frac{\eps}{3} \leq \frac{2 \eps}{3}
% \end{eqnarray*}

%Substituting this value in Equation~\ref{eqn:emdd3encd2}, we have the result.


% Let $f^{(1)}$ be the flow from $D_2^{dec}$ to $D_3$ realizing the EMD between $D_2^{dec}$ and $D_3$. Let us consider the flow $f^{(2)}$ from $D_2$ to $D_{3}^{enc}$ as described below:
% \begin{itemize}
%     \item $f^{(2)}_{\mathbf{X}\mathbf{X}}=D_2(\mathbf{X})=D_{3}^{enc}(\mathbf{X})$ for each $\mathbf{X} \in \{\mathbf{U}'\}\cup S' \cup T'$.
    
%     \item For every $\mathbf{x},\mathbf{y} \in \{0,1\}^{n}$, 
% $f^{(2)}_{\mathbf{XY}} = (1-3\alpha)f^{(1)}_{\mathbf{xy}}$, where $\mathbf{X}= \cE(\mathbf{x})$ and $\mathbf{Y}= \cE(\mathbf{y})$.

%       \item Otherwise, $f^{(2)}_{\mathbf{XY}}=0$.
% \end{itemize}

% Now we have the following observation which directly follows from the encoding procedure.
% \begin{obs}
% For any $\mathbf{x, y}\in \{0,1\}^{n}$, the Hamming distance between their encoding is at most the Hamming distance between them.
% \end{obs}
% Thus we have the following:
% \begin{eqnarray*}
% \mbox{EMD}(D_{3}^{enc},D_2) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^{(2)}_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
% &\leq& \sum_{\mathbf{X} \in \{\mathbf{U}'\} \cup S' \cup T' } f^{(2)}_{{\bf X X}}d_H({\bf X},{\bf X}) + \sum_{\mathbf{x,y}\in \{0,1\}^{n}} f^{(2)}_{{\bf \cE(\mathbf{x})\cE(\mathbf{y})}} d_H(\cE(\mathbf{x}),\cE(\mathbf{y}))\\
% &\leq& 0+ \sum_{\mathbf{x,y}\in \{0,1\}^{n}} f^{(1)}_{\mathbf{x}\mathbf{y}} d_H(\mathbf{x},\mathbf{y})\\
% &=& EMD(D_3,D_2^{dec})\leq \eps/3.
% \end{eqnarray*}
% \end{proof}


Since the distribution $D_{3}$ over $\{0,1\}^{n}$ has support size at most $n$, following the encoding procedure, we can say that $D_3^{enc} \in \cP_{\mbox{Gap}}$. But this would contradict the fact that $D_2$ is $2\eps/3$-far from $\cP_{\mbox{Gap}}$. This completes the proof of the lemma.
\end{proof}

Combining the arguments above, we conclude that if the input distribution $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, the tester \algadpt will output {\sc Reject} with probability at least $2/3$.



==> name1.tex <==
\subsection{Determining the permutation $\pi$}\label{sec:quadratic_determine_permutation}

%\comments{
Here we design an algorithm that, given a distribution $D \in \cP_{\mbox{Gap}}$, can learn the permutation $\pi$ for which $D_{\pi} \in P^0_{\mbox{Gap}}$ with high probability. 

The crux of the algorithm is that if $D \in \cP_{\mbox{Gap}}$, then there exist $\mathbf{U}'=\mathbf{U}_\pi \in \{0,1\}^n$, $\cS'=\{\mathbf{\mathbf{V}}_i'=(\mathbf{V}_i)_\pi: i \in [b]\}$ and $\cT'=\{\mathbf{W}_j'=(\mathbf{W}_j)_\pi:j \in \{0\}\cup [\lceil \log kn\rceil]-1\}$ in the support of $D$ such that $D(\mathbf{U}')=\alpha$, $D(\mathbf{V}_i')=\alpha/b$ for every $i \in [b]$ and  $D(\mathbf{W}_j')=\alpha/\lceil \log kn\rceil$. \comments{Note that $\mathbf{U},\mathbf{V}_i$'s and $\mathbf{V}_j$'s are as defined in the property $\cP_{\mbox{Gap}}^0$}. The main observation is that, if we are given the set of special vectors $\{\mathbf{U'}\} \cup \cS' \cup \cT'$, then we can determine the permutation $\pi$. Our algorithm can find  $\mathbf{U}', \cS'$ and $\cT'$ with high probability, if they exist, by taking $\Oh(\log^2 N/\alpha)=\Oh(\log^2 n/\alpha)$ samples and reading them in their entirety. This is due to the fact that the probability mass of every vector in the set of special vectors is at least $\Omega(\alpha/\log n)$.

%}

The algorithm is described in the following subroutine \findpi (see Algorithm~\ref{algo:perm})~\footnote{This algorithm is not adaptive in itself, but its output is used adaptively in the testing algorithm described later.}.

\begin{algorithm}[H]\label{algo:perm}
%\scriptsize

\SetAlgoLined

\caption{\findpi}
\label{alg:findpi}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^N$.}
\KwOut{Either a permutation $\pi:[N] \rightarrow [N]$, or {\sc Fail}.}
\LinesNumbered
\begin{description}
     \item[(i)] First take a multi-set $\cX$ of $\Oh(\log^2 N/\alpha)$ samples from $D$, and query all the entries of the sampled vectors of $\cX$ to know the vectors of $\cX$ completely.
    
    
    \item[(ii)] Find the set of distinct vectors in $\cX$ that have exactly one $1$. If no such vector exists or there is more than one such vector, {\sc Fail}. Otherwise, denote by $\mathbf{U'}$ the vector that has exactly one $1$, and denote the corresponding index by $i^*$. Set $\pi(i^*)=1$, and proceed to the next step.    
    %let the vector be $\mathbf{U'}$ that has $1$ at the index $i^*$. 
    

    \item[(iii)] Find the set of distinct vectors $\cS' \subseteq \cX \setminus \{\mathbf{U'}\}$ such that every vector in $\cS'$ has $1$ at the index $i^*$ and has at least another $1$ among other indices. If no such vector exists, or $\size{\cS'} \neq b$, {\sc Fail}. Otherwise, if the vectors of $\cS'$ form a chain $\mathbf{V}'_1, \ldots, \mathbf{V}'_b$, where $\mathbf{V}'_j$ has exactly $j+1$ many $1$, then set $\pi(i_j)=j+1$, where $i_j$ is the index where $\mathbf{V}'_j$ has $1$, but $\mathbf{V}'_{j-1}$ has $0$ there, for every $j \in [b]$ (denoting $\mathbf{V'}_0=\mathbf{U'}$ for the purpose here). Also, set $B'=(i_1, \ldots,i_b)$. If $\cS'$ does not form a chain $\mathbf{V}'_1, \ldots, \mathbf{V}'_b$ as mentioned above, {\sc Fail}.
    
    
    \item[(iv)] Let $\cT' \subseteq \cX$ be the set of distinct vectors such that every vector in $\cT'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. If no such vector exists, {\sc Fail}. For every $j$, denote by $\mathbf{W}'_j$ the vector in $\cT'$ for which $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$. For every $j \in \{0\} \cup [\lceil \log kn \rceil -1]$, if either there are no vectors $\mathbf{W}'_j \in \cT'$ or there is more than one distinct vector with $\mathbf{W'_j} \mid_{B'}=b(j)$, {\sc Fail}.
    Also, if there is any vector in $\mathbf{W}'_j \in \cT'$ such that $\mathbf{W}'_j \mid_{B'} = b(j)$ for $\log kn \leq j < 2^b -1$, {\sc Fail}.
    
    \item[(v)] For any $i \in [N]\setminus (\{i^*\} \cup B')$, let $l_i$ be the integer with binary representation $(\mathbf{W'}_0)_i, \ldots, (\mathbf{W'}_{\lceil \log kn \rceil -1})_i$.
Set $\pi(i)=b+2+l_i$ for every $i \in [N]\setminus (\{i^*\} \cup B')$. If $\pi$ is not a permutation of $[N]$, {\sc Fail}.

    \item[(vi)] Take another multi-set $\cX'$ of $\Oh(\log^2 N/\alpha)$ samples from $D$, and query all the entries of the sampled vectors of $\cX'$ to know the vectors of $\cX'$ completely. Let $\cY$ be a set of vectors in $\cX'$ such that $\cY=\{\mathbf{Z} \in \cX': \mathbf{Z} \mid_{{\{i^*\} \cup B'}} \neq \mathbf{0}\mathbf{1}^b \}$. If $\size{\cY}/\size{\cX'} > 4\alpha$, {\sc Fail}. Otherwise, output $\pi$.
    
    %Estimate the fraction of vectors in $X'$ that are in $\{\mathbf{U'}\}\cup S' \cup T'$. If it is less than $4\alpha$. Otherwise, {\sc Fail}.
    
\end{description}

\end{algorithm}

\vspace{10pt}

Let us start by analyzing  the query complexity of \findpi.

\begin{lem}[Query complexity of \findpi]\label{lem:queryfindpi}
The query complexity of the above defined \findpi is $\tOh(N)$.
\end{lem}

\begin{proof}
Note that \findpi takes a multi-set $\cX$ of $\Oh(\log^2 N/\alpha)$ samples from $D$ in Step (i), and queries them completely. So, \findpi performs $\Oh(N \log^2 N/\alpha)$ queries in Step (i). \findpi does not perform any new query in Step (ii), Step (iii), Step (iv) and Step (v). Finally, \findpi takes another multi-set $\cX'$ of $\Oh(\log^2 N/\alpha)$ samples from $D$ and queries them completely, similar to Step (i). Recalling that $\alpha=1/\log n$, the query complexity of \findpi is $\tOh(N)= \tOh(n)$ in total.
\end{proof}


Now we proceed to prove the correctness of \findpi.
\color{blue}
\begin{lem}[Guarantee when $D \in \cP_{\mbox{Gap}}$]\label{lem:findpicompleteness}
If $D$ is a distribution defined over $\{0,1\}^N$ such that $D \in \cP_{\mbox{Gap}}$, then with probability at least $9/10$, \findpi reports permutation $\pi$ such that $D_{\pi} \in \cP_{\mbox{Gap}}^0$.
\end{lem}

We prove the above lemma by a series of intermediate lemmas. \color{black} In the following lemmas, we consider $\mathbf{U}$, $\cS$ and $\cT$ as per the definition of $\cP^0_{\mbox{Gap}}$. Also, consider the permutation $\pi$ such that $D_\pi \in \cP_{\mbox{Gap}}$.
%To argue the completeness of our algorithm, consider a distribution $D$ over $\{0,1\}^N$ such that $D\in \cP_{\mbox{Gap}}$, and let $\pi$ be the permutation for which $D_{\pi} \in \cP^0_{\mbox{Gap}}$. 

%Now consider the following lemma.

%So, there exists the four types of vectors as described in the definition of $\cP_{\mbox{Gap}}$. By using Chernoff bound, we have the following:

\begin{lem}[correctly finding $\pi^{-1}(1)$]\label{lem:hittingU}
With probability at least $1-1/N^3$, $\cX$ will contain the vector $\mathbf{U'}$ for which $\mathbf{U'}_{\pi}=\mathbf{U}$, and $i^*=\pi^{-1}(1)$ will be identified correctly.
\comments{Moreover, \findpi proceeds to Step (iii).}
%Let $\mathbf{U'} \in \{0,1\}^N$ be a vector that has exactly a single $1$ at some index $i^*$, and $D$ be a distribution over $\{0,1\}^N$ such that $D(\mathbf{U'})= \alpha$. Consider the multi-set of samples $X$ taken from $D$ in Step (i) of \findpi such that $\size{X} = \Oh(\log^2 N/\alpha)$. Then with probability at least $1 - \frac{1}{N^3}$, $\mathbf{U'} \in X$. 
\end{lem}

\begin{proof}
By the definition of $\cP^0_{\mbox{Gap}}$, the vector $\mathbf{U'}$ is the only vector in the support of $D$ containing a single $1$. Since $D(\mathbf{U'}) = D(\mathbf{U}_{\pi^{-1}(1)}) = \alpha$, and we are taking $\size{\cX}$ many samples from $D$, the probability that $\mathbf{U'}$ will not appear in $\cX$ is at most $(1- \alpha)^{\size{X}} \leq \frac{1}{N^3}$. Thus, with probability at least $1 - \frac{1}{N^3}$, $\mathbf{U'} \in \cX$ and \findpi in Step (ii) proceeds to the next step
%This completes the proof of the lemma.
\end{proof}

\begin{lem}[correctly finding $B' = \pi^{-1}(B)$]\label{lem:hittingS}
With probability at least $1-1/N^3$, the algorithm \findpi will correctly identify $\mathbf{V'}_1, \ldots, \mathbf{V'}_b$ for which $\mathbf{V'}_{i,\pi} = \mathbf{V}_i$, and $B'={\pi^{-1}(2), \ldots, \pi^{-1}(b+1)}$ will be identified correctly as well. \comments{Moreover, \findpi proceeds to Step (iv).}

%Let $S'= \{\mathbf{V}'_1, \ldots, \mathbf{V}'_b\}$ be a set of vectors in $\{0,1\}^N$ such that for each $\mathbf{V}'_i \in S'$, $\mathbf{V}'_i$ has $1$ at some index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B$. Moreover, $D(\mathbf{V}'_i) = \alpha/b$ for each $i \in [b]$. Then with probability at least $1 - \frac{1}{N^3}$, $S' \subseteq X$, where $X$ is the multi-set of samples obtained from $D$ and $\size{X}= \Oh(\log^2 N/\alpha)$.
\end{lem}

\begin{proof}
%Let us consider an arbitrary vector $\mathbf{V}'_i \in S'$.

Let $\mathbf{V'}_1, \ldots, \mathbf{V'}_b$ denote the vectors for which $\mathbf{V'}_{i,\pi}=\mathbf{V}_i$ for every $i$. Note that these are the only vectors outside $\mathbf{U'}$ in the support of $D$ that have $1$ at the index $i^*$.
As $D(\mathbf{V}'_i)= \frac{\alpha}{b}$, the probability that $\mathbf{V}'_i$ does not appear in $\cX$ is at most $(1- \frac{\alpha}{b})^{\size{X}}$. Since $\size{\cX} = \Oh(\log^2 N/\alpha)$ and $b = \Oh(\log \log kn)$, the probability that $\mathbf{V}'_i \in \cX$ is at least $1 - \frac{1}{N^4}$. Using the union bound over all the vectors of $\cS'$, with probability at least $1-1/N^3$, we know that all of these vectors are in $\cX$, in which case they are identified correctly, so $B'$ is identified correctly as well, and \findpi in Step (iii) proceeds to the next step.
\end{proof}

\begin{lem}[correctly identifying $\pi^{-1}(b+2), \ldots, \pi^{-1}(N)$]\label{lem:hittingT}
Let $\mathbf{W'}_1, \ldots, \mathbf{W'}_{\lceil \log kn \rceil -1}$ denote the vectors for which $\mathbf{W'}_{j,\pi} = \mathbf{W}_j$ for every $j$. With probability at least $1-1/N^3$, all these vectors appear in $\cX$, in which case they are identified correctly, and so are $\pi^{-1}(b+2), \ldots, \pi^{-1}(N)$. \comments{Moreover, \findpi proceeds to Step (vi).}

%Let $T'= \{\mathbf{W}'_1, \ldots, \mathbf{W}'_{\log kn}\}$ be a set of vectors (disjoint from $S'$) in $\{0,1\}^N$ such that for each $\mathbf{W}'_i \in T'$, $\mathbf{W}'_i$ contains $1$ at the index $i^*$, for every $i \in [\log n]$, the decimal evaluation of $\mathbf{W}'_i \mid_{B'}$ is $i$. Moreover, $D(\mathbf{W}'_i) = \alpha/\log kn$ for each $i \in \{0\} \cup [\log kn -1]$. Then with probability at least $1 - \frac{1}{N^3}$, $T' \subseteq X$, where $X$ is the multi-set of samples obtained from $D$ and $\size{X}= \Oh(\log^2 N/\alpha)$.
\end{lem}

The proof of the above lemma is similar to the proof of Lemma~\ref{lem:hittingS} and is omitted. Note that from Lemma~\ref{lem:hittingU}, Lemma~\ref{lem:hittingS} and Lemma~\ref{lem:hittingT}, we know that with probability at least $1-o(1)$, the algorithm \findpi has correctly determined the permutation $\pi$ and proceeded to Step (vi). We will finish up the proof of Lemma~\ref{lem:findpicompleteness} having the following lemma.

%proceeded to Step (v). Since the vectors in $\{\mathbf{U}\} \cup S \cup T$ are disjoint, \findpi correctly determines the permutation $\pi$ with probability at least $1-o(1)$.

\begin{lem}
The probability that \findpi outputs {\sc Fail} in Step (vi) (instead of outputting $\pi$) is at most $1/N^3$.

%With probability at least $1 - \frac{1}{N^3}$, $\size{\cY}/\size{X'} \leq 4 \alpha$.
%the fraction of vectors in $X'$ that are in $\{\mathbf{U}\} \cup S \cup T$ is at most $4 \alpha$.
\end{lem}

\begin{proof}
As $D \in \cP_{\mbox{Gap}}$, from the description of the property, we know that $D(\{\mathbf{U'}\} \cup \cS' \cup \cT')= 3 \alpha$. As $\size{\cX'}= \Oh(\log^2 N/\alpha)$, using the Chernoff bound, we have the result.
\end{proof}

Combining the above lemmas, we conclude that with probability at least $9/10$, the algorithm \findpi outputs a correct permutation $\pi$, completing the proof of Lemma~\ref{lem:findpicompleteness}.

To conclude this section, we show that with high probability, we will not output $\pi$ for which too much weight is placed outside the ``\emph{encoded part}'' of the distribution.

%Now consider the case when $D(\{\mathbf{U'}\}\cup S' \cup T'\}) \geq 5 \alpha$. Then we can say that \findpi will output {\sc Fail} with high probability.

\begin{lem}\label{lem:findpisumfourthtype}
For any distribution $D$ (regardless of whether $D$ is in $\cP_{\mbox{Gap}}$ or not), the probability that \findpi outputs a permutation $\pi$ for which $D(\{\mathbf{X}:\mathbf{X}_{\{i^*\} \cup B'}=\mathbf{0}\mathbf{1}^b\}) \leq 1-5\alpha$ is at most $1/10$.

%Consider any distribution $D$ over $\{0,1\}^N$ such that $D(\{\mathbf{U'}\}\cup S' \cup T'\}) \geq 5 \alpha$. Then with probability at most $1/10$, \findpi outputs a permutation $\pi$.
\end{lem}

\begin{proof}
Recall the set of vectors $\cY$ as defined in Step (vi) of \findpi: $\cY=\{\mathbf{Z} \in \cX': \mathbf{Z} \mid_{{{i^*} \cup B'}} \neq \mathbf{0}\mathbf{1}^b \}$, where $\cX'$ is the multi-set of (new) samples obtained in Step (vi) of \findpi. Consider a distribution $D$ such that $D(\{\mathbf{X}:\mathbf{X}_{\{i^*\} \cup B'}=\mathbf{0}\mathbf{1}^b\}) \leq 1-5\alpha$. This implies that $\E\left[\size{\cY}/\size{\cX'}\right] \geq 5 \alpha$. As $\size{\cX'} = \Oh(\log^2 N/\alpha)$, using the Chernoff bound, we obtain that with probability at least $9/10$, the algorithm \findpi outputs {\sc Fail} in Step (vi), and does not output any permutation $\pi$. This completes the proof.
\end{proof}

\subsection{The upper bound on adaptive testing for property $\cP_{\mbox{Gap}}$}\label{sec:quadratic_adaptive_ub}

In this subsection, we design the adaptive tester for the property $\cP_{\mbox{Gap}}$. Given a distribution $D$ over $\{0,1\}^N$, with high probability, \algadpt outputs {\sc Accept} when $D \in \cP_{\mbox{Gap}}$, and outputs {\sc Reject} when $D$ is far from $\cP_{\mbox{Gap}}$. The formal adaptive algorithm is presented in \algadpt (see Algorithm~\ref{algo:adaptive}). Note that it has only two adaptive steps.

%\comments{

In the first adaptive step, our tester \algadpt starts by calling the algorithm \findpi (as described in Subsection~\ref{sec:quadratic_determine_permutation}) whose  query complexity is $\tOh(n)$. If $D \in \cP_{\mbox{Gap}}$, with high probability, \findpi returns the permutation $\pi$ such that $D_{\pi} \in \cP_{\mbox{Gap}}^0$. Once $\pi$ is known, when we obtain a sample $\mathbf{X}$ from $D$, we can consider it as $\mathbf{X}_\pi$ from $D_{\pi}$. Also, from the structure of the vectors in the support of the distributions in $P^0_{\mbox{Gap}}$, we can decide whether $X_{\pi}$ is a special vector, that is, $X_{\pi} \in \{\mathbf{U}\} \cup \cS \cup \cT$ or $\mathbf{X}_\pi$ is an encoding vector, that is, $\mathbf{X}_\pi=\fen(\mathbf{z},\mathbf{x})$ for some $\mathbf{z}\in [n]^m$ and $\mathbf{x} \in \{0,1\}^n$. Observe that, in the later case, we can decode any bit of $\mathbf{x}$ (say $\mathbf{x}_j$) by finding $\mathbf{X}_\pi$ projected into $C_j$, which can be done by performing $\Oh(\log n)$ queries.

%} 

%\comments{
As the second adaptive step, our algorithm asks for a sequence $\cY$ of $\Oh(n/\eps)$ samples from $D$, that is, from $D_{\pi}$. Let $\cY'\subseteq \cY$ be the sequence of encoding vectors in $\cY$. We now call {\sc Supp-Est}$(\cY', \eps/3)$ (from Lemma~\ref{pre:suppest}), and depending on its output, \algadpt either reports {\sc Accept} or {\sc Reject}. Note that we can execute every query by {\sc Supp-Est}$(\cY', \eps/3)$, by performing $\Oh(\log n)$ queries to the corresponding sample in $\cY'$ \comments{as discussed towords the end of the above paragraph.}
%}  

\comments{
When $D \in \cP_{\mbox{Gap}}$ (that is, $D_\pi \in \cP_{\mbox{Gap}}^0$ for the permutation $\pi$), the set of encoding vectors in $D_\pi$ is the encoding of at most $n$ vectors in $\{0,1\}^n$. So, in that case, \algadpt reports {\sc Accept} with high probability. Now consider the case, when $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. If \algadpt has not rejected $D$ before calling {\sc Supp-Est}$(\cY', \eps/3)$, we will show that the distribution over $\{0,1\}^n$ induced by the vectors decoded from the encoding vectors in $D_{\pi}$ is ${\eps}/3$-far from having support size $n$. Then, \algadpt will reject $D$ with high probability.
}


\begin{algorithm}[H]\label{algo:adaptive}
%\scriptsize
\SetAlgoLined

\caption{\algadpt}
\label{alg:adaptive}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^N$, and a parameter $\eps \in (0,1)$.}
\KwOut{Either {\sc Accept} or {\sc Reject}.}
\LinesNumbered
\begin{description}
     \item[(i)] Call \findpi. If \findpi returns {\sc Fail}, {\sc Reject}. Otherwise, let $\pi$ be the permutation returned by \findpi. Denote for convenience $i^*=\pi^{-1}(1), B'=\pi^{-1}(B)$, and $C'_j=\pi^{-1}(C_j)$ for every $j \in [n]$.
     
     \item[(ii)] Take a multi-set $\cX$ of $\Oh(1/\eps)$ samples from $D$, and query all the entries of the sampled vectors of $\cX$ to know the vectors of $\cX$ completely. If there is any vector $\mathbf{X}$ for which $\mathbf{X} \mid_{\{i^*\} \cup B'} = \mathbf{0}\mathbf{1}^b$ (according to the permutation $\pi$ obtained from Step (i)) for which $\mathbf{X}_{\pi}$ is not in the image of $\mbox{{\sc FE}}$ (i.e. it is not a valid encoding of any vector in $\{0,1\}^n$), {\sc Reject}. Otherwise, proceed to the next step.
     
     %Construct a sequence of vectors $X' \subseteq X$ such that for every $\mathbf{X} \in X'$, $\mathbf{X} \mid_{\{i^*\}\cup B'} = \mathbf{0}\mathbf{1}^b$ (according to the permutation $\pi$ obtained from Step (i)). If the fraction $\frac{\size{X \setminus X'}}{\size{X}} > \frac{\eps}{10}$
     
     %For every $\mathbf{X} \in X$, query the indices $\{i^*\} \cup B'$ (according to the permutation $\pi$ obtained from Step (i)) to $\mathbf{X}$. 
     %For any $\mathbf{X} \in X$, if $\mathbf{X} \mid_{\{i^*\}\cup B'} = \mathbf{0}\mathbf{1}^b$, then choose a uniformly random $j \in [n]$, and check whether $\mathbf{X} \mid_{C'_j} \in \mathcal{E}(0)\cup\mathcal{E}(1)$, that is, whether it is a valid encoding of some value in $\{0,1\}$. If any invalid encoding is found for any $\mathbf{X} \mid_{C'_j}$, {\sc Reject}.

     %Construct the sequence of vectors $X'$ such that $X' = \{\mathbf{X} \in X: \mathbf{X} \mid_{\{i^*\} \cup B'} = \mathbf{0} \mathbf{1}^b\}$. Now sample a set of indices $\cI \subseteq [n]$ without replacement such that $\size{\cI}=\Oh(1/\eps)$. 
     
     %For every $\mathbf{X} \in X'$, choose a $j \in \cI$  randomly, and  check if $\mathbf{X} \mid_{C'_j}$ is a valid encoding of some vector $\mathbf{x} \in \{0,1\}^n$ with respect to the code ensemble $\cE$ by querying the appropriate indices of $\mathbf{X}$. If $\mathbf{X} \mid_{C'_j}$ is not a valid encoding for some $j \in \cI$, {\sc Reject}.
     
     %where $C_j$ denotes the set of indices of $[N]$ such that $C_j= \{b+2+k(j-1), \ldots, b+1+kj\}$.

    \item[(iii)]Take a sequence of samples $\cY$ such that $\size{\cY}=\Oh(n/\eps)$ from $D$. Now construct the sequence of vectors $\cY'$ such that $\cY'= \{\mathbf{Y} \in \cY: \mathbf{Y} \mid_{\{i^*\} \cup B'} = \mathbf{0} \mathbf{1}^b\}$ by querying the indices corresponding to $\{i^*\} \cup B'$.

    \item[(iv)] Call {\sc Supp-Est}$(\cY', \eps/3)$ (from Lemma~\ref{pre:suppest}), where a query to an index $j$ is simulated by querying the indices of $C'_j$ and decoding the obtained vector with respect to to $\mbox{{\sc SE}}$ (that is, checking whether the restriction of the queried vector to $C'_j$ is equal to $\mbox{{\sc SE}}(i,0)$ for some $i$, or equal to $\mbox{{\sc SE}}(i,1)$ for some i). {\sc Reject} if any of the following conditions hold:
    \begin{itemize}
        \item[(a)] $\size{\cY'}/\size{\cY} \leq 1/2$ (due to the absence of sufficiently many samples in $\cY'$ to apply {\sc Supp-Est}).

        \item[(b)] {\sc Supp-Est}$(\cY', \eps/3)$ queries an index $j$ from some $\comments{\mathbf{Y}_i}$ corresponding to an invalid encoding of $\comments{\mathbf{Y}_i} \mid_{C'_j}$ (that is, when $\comments{\mathbf{Y}_i} \mid_{C'_j}$ is not in the image of $\mbox{{\sc SE}}$).
        
        \item[(c)] {\sc Supp-Est}$(\cY',\eps/3)$ outputs {\sc Reject}.
    \end{itemize}

    Otherwise, {\sc Accept}.

\end{description}

\end{algorithm}

\vspace{10pt}

Let us first discuss the query complexity of \algadpt.

\begin{lem}[Query complexity of \algadpt]
The query complexity of the adaptive tester \algadpt for testing the property $\cP_{\mbox{Gap}}$ is $\tOh(N)= \tOh(n)$.    
\end{lem}

\begin{proof}
Note that \algadpt calls the algorithm \findpi in Step (i). Following the query complexity lemma of \findpi (Lemma~\ref{lem:queryfindpi}), we know that \findpi performs $\tOh(N)$ queries.

For every sample taken in Step (ii), the sampled vectors of the multi-set $\cX$ are queried completely. Since we take $\Oh(1/\eps)$ samples, this step requires $\Oh(N/\eps) = \widetilde{\Oh}(n/\eps)$ queries in total.  
    
%the indices of $\{i^*\}\cup B'$ are queried (taking $b+1=\Oh(\log \log kn/\eps)$ many queries), as well as possibly the indices of some $C'_j$ (taking $k=\Oh(\log n)$ many queries). Since we take $\Oh(1/\eps)$ many samples, this step requires $\Oh(\log n/\eps)$ many queries in total.

%In Step (ii), \algadpt first takes a multi-set of samples $X$ such that $\size{X}= \Oh(1/\eps)$ and then queries the indices of $\{i^*\} \cup B'$ of the vectors of $X$ to obtain $X'$. This procedure requires $\Oh(\log \log kn/ \eps)$ many queries. Also, in the same step, \algadpt tests whether the vectors of $X'$ are valid encodings with respect to the code ensemble $\cE$. This requires $\Oh(\log n/\eps^2)$ many queries.

Then in Step (iii), \algadpt takes a multi-set $\cY$ of $\Oh(n/\eps)$ samples, and queries for the indices in $\{i^*\} \cup B'$ to obtain the vectors in $\cY'$, which takes $\Oh(n \log \log kn/\eps)$ queries. Finally, in Step (iv), \algadpt calls the algorithm {\sc Supp-Est}, which performs $\tOh(n)$ queries (following Lemma~\ref{pre:suppest}), each of them simulated by $\Oh(\log n)$ queries to some $\comments{\mathbf{Y}_i} \mid_{{C'_j}}$. Thus, in total, \algadpt performs $\tOh(N) = \tOh(n)$ queries.
\end{proof}

Now we prove the correctness of \algadpt. We will start with the completeness proof.

\begin{lem}[Completeness]
Let $D$ be a distribution defined over $\{0,1\}^N$. If $D \in \cP_{\mbox{Gap}}$, then the algorithm \algadpt will output {\sc Accept} with probability at least $2/3$.
\end{lem}

\begin{proof}
Consider a distribution $D \in \cP_{\mbox{Gap}}$. From the completeness lemma of \findpi (Lemma~\ref{lem:findpicompleteness}), we infer that with probability at least $9/10$, \findpi returns the correct permutation $\pi$ in Step (i). Then, by the definition of $\cP_{\mbox{Gap}}$, the algorithm \algadpt can never encounter any samples with invalid encodings in Step (ii) which could cause it to {\sc Reject}. Thus, with probability at least $9/10$, the algorithm proceeds, with the correct permutation $\pi$, to Step (iii) and Step (iv).
    
%and no invalid encodings have been encountered. Thus \algadpt proceeds to Step (ii) with the same probability. Since $D \in \cP_{\mbox{Gap}}$, the total mass of the valid encoding vectors of $D$ is $1-3\alpha$. Thus, using the Chernoff bound, we can say that in Step (ii), the fraction of sampled vectors in $X$ that are not in $X'$ is at most $\eps/10$. So, \algadpt successfully completes this step and proceeds to Step (iii) and Step (iv).

As $D \in \cP_{\mbox{Gap}}$, $D(\{\mathbf{U'}\} \cup \cS' \cup \cT') = 3 \alpha$. As $\size{\cY}= \Oh(n/\eps)$, using the Chernoff bound, we can say that, with probability at least $9/10$, $\size{\cY'}/\size{\cY} \geq 1/2$. Moreover, as the vectors in $\cY'$ are valid encodings with respect to the function $\mbox{{\sc FE}}$ of at most $n$ vectors from $[2n]$, following the support estimation upper bound lemma (Lemma~\ref{pre:suppest}), we obtain that {\sc Supp-Est} outputs {\sc Accept} with probability at least $9/10$. Combining these, we conclude that \algadpt outputs {\sc Accept} with probability at least $2/3$.
\end{proof}

Now we prove that when $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, \algadpt will output {\sc Reject} with probability at least $2/3$.

\begin{lem}[Soundness]\label{lem:sound}
    Let $\eps \in (0,1)$ be a proximity parameter. Assume that $D$ is a distribution defined over $\{0,1\}^N$ such that $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. Then \algadpt outputs {\sc Reject} with probability at least $2/3$.
\end{lem}

From the description of \algadpt (Algorithm~\ref{algo:adaptive}), if the tester reports {\sc Reject} before executing all the steps of {{\sc Supp-Est}}$(\cY',\eps/3)$ in Step (iv),  then we are done. So, assume that \algadpt executes all the steps of {{\sc Supp-Est}}$(\cY',\eps/3)$. Let $\cY'$ be the set of samples from distribution $D^{\#}$ over $\{0,1\}^n$. Note that $\dhash$ is unknown and we are accessing $D^{\#}$ indirectly via decoding sample from $D$ over $\{0,1\}^n$. From the correctness {{\sc Supp-Est}}$(\cY',\eps/3)$, we will be done with the proof of Lemma~\ref{lem:sound} by having the following lemma.
\begin{lem}\label{lem:far-D-star}
$D^{\#}$ is $\eps/3$-far from having support $n$. 
\end{lem}
\comments{We prove the above lemma by a series of claims.}
%\begin{proof}
Let $D$ be a distribution which is $\eps$-far from $\cP_{\mbox{Gap}}$, and $\mathcal{V}$ denote the set $\{\mathbf{X} \in \mbox{Supp}(D) : \mathbf{X} \mid_{\{i^*\}\cup B'}=\mathbf{0}\mathbf{1}^b\}$, and let us define $\mathcal{U}= \mbox{Supp}(D) \setminus \mathcal{V}$. Let us start with the following observation.

%If \algadpt outputs {\sc Reject} in either Step (i) or Step (ii), then we are done. Otherwise, let us assume that \algadpt has proceeded to Step (iii) and Step (iv). Now we need to argue that when we call the algorithm {\sc Supp-Est}, it will output {\sc Reject} with probability at least $9/10$.

\begin{obs}\label{obs:sumdothervec}
$D(\mathcal{U}) \leq 5\alpha$, unless the algorithm \algadpt has rejected with probability at least $1-1/N^3$ in Step (i).
%$D(\{\mathbf{U'}\}\cup S' \cup T') \leq 5\alpha$ with probability at least $1- \frac{1}{N^3}$.
\end{obs}

\begin{proof}
Since \algadpt in Step (i) invokes the algorithm \findpi, this follows immediately from Lemma~\ref{lem:findpisumfourthtype}.
%Since \findpi has not output {\sc Fail} for the input distribution $D$ in Step $(vi)$, this implies that the fraction of vectors in $Y'$ that belong to the set $\{\mathbf{U'}\} \cup S' \cup T'$ is at most $4 \alpha$. Since $\size{Y} = \Oh(n/\eps)$, using the Chernoff bound, we can say that with probability at least $1- \frac{1}{N^3}$, $D(\{\mathbf{U'}\} \cup S' \cup T') \leq 5 \alpha$.
\end{proof}

% Thus with probability at least $1- \frac{1}{N^3}$, we can say that: 
% \begin{itemize}

%     \item[(i)] There exists a vector $\mathbf{U}' \in \{0,1\}^N$ that has $0$ at some index $i^*$ and $0$ in all other indices. 
    
%     %Also, $D(\mathbf{U})= \alpha$.
    
%     \item[(ii)] There exists a set of vectors $S'=\{\mathbf{V'}_1, \ldots, \mathbf{V'}_b\}$ in $\{0,1\}^N$ such that for every $\mathbf{V'}_i \in S$, $\mathbf{V'}_i$ has $1$ at the index $i^*$, and exactly $i$ many $1$s in the indices corresponding to $B'$ and $0$ in all other indices. 
    
%     %Moreover, $D(\mathbf{V_i}) = \alpha/\size{B}$ for every $i \in [\size{B}]$.

%     \item[(iii)] There exists a set of vectors $T'= \{\mathbf{W_0}, \ldots, \mathbf{W}_{\lceil \log kn \rceil -1}\}$ (disjoint from $S'$) in $\{0,1\}^N$ such that each vector in $T'$ has $0$ at the index $i^*$, and does not have $1$ in all indices of $B'$. For every $j$, denote by $\mathbf{W}'_j$ the vector in $T'$ for which $\mathbf{W}'_j \mid_{B'} = b(j)$, where $b(j)$ denotes the binary representation of $j$.

%     %for each $\mathbf{W}_i \in T'$, $\mathbf{W}_i$ is of the form $\mathbf{0}(b(i))(\mathbf{0}^{2^i}\mathbf{1}^{2^i})^{kn/2^{i+1}}$, where $b(i)$ denotes the binary representation of $i$.
%     %for each $\mathbf{W_i} \in T$, $\mathbf{W_i}$ has $0$ at the index $i^*$ and the decimal evaluation of $\mathbf{W_i}$ is $i$ when projected to the indices in $B$. Let $N' = [N]\setminus B\cup \{i^*\}$ and $\mathbf{W}_i'=\mathbf{W}_i \mid_{N'}$ for every $i \in [\log n]$ such that for every $j \in N'$, the $j$-th bit of $\mathbf{W}'_i$ is $1$ if and only if $j$ divided by $2^i$ produces an odd number. 
    
%     %Moreover, $D(\mathbf{W_i}) = \alpha/\log n$ for every $i \in [\log n]$.
%     \item[(iv)] $D(\{\mathbf{U}'\}\cup S' \cup T') \leq 5\alpha$.
    
%     \item[(v)] Let $\pi$ be the permutation obtained from \findpi. Let $\mathcal{V}$ be the set of vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$. For each vector $\mathbf{V} \in \mathcal{V}$, consider a set of $\Gamma_{\mathbf{V}}=\{\mathbf{v_1,\ldots,\mathbf{v}_{n}}\}$ of $n$ vectors in $\{0,1\}^{n}$, such that
%     the $j$-th index of $\mathbf{v}_i$ has the same value present in the $\{\pi((i-1)\lceil \log kn \rceil +j)$-th index of $\mathbf{V}$. Let $\Gamma'_{\mathbf{V}} \subseteq \Gamma_{\mathbf{V}}$ be the set of vectors that are not valid encoding with respect to $\cE$. Let $\Gamma=\bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$.
    
%     %Then $\sum_{\mathbf{V}\in \mathcal{V}} D(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \alpha$.
    
    
%    % $\mathbf{V}$ is not an encoding with respect to $\cE$. Then $D(\mathcal{V})\leq \alpha$.
%     %and the remaining set of indices are code ensemble of vectors in $\{0,1\}^{n/\log n}$.
    
% \end{itemize}

%Let $\mathcal{V}$ be the set of vectors in the support of $D$ that are not in $\{\mathbf{U}'\} \cup S' \cup T'$. For each vector $\mathbf{V} \in \mathcal{V}$, consider a set of $\Gamma_{\mathbf{V}}=\{\mathbf{v_1,\ldots,\mathbf{v}_{n}}\}$ of $n$ vectors in $\{0,1\}^{n}$, such that the $j$-th index of $\mathbf{v}_i$ has the same value present in the $\{\pi((i-1)\lceil \log kn \rceil +j)$-th index of $\mathbf{V}$, where $\pi$ is the permutation returned by \findpi. Let $\Gamma'_{\mathbf{V}} \subseteq \Gamma_{\mathbf{V}}$ be the set of vectors that are not valid encodings with respect to $\cE$. Let $\Gamma=\bigcup\limits_{\mathbf{V} \in \mathcal{V}} \Gamma'_{\mathbf{V}}$ be the set of all such vectors. 


Let $\mathcal{V}^{\mbox{inv}} \subseteq \mathcal{V}$ denote the following set of vectors:
$$\mathcal{V}^{\mbox{inv}} = \{\mathbf{X} \in \mathcal{V}: \mathbf{X} \neq \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \ \mbox{for all} \ \mathbf{z} \in [n]^m, \mathbf{x} \in \{0,1\}^n\}$$

For every vector $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$, let $\Gamma'_{\mathbf{V}}=\{j\in [n]: \mathbf{V}\mid_{C'_j} \ \mbox{is not in the image of} \ \mbox{{\sc SE}}\}$ denotes \comments{the set of indices in $[n]$ of chunks of all the ``\emph{locally invalid}'' encodings} in the vector $\mathbf{V}$~\footnote{Note that it may be the case that $\Gamma'_{\mathbf{V}}=\emptyset$, for example when for every $j \in [n]$, we have $\mathbf{V} \mid_{C'_j} = \mbox{{\sc SE}}(i_j, \mathbf{x}_j)$, for some $i_1, \ldots, i_n$ and $\mathbf{x}_1, \ldots, \mathbf{x}_n$ for which $i_1, \ldots, i_n$ are not in the image of $\mbox{{\sc GE}}$.}.
\begin{obs}\label{obs:v-enc}
$D(\mathcal{V}^{\mbox{inv}}) \leq {\eps}/10$.
\end{obs}
The above observation holds as otherwise, \algadpt would have rejected in Step-(ii).
%Now we have the following lemma.

% \begin{lem}\label{lem:sumencvector}
%     $\sum_{\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}} D(\mathbf{V})\frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \eps/10$, unless \algadpt has rejected with probability at least $2/3$ in Step (ii).
% \end{lem}

% \begin{proof}
% For every $\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}$, the probability that a sample $\mathbf{X}$ taken in Step (ii) is equal to $\mathbf{V}$ is $D(\mathbf{V})$, and then the probability that $\mathbf{V} \mid_{C'_j}$ is an invalid encoding is exactly $|\Gamma'_{\mathbf{V}}|/n$. This implies that for every sample $\mathbf{X} \in X$, the probability that it causes a rejection is exactly $\sum_{\mathbf{V} \in \mathcal{V}^{\mbox{invalid}}}D(\mathbf{V})|\Gamma'_{\mathbf{V}}|/n$.  The lemma follows since we have taken $\Oh(1/\eps)$ many independent samples in Step (ii).

% %Recall that during the execution of the tester \algadpt in Step (ii), \algadpt selects a subset of indices $\cI \subseteq [n]$, and for every $\mathbf{V} \in X'$, chooses an index $j \in \cI$ randomly and checks whether $\mathbf{V} \mid_{C'_j}$ is a valid encoding with respect to $\cE$ or not. As $\Gamma'_{\mathbf{V}}$ is the set of vectors that are not valid encodings of any vector $\mathbf{V}$, the probability that \algadpt \ {\sc Rejects} a fixed vector $\mathbf{V}$ is $\frac{\size{\Gamma'_{\mathbf{V}}}}{n}$. As $\size{\cI} = \Oh(1/\eps)$, applying the Chernoff bound and summing over all vectors $\mathbf{V} \in \mathcal{V}$, we have the result.
% \end{proof}


\vspace{2 pt}
Let us define a distribution $D_1$ over $\{0,1\}^N$ using the following procedure:
\begin{itemize}
     \item Set $D_1(\mathbf{X})= D(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U}$. 
    
    \item Recall that $\Gamma'_{\mathbf{V}}=\{j\in [n]: \mathbf{V}\mid_{C'_j} \ \mbox{is not in the image of} \ \mbox{{\sc SE}}\}$ for every vector $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$. For every vector $\mathbf{V}\in \mathcal{V}^{\mbox{inv}}$, we perform the following steps:

    \begin{itemize}
        \item[(a)] For every $j \notin \Gamma'_{\mathbf{V}}$, decode the vector $\mathbf{V} \mid_{C'_j}$ using $\mbox{{\sc SE}}$ to obtain $\mathbf{x}_j \in \{0,1\}$.

        \item[(b)] For every $j \in \Gamma'_{\mathbf{V}}$, choose an arbitrary value $\mathbf{x}_j$ from $\{0,1\}$.

        \item[(c)] Using $\mathbf{x} = (\mathbf{x}_1, \ldots, \mathbf{x}_n)$ obtained from (a) and (b), construct a new vector $\mathbf{V}'$ for which $\mathbf{V}'_{\pi}=\mbox{{\sc FE}}(\mathbf{z},\mathbf{x})$ for an arbitrary $\mathbf{z} \in [n]^m$, where $\pi$ is the permutation obtained from \findpi in Step (i) of \algadpt.
    \end{itemize}    

    \item For every vector $\mathbf{V} \in \mathcal{V} \setminus \mathcal{V}^{\mbox{inv}}$, set $\mathbf{V}' = \mathbf{V}$.

    \item Finally define $D_1(\mathbf{W})=\sum_{\mathbf{V}: \mathbf{V'} =\mathbf{W}} D(\mathbf{V})$ for every $\mathbf{W} \in \mathcal{V}$.

\end{itemize}

Let $\mathcal{V}'$ be the set of vectors in $\{0,1\}^N$ that are in the support of $D_1$ but not in $\mathcal{U}$. From the construction of $D_1$, the following observation follows.
\begin{obs}\label{obs:v-dash}
$D_1(\mathcal{U})=D(\mathcal{U})\leq 5 \alpha$ and $D_1(\mathcal{V}')=D(\mathcal{V})=1-D(\mathcal{U})\geq 1-5\alpha.$
\end{obs}

Now we prove that the distributions $D$ and $D_1$ are not far in Earth Mover Distance.

\begin{lem}\label{lem:d1d2emd}
The Earth Mover Distance between $D$ and $D_1$ is at most $\eps/10$.
\end{lem}

\begin{proof}
Recall that the EMD between $D$ and $D_1$ is the solution to the following LP:
\begin{eqnarray*}
    &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
    &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D(\mathbf{X})~\forall \ \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
    \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_1(\mathbf{Y})~\forall \ \mathbf{Y} \in \{0,1\}^N.
\end{eqnarray*}

Consider the flow $f^*$ such that $f^*_{\mathbf{XX}}=D(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U} \cup (\mathcal{V} \setminus \mathcal{V}^{\mbox{inv}})$, $f^*_{\mathbf{VV'}}=D_1(\mathbf{V})$ for every $\mathbf{V} \in \mathcal{V}^{\mbox{inv}}$, and $f^*_{\mathbf{X}\mathbf{Y}}=0$ for all other vectors. Then we have the following:
\begin{eqnarray*}
\mbox{EMD}(D,D_1) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^*_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
&\leq& \sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}^{\mbox{inv}}} f^*_{{\bf X X}}d_H({\bf X},{\bf X}) + \sum_{{\bf V} \in \mathcal{V}^{\mbox{inv}}} f^*_{{\bf V} {\bf V}'}d_H({\bf V},{\bf V'})\\
&\leq& 0 + \sum_{\mathbf{V}\in \mathcal{V}^{\mbox{inv}}}D(\mathbf{V})d_H({\bf V},{\bf V'}).
\end{eqnarray*}

To bound the second term of the last expression, note that $$\sum\limits_{\mathbf{V}\in \mathcal{V}^{\mbox{inv}}}D(\mathbf{V})d_H({\bf V},{\bf V'}) \leq D(\mathcal{V}^{\mbox{inv}}) \leq \eps/10$$. This follows from Observation~\ref{obs:v-enc}. Thus, we conclude that $\mbox{EMD}(D,D_1) \leq \eps/10$, completing the proof of the lemma.
\end{proof}

Now we have the following observation regarding the rejection probabilities of \algadpt for the distributions $D$ and $D_1$.

\begin{obs}
The probability that the tester \algadpt outputs {\sc Reject} in Step (iv) when the input distribution is $D$ is at least as large as the probability that \algadpt outputs {\sc Reject} in Step (iv) when the input distribution is $D_1$.
%Let $Q$ be the set of indices queried by the algorithm {\sc Alg-Adaptive} in Step (iv). Then {\sc Alg-Adaptive} is oblivious to $D_1$ and $D_2$ with respect to $Q$.
\end{obs}

\begin{proof}
Note that in the distribution $D$, there can be some vectors in $\mbox{Supp}(D)$ that are not valid encodings with respect to the function $\mbox{{\sc FE}}$. Thus during execution, the tester \algadpt can {\sc Reject} $D$ by Condition (ii) and Condition (iv) (b). However, by the construction of $D_1$ from $D$, we have replaced the invalid encoding vectors with valid encoding vectors. Thus, the only difference it makes here is that \algadpt may eventually accept a sample from $D_1$ when encountering such a place where a sample from $D$ would have been immediately rejected by Condition (ii) or Condition (iv) (b). Other than this difference, the distributions $D$ and $D_1$ are identical. So, the probability that \algadpt outputs {\sc Reject} $D$ is at least as large as the probability that it {\sc Rejects} $D_1$.
\end{proof}
From now on words, we can assume that the input to the algorithm \algadpt is the distribution $D_1$ instead of $D$.

Now, we deifne the distribution $\dhash$ as stated in Lemma~\ref{lem:far-D-star}.
\begin{equation}\label{def:enc-dist}
    \dhash(\mathbf{x})=D_1^{{enc}}(\mathbf{x})=\frac{1}{D_1(\mathcal{V}')}\sum_{\substack{\mathbf{Y}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}} D_1(\mathbf{Y}) = \frac{1}{D_1(\mathcal{V}')}\sum_{\mathbf{z}\in [n]^m}D_1(\mathrm{FE}(\mathbf{z},\mathbf{x})_{\pi^{-1}}).
\end{equation}

Now, let us come back to the proof of Lemma~\ref{lem:far-D-star}. For the sake of contradiction, assume that $\dhash=D_1^{dec}$ is $\eps/3$-close to having support size at most $n$. Let $D_{2}$ be a distribution over $\{0,1\}^{n}$ having support size at most $n$ such that the Earth Mover Distance between $D_2$ and $D_1^{dec}$ is at most $\eps/3$.
Given the distribution $D_{3}$ over $\{0,1\}^{n}$, and the flow $f'_{\mathbf{x}\mathbf{y}}$ from $D_2$ to $D_1^{dec}$ realizing the EMD of at most $\eps/3$ between them, let us consider the distribution $D_2^{enc}$ over $\{0,1\}^N$ such that for any $\mathbf{X} \in \mathcal{V}'$, for which $\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x})$ for some $\mathbf{z} \in [n]^m$, we have $D_2^{enc}(\mathbf{X})=\sum\limits_{\mathbf{y} \in \{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_1(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_1^{dec}(\mathbf{y})}$, and for every $\mathbf{X} \in \mathcal{U}$, $D_2^{enc}(\mathbf{X}) = D_1(\mathbf{X})$. The following claim upper bounds the distance of $D_2^{enc}$ from $\cP_{Gap}$ and the EMD between $D_2^{enc}$ and $D_1$ when $D_1^{dec}$ is $\eps/3$-close to having support $n.$
\begin{cl}\label{cl:close-P-gap}
$D_2^{enc}$ is $6\alpha$-close to property $\cP_{\mbox{Gap}}$.
\end{cl}

\begin{cl}\label{cl:emd-far}
Let $D_2^{enc}$ be the distribution over $\{0,1\}^N$ obtained from $D_2$. Then the EMD between $D_{2}^{enc}$ and $D_1$ is at most $\eps/3$.
\end{cl}
From Lemma~\ref{lem:d1d2emd}, $\mbox{EMD}(D,D_1)\leq \eps/10$. So, the above  two claims imply that $D$ is $(\eps/3+\eps/10+6\alpha)$-close to $\cP_{mbox{Gap}}$, which is a contradiction to the fact that $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$. Hence, we will be done with the proof of Lemma~\ref{lem:far-D-star} by proving Claims~\ref{cl:close-P-gap} and \ref{cl:emd-far}.
\begin{proof}[ Proof of Claim~\ref{cl:close-P-gap}]
 We define another distribution $D_3$ over $\{0,1\}^N$ from $D_2^{enc}$ as follows such that $D_3$ is in $\cP_{\mbox{Gap}}$ and $\mbox{EMD}(D_2,D_3)\leq 6 \alpha$.  $D_3(\mathbf{U}') = \alpha$, $D_3(\mathbf{X}) = \frac{\alpha}{b}$ for every $\mathbf{X} \in \cS'$, $D_3(\mathbf{X}) = \frac{\alpha}{\lceil \log kn \rceil}$ for every $\mathbf{X} \in \cT'$, and $D_3(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D_2^{enc}(\mathbf{X})}{D_2^{enc}(\mathcal{V}')}$ for every $\mathbf{X} \in \mathcal{V}'$. Then we have the following lemma.
Recall that all the vectors in $\mathcal{V}$ are valid encodings. From the definition of $\cP_{\mbox{Gap}}$ and $D_3$, it is clear that $D_3 \in \cP_{\mbox{Gap}}$


%From Observation~\ref{obs:sumdothervec}, we know that $D(\{\mathbf{U}'\} \cup S' \cup T') \leq 5 \alpha$. As $D_1(\mathbf{X})= {(1 - 3 \alpha)} \cdot \frac{D(\mathbf{X})}{D(\mathcal{V})}$ for every $\mathbf{X} \in \mathcal{V}$, and $\mathcal{V}^{\mbox{invalid}} \subseteq \mathcal{V}$, we can say that for every $\mathbf{X} \in \mathcal{V}^{\mbox{invalid}}$, $D_1(\mathbf{X}) \leq \frac{1- 3 \alpha}{1 - 5 \alpha} D(\mathbf{X})$. Since $\alpha=1/\log n$, from Lemma~\ref{lem:sumencvector}, we know that $\sum_{\mathbf{V}\in \mathcal{V}^{\mbox{invalid}}} D(\mathbf{V})\cdot \frac{\size{\Gamma'_{\mathbf{V}}}}{n} \leq \frac{\eps}{10}$, for sufficiently large $n$, we have the result.


Now we show that the Earth Mover Distance between the distributions $D_1$ and $D_2$ is not large.

\begin{lem}\label{lem:dd1emd}
The Earth Mover Distance between $D_1$ and $D_2$ is at most $6\alpha$.
\end{lem}

\begin{proof}
We will bound the Earth Mover Distance between $D_1$ and $D_2$ in terms of the variation distance between them as follows:
\begin{eqnarray}
    \mbox{EMD}(D_1,D_2) &\leq& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N}|D_1(\mathbf{X}) - D_2(\mathbf{X})| \nonumber \\ &=& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{V}'}|D_1(\mathbf{X}) - D_2(\mathbf{X})| + \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}'}|D_1(\mathbf{X}) - D_2(\mathbf{X})| \label{eqn:emddd1}
\end{eqnarray}

\color{blue}

Let us bound the first term as follows:
\begin{eqnarray*}
    \sum_{\mathbf{X} \in \mathcal{V}}|D_1(\mathbf{X}) - D_2(\mathbf{X})|
    &=& \sum_{\mathbf{X} \in \mathcal{V}'}| (1- 3 \alpha) \frac{D_1(\mathbf{X})}{D_1(\mathcal{V}')} - D_1(\mathbf{X})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}'} \frac{D_1(\mathbf{X})}{D_1(\mathcal{V})} |(1- 3 \alpha) - D_1(\mathcal{V}')| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}'} \frac{D_1(\mathbf{X})}{D_1(\mathcal{V}')} |3 \alpha - (1- D_1(\mathcal{V}'))| \\ &\leq & \sum_{\mathbf{X} \in \mathcal{V}'} 3 \alpha \frac{D_1(\mathbf{X})}{D_1(\mathcal{V}')} \leq 3 \alpha ~~~(\because D_1(\mathcal{V}')=1-D_1(\mathcal{U})\geq 1- 5 \alpha)
\end{eqnarray*}

\color{black}

From Observation~\ref{obs:v-dash}, $D_1(\mathcal{U}) \leq 5 \alpha$. From the definition of $D_2$, $D_2(\mathcal{U}) = 3 \alpha$, we have
   $$\sum_{\mathbf{X} \in \{0,1\}^N \setminus \mathcal{V}'}|D_1(\mathbf{X}) - D_2(\mathbf{X})| \leq 8 \alpha.$$
Following Equation~\ref{eqn:emddd1}, we conclude that $\mbox{EMD}(D_1,D_2) \leq 6 \alpha$, which completes the proof.

\end{proof}
\end{proof}

\begin{proof}



\begin{proof}[Proof of Claim~\ref{cl:emd-far}]

\color{blue}

Recall that the EMD between $D_2^{enc}$ and $D_1$ is the solution to the following LP:
\begin{eqnarray*}
    &&\mbox{Minimize}\quad{\sum_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})}\\
    &&\mbox{Subject to}\quad\sum_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_2^{enc}(\mathbf{X})~\forall \mathbf{X} \in \{0,1\}^N \; \mbox{and} \;
    \sum_{\mathbf{X} \in \{0,1\}^N} f_{\mathbf{X}\mathbf{Y}} = D_1(\mathbf{Y})~\forall \mathbf{Y} \in \{0,1\}^N.
\end{eqnarray*}

Let $f'_{\mathbf{x} \mathbf{y}}$ be the flow realizing the EMD between $D_2$ and $D_1^{dec}$. Using $f'$, we now construct a new flow $f^\star$ between $D_2^{enc}$ and $D_1$ as follows:

\begin{itemize}
    \item[(1)]  For vectors $\mathbf{X}, \mathbf{Y} \in \mathcal{U}$,
    
\begin{itemize}
    \item[(i)] If $\mathbf{X} \neq \mathbf{Y}$, then set $f^\star_{\mathbf{X} \mathbf{Y}}=0$. 

    \item[(ii)] If $\mathbf{X} = \mathbf{Y}$, then set $f^\star_{\mathbf{X} \mathbf{Y}} = D_2^{enc}(\mathbf{X})=D_1(\mathbf{Y})$.
    \end{itemize}
    
    \item[(2)] For two vectors $\mathbf{X}, \mathbf{Y} \in \mathcal{V}$, we take the vectors $\mathbf{x}, \mathbf{y} \in \{0,1\}^n$ such that $\mathbf{X}, \mathbf{Y} \in \{0,1\}^N$ are their
valid encodings (by construction such vectors $\mathbf{x}, \mathbf{y}$ exist), and vectors $\mathbf{z}_1,\mathbf{z}_2$ such that $\mathbf{X}=\fen(\mathbf{z}_1,\mathbf{x})$ and $\mathbf{Y}=\fen(\mathbf{z}_2, \mathbf{y})$. Now we set the flow as follows:
\begin{itemize}
    \item[(i)] If $\mathbf{z}_1 \neq \mathbf{z}_2$, then set $f^\star_{\mathbf{X} \mathbf{Y}} = 0$.

    \item[(ii)] If $\mathbf{z}_1 = \mathbf{z}_2$, then set $f^\star_{\mathbf{X} \mathbf{Y}} =  f'_{\mathbf{x} \mathbf{y}} \cdot \frac{D_1(\mathbf{Y})}{D_1^{dec}(\mathbf{y})}$.
\end{itemize}

\item[(3)] If one of $\mathbf{X}$ and $\mathbf{Y}$ is in $\mathcal{U}$ and the other one is in $\mathcal{V}$, then $f^\star_{\mathbf{X}\mathbf{Y}}=0$.

\end{itemize}


We first argue that the flow $f^*_{\mathbf{X} \mathbf{Y}}$ constructed as above is indeed a valid flow, that is, we have:
$(i) \sum\limits_{\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}} = D_2^{enc}(\mathbf{X})$, and $(ii) \sum\limits_{\mathbf{X} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}} = D_1(\mathbf{Y})$. 

%We prove the first one and omit the other similar proof.

To prove $\sum\limits_{\mathbf{Y} \in \{0,1\}^N} f_{\mathbf{X} \mathbf{Y}} = D_2^{enc}(\mathbf{X})$, first observe that it holds when $\mathbf{X} \in \mathcal{U}$ from (1) and (3) in the description of $f^{\star}_{\mathbf{X} \mathbf{Y}}$. Now consider when $\mathbf{X} \in \mathcal{V}$. Assume $\mathbf{X}_{\pi}=\fen\left(\mathbf{z},\mathbf{x}\right)$, where $\mathbf{z} \in [n]^m$ and $\mathbf{x} \in \{0,1\}^n$. So, from (2) in the description of $f^\star_{\mathbf{X}\mathbf{Y}}$, we have
$$\sum\limits_{\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X} \mathbf{Y}}=\sum\limits_{\mathbf{y} \in \{0,1\}^n} f^\star_{\mathbf{X} \mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}}} = \sum_{\mathbf{y}\in\{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_1(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_1^{dec}(\mathbf{y})}=
D_2^{enc}(\mathbf{X}).$$

%\sum\limits_{\mathbf{y} \in \{0,1\}^n}f'_{\mathbf{x} \mathbf{y}} \cdot \frac{D_1(\mathbf{X})}{D_1^{dec}(\mathbf{x})}=D_3(\mathbf{x})\cdot \frac{D_1(\mathbf{X})}{D_1^{dec}(\mathbf{x})}= 

%\remove{For example, for $Y \in \mathcal{U}$ it is (by the construction above) quite clear that $\sum_X f_{XY} = f_{YY} = D_1(Y)$, and for $Y=FE(z,y)$ for some $z,y$ (which is the only other non-zero option) we have $\sum_X f_{XY} = \sum_{z',x} f_{FE(z',x),Y} = \sum_x f_{FE(z,x),Y}= \sum_x f'_{xy} \cdot \frac{D_1(Y)}{D_1^{dec}(y)} = D_1(Y)$.}

For (ii), consider $\mathbf{Y}_{\pi} = \mathrm{FE}(\mathbf{z}, \mathbf{y})$ for some $\mathbf{z} \in [n]^m$. Then we have the following:
$$\sum_{\mathbf{X}\in\{0,1\}^N}f_{\mathbf{X}\mathbf{Y}}^{\star}=\sum_{\mathbf{x}\in\{0,1\}^n}f'_{\mathbf{x}\mathbf{y}}\frac{D_1(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_1^{dec}(\mathbf{y})}=D_1^{dec}(\mathbf{y})\frac{D_1(\mathrm{FE}(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_1^{dec}(\mathbf{y})}=D_1(\mathbf{Y}).$$

In the above, we have used the fact that $f'_{\mathbf{x} \mathbf{y}}$ is a valid flow from $D_2$ to $D_1^{dec}$.\\

Now, to bound EMD between $D_2^{enc}$ and $D_1$, let us bound the sum $\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})$.
%From (1) and (3) in the description of $f^\star$, $\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})=\sum\limits_{\mathbf{X},\mathbf{Y} \in \mathcal{V}} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y}).$
\begin{eqnarray*}
&&\sum\limits_{\mathbf{X},\mathbf{Y} \in \{0,1\}^N} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})\\
&=&\sum\limits_{\mathbf{X},\mathbf{Y} \in \mathcal{V}} f^\star_{\mathbf{X}\mathbf{Y}} d_H(\mathbf{X},\mathbf{Y})~~~\left(\mbox{From (1) and (3) in the description of $f^\star$}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f^\star_{\mathbf{\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}}\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}}}\cdot d_H({\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}},\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})\\ &&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\left(\mbox{From (2) in the description of $f^\star$}\right)\\
&\leq&\sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f^\star_{\mathbf{\fen(\mathbf{z},\mathbf{x})_{\pi^{-1}}}\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}}}\cdot d_H(\mathbf{x},\mathbf{y})~~~\left(\mbox{Observation~\ref{obs:FEproperties} (iii)}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\sum\limits_{\mathbf{z}\in [n]^m} f'_{\mathbf{x}\mathbf{y}}\frac{D_1(\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_1(\mathbf{y})}\cdot d_H(\mathbf{x},\mathbf{y})~~~\left(\mbox{From (2) in the description of $f^\star$}\right)\\
&=& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n}\left(f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y})\cdot  \sum\limits_{\mathbf{z}\in [n]^m} \frac{D_1(\fen(\mathbf{z},\mathbf{y})_{\pi^{-1}})}{D_1(\mathbf{y})}\right)\\
&=& D_1(\mathcal{V}') \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n} f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y})~~~(\mbox{By Equation}~\eqref{def:enc-dist})\\
&\leq& \sum\limits_{\mathbf{x},\mathbf{y} \in \{0,1\}^n} f'_{\mathbf{x}\mathbf{y}}d_H(\mathbf{x},\mathbf{y}) \leq \frac{\eps}{3}.
\end{eqnarray*}
The last inequality follows from the fact that $f'$ realizes the EMD between $D_3$ and $D^{dec}_2$.
\end{proof}

\color{black}

% \remove{As before, we will bound the Earth Mover Distance between $D_3^{enc}$ and $D_2$ in terms of their variation distance.
% \begin{eqnarray}
%     EMD(D_{3}^{enc}, D_2) &\leq& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \{0,1\}^N}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| \nonumber \\ &=& \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| + \frac{1}{2} \cdot \sum_{\mathbf{X} \in \mathcal{U}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| \label{eqn:emdd3encd2}
% \end{eqnarray}

% As $D_3^{enc}(\mathbf{X}) = D_2(\mathbf{X})$ for every $\mathbf{X} \in \mathcal{U}$, the second term in the above equation is $0$. Now let us bound the first term. Since for every $\mathbf{X} \in \mathcal{V}$,
% $D_3^{enc}(\mathbf{X})=(1-3\alpha)D_3(\mathbf{x}) \cdot \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}$, we can deduce the following:
% \begin{eqnarray*}
% \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| &=& \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}} |(1-3\alpha)D_3(\mathbf{x})\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}-D_2(\mathbf{X})| \\
% &\leq& 3\alpha \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}}\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}D_3(\mathbf{x}) + \\ && \sum_{\mathbf{x}\in Supp(D_2^{dec})} \sum_{\substack{\mathbf{X}_{\pi} = \mbox{{\sc FE}}(\mathbf{z},\mathbf{x}) \\ \mbox{for some} \ \mathbf{z} \in [n]^m}}\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})}|D_3(\mathbf{x})-D_2^{dec}(\mathbf{x})| \\
% &=&3\alpha + \sum_{\mathbf{x}\in Supp(D_2^{dec})}|D_3(\mathbf{x})-D_2^{dec}(\mathbf{x})| \\
% &\leq& 3\alpha+\frac{2\eps}{3} \leq \eps
% \end{eqnarray*}
% }
% \begin{eqnarray*}
%     \sum_{\mathbf{X} \in \mathcal{V}}|D_{3}^{enc}(\mathbf{X}) - D_2(\mathbf{X})| &=& \sum_{\mathbf{X} \in \mathcal{V}}|(1-3\alpha)D_{3}(\mathbf{x}) \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} - D_2(\mathbf{X})| \\ &=& \sum_{\mathbf{X} \in \mathcal{V}} |(1-3\alpha)\frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} -1| \\ &\leq & \sum_{\mathbf{X} \in \mathcal{V}} D_2(\mathbf{X}) |\frac{D_3(\mathbf{x}) - D_2^{dec}(\mathbf{x})}{D_2^{dec}(\mathbf{x})}| \\ &\leq& \sum_{\mathbf{X} \in \mathcal{V}} \frac{D_2(\mathbf{X})}{D_2^{dec}(\mathbf{x})} \cdot \frac{\eps}{3} \leq \frac{2 \eps}{3}
% \end{eqnarray*}

%Substituting this value in Equation~\ref{eqn:emdd3encd2}, we have the result.


% Let $f^{(1)}$ be the flow from $D_2^{dec}$ to $D_3$ realizing the EMD between $D_2^{dec}$ and $D_3$. Let us consider the flow $f^{(2)}$ from $D_2$ to $D_{3}^{enc}$ as described below:
% \begin{itemize}
%     \item $f^{(2)}_{\mathbf{X}\mathbf{X}}=D_2(\mathbf{X})=D_{3}^{enc}(\mathbf{X})$ for each $\mathbf{X} \in \{\mathbf{U}'\}\cup S' \cup T'$.
    
%     \item For every $\mathbf{x},\mathbf{y} \in \{0,1\}^{n}$, 
% $f^{(2)}_{\mathbf{XY}} = (1-3\alpha)f^{(1)}_{\mathbf{xy}}$, where $\mathbf{X}= \cE(\mathbf{x})$ and $\mathbf{Y}= \cE(\mathbf{y})$.

%       \item Otherwise, $f^{(2)}_{\mathbf{XY}}=0$.
% \end{itemize}

% Now we have the following observation which directly follows from the encoding procedure.
% \begin{obs}
% For any $\mathbf{x, y}\in \{0,1\}^{n}$, the Hamming distance between their encoding is at most the Hamming distance between them.
% \end{obs}
% Thus we have the following:
% \begin{eqnarray*}
% \mbox{EMD}(D_{3}^{enc},D_2) &\leq& \sum_{{\bf X},{\bf Y} \in \{0,1\}^N} f^{(2)}_{{\bf X Y}}d_H({\bf X},{\bf Y}) \\
% &\leq& \sum_{\mathbf{X} \in \{\mathbf{U}'\} \cup S' \cup T' } f^{(2)}_{{\bf X X}}d_H({\bf X},{\bf X}) + \sum_{\mathbf{x,y}\in \{0,1\}^{n}} f^{(2)}_{{\bf \cE(\mathbf{x})\cE(\mathbf{y})}} d_H(\cE(\mathbf{x}),\cE(\mathbf{y}))\\
% &\leq& 0+ \sum_{\mathbf{x,y}\in \{0,1\}^{n}} f^{(1)}_{\mathbf{x}\mathbf{y}} d_H(\mathbf{x},\mathbf{y})\\
% &=& EMD(D_3,D_2^{dec})\leq \eps/3.
% \end{eqnarray*}
% \end{proof}


Since the distribution $D_{3}$ over $\{0,1\}^{n}$ has support size at most $n$, following the encoding procedure, we can say that $D_3^{enc} \in \cP_{\mbox{Gap}}$. But this would contradict the fact that $D_2$ is $2\eps/3$-far from $\cP_{\mbox{Gap}}$. This completes the proof of the lemma.
\end{proof}

Combining the arguments above, we conclude that if the input distribution $D$ is $\eps$-far from $\cP_{\mbox{Gap}}$, the tester \algadpt will output {\sc Reject} with probability at least $2/3$.


==> vc_dim.tex <==
\section{Learning Clusterable Distributions}

\begin{defi}[$(\zeta, \delta, r)$-clusterable distribution]\label{defi:cluster}

For $\zeta,\delta>0$ and $r \in \N$, a distribution $D$ over $\{0,1\}^n$ is said to be $(\zeta, \delta,r)$-clusterable if there exists a partition $C_0, \ldots, C_s$ of $\{0,1\}^n$, where $D(C_0) \leq \zeta$, $s \leq r$, and $\mu(\mathbf{u},\mathbf{v})\leq \delta$ for every $1 \leq i \leq s$ and $\mathbf{u},\mathbf{v} \in C_i$.




% Let  $V$ be a set of vectors in $\{0,1\}^n$ and $C_0, \ldots, C_s$ be a partition of $V$. A distribution $D$ supported over $V$ is said to be a $(\zeta, \delta,r)$-clusterable distribution if $s  \leq r, D(C_0) \leq \zeta$ and for every $1 \leq i \leq s$ and $\mathbf{u}, \mathbf{v} \in C_i$, $\mu(\mathbf{u}, \mathbf{v}) \leq \delta$, where $\mu$ denotes the normalized Hamming distance. 

%Here $\mathbf{C}_1, \ldots, \mathbf{C}_r$ are said to be the \emph{clusters} of the distribution $D$;



\begin{theo}\label{theo:mainthm}
Let $n \in \N$; $r \in \N$, $\zeta, \delta, \eps\in (0,1)$ are independent of $n$ such that $\eps= 25 (\zeta +  \delta)$. Given sample and query access to an unknown distribution $D$ over $\{0,1\}^n$, there exists an algorithm that makes number of queries that only depends on $\eps$ and $r$, and produces a distribution with the following guarantee:
\begin{description}
    \item[(i)] If $D$ is $(\zeta, \delta, r)$-clusterable, then with probability at least $\frac{2}{3}$, the algorithm outputs a full description of a distribution $D'$ over $\{0,1\}^n$ such that $d_{EM}(D, D'_{\sigma}) \leq \eps$ for some permutation $\sigma:[n] \rightarrow [n]$.
    
    \item[(ii)] For any $D$, the algorithm will not output a distribution which is $\eps$-far from $D$ with probability more than $\frac{1}{3}$. However, if the distribution $D$  is not $(\zeta, \delta, r)$-clusterable, the algorithm may output {\sc Fail} with any probability.
\end{description}
\end{theo}

In order to prove the above theorem, we will use the notion of a clustered distribution with respect to a set $S$, defined as follows:

\begin{defi}[$(\eta, \xi)$-clustered distribution with respect to a set]\label{def:concdist}
Let $\eta ,\xi \in (0,1)$, and  $\mbox{{\sc NGB}}_{\eta}({\bf x})$ denotes the set of vectors in $\{0,1\}^n$ that are at a distance of at most $\eta$ from ${\bf x}$. Let $D$ be a distribution over $\{0,1\}^n$, $S= \{\mathbf{s}_1, \ldots, \mathbf{s}_{t}\}$ be a sequence of $t$ vectors in $\{0,1\}^n$.

\begin{description}
\item[(i)]   $D$ is said to be $(\eta,\xi)$-clustered around $S$  with weights $w_0, \ldots, w_{t_1}$ if $D({\sc NGB}_{\eta}(\mathbf{s}_i)) \geq w_i$, for each $i \in [t_1]$, $D(\bigcup\limits_{i=1}^{t_1} NGB_{\eta}(\mathbf{s}_i)) \geq 1 - \xi$, $ w_0 \leq \xi$,  where $w_0,\ldots,w_t \in [0,1]$ such that $\sum\limits_{i=0}^t w_i =1$;

\item[(ii)] $D$ is said to be  $(\eta,\xi)$-clustered around $S$ if $D$ is $(\eta,\xi)$-clustered around $S$ with weights $w_0, \ldots, w_t$ for some $w_0, \ldots, w_t$ with $w_0 \leq \xi$, where $w_0,\ldots,w_t \in [0,1]$ such that $\sum\limits_{i=0}^t w_i =1$.

\end{description}
%$D(\mbox{{\sc NGB}}_{\eta}(s_i)) \geq w_i$, $D({\sc NGB}_{\eta}(s_i) \setminus \bigcup_{j=1}^{i-1} {\sc NGB}_{\eta}(s_j)) = w_i$, for each $i \in [t_1]$ and $D(\{0,1\}^n \setminus \bigcup_{i=1}^t\mbox{{\sc NGB}}(s_i)) = w_0 \leq \xi$

\end{defi}


Now let us consider the following lemma which will be used to prove Theorem~\ref{theo:mainthm}. In this lemma, along with all associated lemmas, the input includes sequence of strings $S$, and we have query access to these strings.

\begin{lem}\label{lem:conc}
Let $n \in \N$, $r, t_1 \in \N$, $ \eta, \xi \in (0,1)$ be parameters independent of $n$, and let $S^{(1)}=\{\mathbf{s}_1^{(1)},\ldots,\mathbf{s}^{(1)}_{t_1}\}$ be a sequence of vectors in $
\{0,1\}^n$ such that $\eps_1= 8 \eta +  3 \xi$. There exists an algorithm \cluster, that has sample and query access to an unknown distribution $D$ over $\{0,1\}^n$ which is $(\eta, \xi)$-clustered around  $S^{(1)}$,  that performs a number of queries that only depends on $\eps_1$ and $t_1$, to $D$ and produces a distribution with the following guarantee: 
\begin{center}
With probability at least $1 - \frac{1}{t_1^2}$, the algorithm outputs a full description of a distribution $D'$ over $\{0,1\}^n$ such that $d_{EM}(D, D'_{\sigma}) \leq \eps_1$ holds for some permutation $\sigma:[n] \rightarrow [n]$.
 \end{center}

\end{lem}

%\begin{algorithmic}

\begin{algorithm}[H]
%\scriptsize

\SetAlgoLined

\caption{\clus (Theorem~\ref{theo:mainthm})}
\label{alg:testcluster--}
\KwIn{Sample and Query access to a distribution $D$ over $\{0,1\}^n$}
\KwOut{Either {\sc Reject} or outputs a distribution $D'$ over $\{0,1\}^n$}
%\LinesNumbered
\begin{itemize}
\item[(i)] First take $t_1=\Oh(\frac{r}{\zeta} \log \frac{r}{\zeta})$ many samples from $D$. Let $S^{(1)}= \{\mathbf{s}_1^{(1)}, \mathbf{s}_2^{(1)}, \ldots, \mathbf{s}_{t_1}^{(1)}\}$ be the set of vectors obtained. 
 
 %These vectors will be considered as prospective cluster centers in the algorithm below.


\item[(ii)] Now take another set of samples $S^{(2)} = \{\mathbf{s}_1^{(2)}, \mathbf{s}_2^{(2)}, \ldots, \mathbf{s}_{t_2}^{(2)}\}$ from $D$, where $t_2= \Oh(\frac{t_1^2}{\zeta^2} \log t_1$). Also, sample a set of indices $J \subset [n]$ randomly, such that $\size{J} = \Oh(\frac{\log \size{S^{(1)}}}{\delta})$. Now consider $S^{(2)}_{\mid J}$, the set of vectors of $S^{(2)}$ projected on $J$. For every $\mathbf{s} \in S^{(2)}$, if there exists a $k \in [t_1]$ such that $\mu({\mathbf{s}_{k}^{(1)}}_{\mid J}, \mathbf{s}_{\mid J})\leq 2 \delta$ for some $\mathbf{s}^{(1)}_k$, we assign $\mathbf{s}$ to $\mathbf{s}^{(1)}_k$, breaking ties by assigning $\mathbf{s}$ to the vector in $S^{(1)}$ with the minimum index. Otherwise, we do not assign $\mathbf{s}$ to any vector in $S^{(1)}$. 




%Let $\phi:S^{(2)} \rightarrow S^{(1)} \cup \{\mathbf{u}\}$ be the assignment function such that $\phi(\mathbf{x})$ is the vector in $S^{(1)}$ to which $\mathbf{x}$ has been assigned to.
    
    %Now we greedily form cluster centers  $O_1,O_2,\ldots$ as follows. Set $O_1=s_1^{(1)}$. Assume that we have created cluster centers $O_1,\ldots,O_i$ and considered the vectors $s_1^{(1)},\ldots,s_j^{(1)}$, where $i \leq j$. If there exists an $k \in [i]$ such that $\mu({s_{j+1}^{(1)}}_{\mid I}, s_{\mid J})\leq 2 \delta$ for all vectors $s$ assigned to cluster center $O_k$, we assign $s_{j+1}^{(1)}$ to $O_k$, breaking ties by assigning $s_{j+1}^{(1)}$ to the cluster center with the minimum index. Otherwise, we create a new cluster center $O_{i+1}=s_{j+1}^{(1)}$.
    
    \item[(iii)] If the fraction of samples in $S^{(2)}$, that are not assigned to any vector in $S^{(1)}$ exceeds $3 \zeta$, then output {\sc Reject}.
    
    \item[(iv)] Otherwise, call Algorithm \cluster (described in Algorithm~\ref{alg:testcluster}) with $\zeta'=5\zeta$ and $\delta'=3\delta$, and report the distribution $D'$ returned by \cluster.
    
    

%If $\sum\limits_{i=1}^{t_1} w(\mathbf{s}^{(1)}_i) \geq 1 - 3 \zeta$, we {\sc Accept} and return $\mathbf{s}^{(1)}_1, \ldots,\mathbf{s}^{(1)}_{t_1}$, along with $w(\mathbf{s}^{(1)}_1), \ldots, w(\mathbf{s}^{(1)}_{t_1})$. Otherwise, we report {\sc Reject}.
    
    
    %Assume $O_1, \ldots, O_{\ell}$ be the set of cluster centers determined in Step (i). For each $x \in \{O_1, \ldots, O_{\ell}\}$, the weight of $x$ is denoted and defined as follows:
%$$w(x)=\frac{\mbox{The number of elements in $S^{(1)}$ assigned to $x$}}{\size{S^{(1)}}}. $$

%\item[(iii)] Without loss of generality, let us assume $O_1, \ldots, O_{\ell}$ are the cluster centers sorted in non-increasing order of their weights determined in Step (ii). If there exist $m \leq r$ cluster centers such that $\sum\limits_{i=1}^m w(O_i) \geq 1 - 3 \eps$, we {\sc Accept} and return $O_1, \ldots, O_m$, along with $w(O_1), \ldots, w(O_m)$. Otherwise, we report {\sc Reject}.

    
\end{itemize}
        
\end{algorithm}

%\end{algorithmic}

\begin{proof}[Proof of Theorem~\ref{theo:mainthm}]

First let us argue the query complexity of the algorithm \clus.
\clus does not perform any query in Step (i) and Step (iii). It performs at most $\Oh(\size{S^{(1)}} \size{S^{(2)}} \size{J})$ many queries in Step (ii) which is at most $\Oh(\frac{r^2}{\zeta^5 \delta} \log^5 \frac{r}{\zeta})$. Moreover, in Step (iv), \clus calls \cluster, and as we discussed before, the total number of queries made by \cluster is a function of only $\eta= 3 \delta, \xi=5 \zeta$ and $t_1=\size{S^{(1)}}=\Oh\left(\frac{r}{\zeta}\log \frac{r}{\zeta}\right))$.
As $\eps= 25 (\zeta + \delta)$, we can say that the number of queries performed by the algorithm \clus depends only on $\eps$ and $r$.

%Now let us consider the algorithm \clus.

In order to prove (i) and (ii), we will use the following claim which we will prove later.

\begin{cl}\label{cl:concfar}
\begin{description}
    \item[(i)]  If $D$ is $(\zeta, \delta, r)$-clusterable, then $D$ is $(\delta,2\zeta)$-clustered around $S^{(1)}$, and the fraction of samples in $S^{(2)}$ that are not assigned to any vector in $S^{(1)}$ will be at most $3\zeta$, with probability at least $1 - \frac{1}{t_1^4}$.
    
    \item[(ii)] If $D$ is not $(3\delta,5\zeta)$-clustered around set  $S^{(1)}$, then the fraction of samples in $S^{(2)}$ that are not assigned to any vector in $S^{(1)}$ will be at least  $3\zeta$, with probability at least $1 - \frac{1}{t_1^4}$.
\end{description}
\end{cl}

Now we proceed to prove (i) and (ii) as follows.


\begin{description}

\item[(i)] Observe that by Claim~\ref{cl:concfar} (i), we can say that when $D$ is $(\zeta, \delta,r)$-clusterable, the fraction of samples in $S^{(2)}$ that are not assigned to any vector in $S^{(1)}$ is at most $3 \zeta$. Thus, the algorithm \clus will not reject $D$ in Step (iii) with probability at least $1 - \frac{1}{t_1^4}$. Moreover, as $D$ is $(\delta, 2 \zeta)$-clustered around $S^{(1)}$, by Lemma~\ref{lem:conc}, we can say that the algorithm \clus will output a distribution $D'$ such that $d_{EM}(D, D'_{\sigma}) \leq \eps$ for some permutation $\sigma$ over $[n]$ with probability at least $1 - \frac{1}{t_1^2}$. This completes the proof of $(i)$. 

\item[(ii)] We proceed in similar fashion as (i). By Claim~\ref{cl:concfar} (ii), we know that when $D$ is not $(3 \delta, 5 \zeta)$-clustered around $S^{(1)}$, then the fraction of samples in $S^{(2)}$ that are not assigned to any vector in $S^{(1)}$ is at least $3 \zeta$ with probability at least $1 - \frac{1}{t_1^4}$. So, the algorithm \clus will reject $D$ in Step (iii) with probability at least $1 - \frac{1}{t_1^4}$. Thus, any distribution $D$ that passes Step (iii) of \clus is $(3 \delta, 5 \zeta)$-clustered around $S^{(1)}$ with probability at least $1 - \frac{1}{t_1^4}$. Then, by Lemma~\ref{lem:conc}, we can say that \clus will output a distribution $D'$ such that $d_{EM}(D, D'_{\sigma}) \leq \eps$ for some permutation $\sigma$ over $[n]$ with probability at least $1- \frac{1}{t_1^2}$. Thus, (ii) holds as well.

\end{description}

\end{proof}

\begin{proof}[Proof of Claim~\ref{cl:concfar}]

\begin{itemize}
    \item[(i)] Suppose the distribution $D$ is $(\zeta, \delta, r)$-clusterable with the clusters $C_1, \ldots, C_r$, that is $\sum\limits_{i=1}^r D(C_i) \geq 1 - \zeta$ and for any two vectors $\mathbf{x}, \mathbf{y} \in C_i$, $\mu(\mathbf{x}, \mathbf{y}) \leq \delta$ for any $i \in [r]$.
    
    We say a cluster $C_i$ is \emph{large} if $D(C_i) \geq \frac{\zeta}{10 r}$. As $\size{S^{(1)}} = \Oh(\frac{r}{\zeta} \log \frac{r}{\zeta}$), we have the following observation:

\begin{obs}
\label{obs:largeclusternonempty}
With probability at least $1 - \frac{1}{t_1^4}$, for any large cluster $C_i$, $C_i \cap S^{(1)} \neq \emptyset$ holds.
\end{obs}

\begin{proof}
Let us consider an arbitrary cluster $C_i$ with $i \in [r]$. As $D(C_i) \geq \frac{\zeta}{10r}$, the probability that no vectors of $S^{(1)}$ belong to $C_i$ is at most $(1 - \frac{\zeta}{10r})^{\size{S^{(1)}}}$. Using the union bound, the claim follows.
\end{proof}


    
%Then using the union bound along with Observation~\ref{obs:largeclusternonempty}, we can say that $\mathbf{C}_i \cap S^{(1)} \neq \emptyset$ for each large cluster $\mathbf{C}_i$ with probability at least $1 - \frac{1}{r^2}$. 
Following Observation~\ref{obs:largeclusternonempty}, with probability at least $1- \frac{1}{t_1^4}$, $S^{(1)}$ contains at least one point from each large cluster. Now, if we consider the $\delta$-neighborhood of $S^{(1)}$, that is, ${\sc NGB}_{\delta}(S^{(1)})$, we can say that all points in large clusters are in ${\sc NGB}_{\delta}(S^{(1)})$, with probability at least $1- \frac{1}{t_1^4}$. By the definition of large cluster, the mass on the points that are not in any big cluster is at most $2 \zeta$. Hence, $D({\sc NGB}_{\delta}(S^{(1)})) \geq (1 - 2 \zeta)$. Thus, by Definition~\ref{def:concdist}, we can say that $D$ is $(\delta, 2\zeta)$-clustered around the set $S^{(1)}$. 

%Now note that the total mass of $D$ over the clusters which are not large is at most $\zeta$. Moreover, as $D$ is $(\zeta, \delta, r)$-clusterable, we know that $\sum\limits_{i=1}^r D(\mathbf{C}_i) \geq 1 - \zeta$. Thus, by Definition~\ref{def:concdist}, we can say that $D$ is $(2\zeta, \delta)$-concentrated with respect to $S^{(1)}$. 
    
%Before directly proceeding to prove the second result, let us first consider the following claim which states that if the normalized Hamming distance between two vectors $\mathbf{x}$ and $\mathbf{y}$ are small, the same also holds with high probability when $\mathbf{x}$ and $\mathbf{y}$ are projected on a set of random indices $I$. Similar result also holds when the distance is large between the two vectors $\mathbf{x}$ and $\mathbf{y}$.

% \begin{cl}\label{cl:distchernoff}
% Let us assume $\mathbf{u}, \mathbf{v} \in \{0,1\}^n$ and $K \subseteq [n]$ be a set of indices chosen uniformly at random. Then the following hold:

% \begin{itemize}
%     \item[(i)] If $\mu(\mathbf{u}, \mathbf{v}) \leq \delta$, then $\mu(\mathbf{u}_{\mid K}, \mathbf{v}_{\mid K}) \leq 2 \delta$ with probability at least $1 - e^{-\Oh(\delta\size{K} )}$.
    
%     \item[(ii)] If $\mu(\mathbf{u}, \mathbf{v}) > 3 \delta$, then $\mu(\mathbf{u}_{\mid K}, \mathbf{v}_{\mid K}) > 2 \delta$ with probability at least $1 - e^{-\Oh(\delta \size{K} )}$.
% \end{itemize}
% \end{cl}

% \begin{proof}
% Follows from the fact that $K$ has been chosen uniformly at random along with Chernoff bound.
% \end{proof}
    
    
For the second part, let us define a binary random variable $X_i$ that takes value $1$ if and only if the $i$-th sample of $S^{(2)}$, that is,  $\mathbf{s}_i^{(2)}$ is not assigned to any vector in $S^{(1)}$. Note that $X_i$ is $1$ if $\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}^{(1)} \mid_J) > 2 \delta$ for all $\mathbf{s}^{(1)} \in S^{(1)}$, following Step (ii) of \clus.
    
Now there can be two possibilities when $\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}^{(1)} \mid_J) > 2 \delta$. They are when $\mathbf{s}_i^{(2)} \in {\sc NGB}_{\delta}({S^{(1)}})$, and when $\mathbf{s}_i^{(2)} \notin {\sc NGB}_{\delta}({S^{(1)}})$. Note that for the first case, $X_i =1$ will hold only when $\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}^{(1)_j} \mid_J) > 2 \delta$ hold for each $j \in S^{(1)}$. So, the probability of the event $X_i=1$ is as follows:
\begin{eqnarray*}
\pr(X_i=1) &\leq& \pr(\mathbf{s}_i^{(2)} \in {\sc NGB}_{\delta}({S^{(1)}}))\cdot \prod\limits_{j=1}^{\size{S^{(1)}}}\pr(\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}_j^{(1)} \mid_J) > 2 \delta) + \pr(\mathbf{s}_i^{(2)} \notin {\sc NGB}_{\delta}({S^{(1)}})) \cdot 1 \\ &\leq& 1\cdot \frac{\zeta}{2} + 2\zeta \leq \frac{5 \zeta}{2}~~~~~\left(\because \ \size{S^{(1)}}= \Oh(\frac{r}{\zeta} \log \frac{r}{\zeta})\ \mbox{and} \ \size{J} = \Oh(\frac{\log \size{S^{(1)}}}{\delta})\right)
\end{eqnarray*}

Let us now define another random variable $X$ as $X=\sum\limits_{i=1}^{\size{S^{(2)}}} X_i$.
    
Applying Hoeffding's inequality, we can say that $X \leq 3 \zeta$ holds with probability at least $1 - \frac{1}{t_1^4}$. Thus, we can say that  with probability at least $1 - \frac{1}{t_1^4}$, the fraction of samples in $S^{(2)}$ that are not assigned to some vector in $S^{(1)}$ will be at most $3\zeta$.
    
    
    %Then, by Lemma~\ref{lem:conc}, we can say that the algorithm \cluster outputs a distribution $D'$ such that $d_{EM}(D, D'_{\sigma}) \leq \eps$ for some permutation $\sigma$ over $[n]$. This completes the proof of $(i)$.
    
    \item[(ii)] We proceed in similar manner as above. Let us define a binary random variable $Y_i$ that takes value $1$ if and only if the $i$-th sample of $S^{(2)}$, that is, $\mathbf{s}_i^{(2)}$ is not assigned to any vector in $S^{(1)}$. Note that $Y_i$ is $1$ if $\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}^{(1)} \mid_J) > 2 \delta$ for all $\mathbf{s}^{(1)} \in S^{(1)}$. Similar to the analysis before, we break it into two possible cases: when $\mathbf{s}_i^{(2)} \in {\sc NGB}_{3\delta}({S^{(1)}})$ and when $\mathbf{s}_i^{(2)} \notin {\sc NGB}_{3\delta}({S^{(1)}})$.
    
    So, the probability of $Y_i = 1$ is:
    \begin{eqnarray*}
    \pr(Y_i = 1) &\geq& \pr(\mathbf{s}_i^{(2)} \in {\sc NGB}_{3\delta}({S^{(1)}}))\cdot \prod\limits_{j=1}^{\size{S^{(1)}}}\pr(\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}_j^{(1)} \mid_J) > 2 \delta) + \\
    && \pr(\mathbf{s}_i^{(2)} \notin {\sc NGB}_{3\delta}({S^{(1)}})) \cdot \prod\limits_{j=1}^{\size{S^{(1)}}}\pr(\mu(\mathbf{s}_i^{(2)} \mid_J, \mathbf{s}_j^{(1)} \mid_J) > 2 \delta) \\ &\geq& 0 + 5\zeta \cdot (1 - \frac{\zeta}{2}) > \frac{9 \zeta}{2}~~~~~\left(\because \ \size{S^{(1)}}= \Oh \left(\frac{r}{\zeta} \log \frac{r}{\zeta}\right)\ \mbox{and} \ \size{J} = \Oh\left(\frac{\log \size{S^{(1)}}}{\delta}\right)\right)
    \end{eqnarray*}
    
Now we define a new random variable $Y$ as $Y= \sum\limits_{i=1}^{\size{S^{(2)}}} Y_i$.
    
Applying Hoeffding's inequality, we can say that $Y > 3 \zeta$ holds with probability at least $1 - \frac{1}{t_1^4}$. So, we conclude that with probability at least $1 - \frac{1}{t_1^4}$, the fraction of samples in $S^{(2)}$ that are not assigned to some vector in $S^{(1)}$ will be at least  $3\zeta$.
    
\end{itemize}
\end{proof}

    
    
    % First we prove the following claim.
    
    % \begin{cl}
    % If $\sum\limits_{i=1}^{t_1} D(\mathbf{s}^{(1)}_i) \leq 1 - 5 \zeta$, then $\sum\limits_{i=1}^{t_1} w(\mathbf{s}^{(1)}_i) \leq 1 - 3 \zeta$ holds with probability at least ??.
    % \end{cl}
    
    % \begin{proof}
    % Let $X_j$ be a binary random variable which is $1$ if and only of the $j$-th sample of $S^{(2)}$ is assigned to $\mathbf{s}_i^{(1)}$. So, we have $w(\mathbf{s}_i^{(1)}) = \frac{1}{\size{S^{(2)}}} \sum\limits_{j=1}^{\size{S^{(2)}}} X_j$.
    % Note that $\E[w(\mathbf{s}_i^{(1)})] = D(\mathbf{s}_i^1)$.
    
    % Let $Z$ be a random variable such that $Z = \sum\limits_{i=1}^{t_1} w(\mathbf{s}_i^{(1)})$. Thus, $\E[Z]= \E[\sum\limits_{i=1}^{t_1} w(\mathbf{s}_i^{(1)})] = \sum\limits_{i=1}^{t_1} D(\mathbf{s}_i^{(1)})$
    
    % Applying Chernoff bound, we can say that $\pr(Z > 1 - 3 \zeta) \leq e^{-4 \zeta^2 t_1}$
    
    
    %  %$\pr(X_i=1)\geq \pr(s_i^{2} \in NBG_{3\delta}{S^{(1)}})\cdot \pr(\mu() > 2 \delta) + \pr(s_i^{2} \notin NBG_{3\delta}{S^{(1)}}) \cdot \pr(\mu() \geq 2 \delta) \geq 0 + 5\zeta \cdot  ?? \geq ?? > 4.5 \delta$
     
    % \end{proof}
    
    %Following the above observation, we can say that when $\sum\limits_{i=1}^{t_1} D(\mathbf{s}^{(1)}_i) \leq 1 - 5 \zeta$, $\sum\limits_{i=1}^{t_1} w(\mathbf{s}^{(1)}_i) \leq 1 - 3 \zeta$ holds with probability at least ??. Then the algorithm \find will reject $D$ in Step (iii), which implies that $D$ will be rejected by the algorithm \cluster in Step (i). So, when \cluster outputs a distribution $D'$, we know that $\sum\limits_{i=1}^{t_1} w(\mathbf{s}^{(1)}_i) \geq 1 - 3 \zeta$. This implies that $D$ is $(5 \zeta, \delta)$-concentrated with respect to $S^{(1)}$. By Lemma~\ref{lem:conc}, we know that the algorithm \cluster outputs a distribution $D'$ such that $d_{EM}(D, D'_{\sigma}) \leq \eps$ for some permutation $\sigma$.
    
    %Using Claim~\ref{}, we know that $d_{EM}(D, D'_{\sigma}) \leq 6 \zeta$.
    
    
    %Recall that, by Lemma~\ref{lem:conc}, if $D$ is not $(\zeta, \delta)$-concentrated with respect to the set $S^{(1)}$, the algorithm \cluster will reject $D$ with high probability in Step (i) (when \cluster calls \find, $D$ will be rejected in Step (iii) of \find ). 
    









%The partition is said to be a $(\delta, r)$-clustering of $V$ if $s + 1 \leq r, D(C_0) \leq \delta$, and for every $1 \leq i \leq s$ and $u, v \in C_i$, $\mu(u, v) \leq \delta$, where $\mu$ denotes the normalized Hamming distance.
%Finally, for a partition block $B$ and a row $u$ that intersects $B$, let $u \mid_B$ be the restriction of $u$ to the columns in $B$.
\end{defi}

\input{conc.tex}
